Atomtronic circuits: from many-body physics to quantum technologies

Atomtronics is an emerging field that aims to manipulate ultracold atom moving in matter wave circuits for both fundamental studies in quantum science and technological applications. In this colloquium, we review recent progress in matter-wave circuitry and atomtronics-based quantum technology. After a short introduction to the basic physical principles and the key experimental techniques needed to realize atomtronic systems, we describe the physics of matter-waves in simple circuits such as ring traps and two-terminal systems. The main experimental observations and outstanding questions are discussed. We also present possible applications to a broad range of quantum technologies, from quantum sensing with atom interferometry to future quantum simulation and quantum computation architectures.

==> figures/bib_Backup.tex <==

@article{koepsell2019imaging,
	author = {Koepsell, Joannis and Vijayan, Jayadev and Sompet, Pimonpan and Grusdt, Fabian and Hilker, Timon A. and Demler, Eugene and Salomon, Guillaume and Bloch, Immanuel and Gross, Christian},
	journal = {Nature},
	number = {7769},
	pages = {358--362},
	title = {Imaging magnetic polarons in the doped Fermi--Hubbard model},
	volume = {572},
	year = {2019}}

@article{pigneur2018relaxation,
	author = {Pigneur, Marine and Berrada, Tarik and Bonneau, Marie and Schumm, Thorsten and Demler, Eugene and Schmiedmayer, J\"org},
	journal = {Phys. Rev. Lett.},
	month = {Apr},
	pages = {173601},
	title = {Relaxation to a Phase-Locked Equilibrium State in a One-Dimensional Bosonic Josephson Junction},
	volume = {120},
	year = {2018}}




@article{glazman1988reflectionless,
	author = {{Glazman}, L.~I. and {Lesovik}, G.~B. and {Khmel'Nitski{\v \i}}, D.~E. and {Shekhter}, R.~I.},
	journal = {ZhETF Pisma Redaktsiiu},
	month = aug,
	pages = {218},
	title = {{Reflectionless quantum transport and fundamental ballistic-resistance steps in microscopic constrictions}},
	volume = 48,
	year = 1988}


@article{abad2014persistent,
  title = {Persistent currents in two-component condensates in a toroidal trap},
  author = {Abad, M. and Sartori, A. and Finazzi, S. and Recati, A.},
  journal = {Phys. Rev. A},
  volume = {89},
  issue = {5},
  pages = {053602},
  numpages = {9},
  year = {2014},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.89.053602},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.89.053602}
}
@article{abad2016persistent,
  title = {Persistent currents in coherently coupled Bose-Einstein condensates in a ring trap},
  author = {Abad, Marta},
  journal = {Phys. Rev. A},
  volume = {93},
  issue = {3},
  pages = {033603},
  numpages = {11},
  year = {2016},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.93.033603},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.93.033603}
}

@article{gritsev2007linear,
	author = {Gritsev, Vladimir and Polkovnikov, Anatoli and Demler, Eugene},
	journal = {Phys. Rev. B},
	month = {May},
	pages = {174511},
	title = {Linear response theory for a pair of coupled one-dimensional condensates of interacting atoms},
	volume = {75},
	year = {2007}
}


@article{schweigler2021decay,
	author = {Schweigler, Thomas and Gluza, Marek and Tajik, Mohammadamin and Sotiriadis, Spyros and Cataldini, Federica and Ji, Si-Cong and M{\o}ller, Frederik S. and Sabino, Jo{\~a}o and Rauer, Bernhard and Eisert, Jens and Schmiedmayer, J{\"o}rg},
	journal = {Nature Physics},
	number = {5},
	pages = {559--563},
	title = {Decay and recurrence of non-Gaussian correlations in a quantum many-body system},
	volume = {17},
	year = {2021}}


@article{abanin2019colloquium,
	author = {Abanin, Dmitry A. and Altman, Ehud and Bloch, Immanuel and Serbyn, Maksym},
	journal = {Rev. Mod. Phys.},
	month = {May},
	pages = {021001},
	title = {Colloquium: Many-body localization, thermalization, and entanglement},
	volume = {91},
	year = {2019}}


@article{affleck1988critical,
	author       = {Affleck, Ian},
	title        = {Critical behaviour of SU (n) quantum chains and topological non-linear \$\sigma\$-models},
	journal      = {Nuclear Physics B},
	year         = 1988,
	volume       = 305,
	number       = 4,
	pages        = {582--596},
}
@article{aghamalyan2016atomtronic,
	author       = {Aghamalyan, D and Nguyen, NT and Auksztol, F and Gan, KS and Valado, M Martinez and Condylis, PC and Kwek, LC and Dumke, R and Amico, L},
	title        = {An atomtronic flux qubit: a ring lattice of Bose--Einstein condensates interrupted by three weak links},
	journal      = {New Journal of Physics},
	year         = 2016,
	volume       = 18,
	number       = 7,
	pages        = {075013},
}
@article{aghamalyan_atomtronic_2016,
	author       = {Aghamalyan, D. and Nguyen, N. T. and Auksztol, F. and Gan, K. S. and Valado, M. Martinez and Condylis, P. C. and Kwek, L.-C. and Dumke, R. and Amico, L.},
	title        = {An atomtronic flux qubit: a ring lattice of {Bose}{\textendash}{Einstein} condensates interrupted by three weak links},
	journal      = {New J. Phys.},
	year         = 2016,
	volume       = 18,
	number       = 7,
	pages        = {075013},
}
@article{aghamalyan2015coherent,
	author       = {Aghamalyan, Davit and Cominotti, Marco and Rizzi, Matteo and Rossini, Davide and Hekking, Frank and Minguzzi, Anna and Kwek, Leong Chuan and Amico, Luigi},
	title        = {Coherent superposition of current flows in an atomtronic quantum interference device},
	journal      = {New J. Phys.},
	year         = 2015,
	volume       = 17,
	number       = 4,
	pages        = {045023},
}
@phdthesis{aghamalyan2015atomtronics,
	author       = {Aghamalyan, Davit},
	title        = {Atomtronics: Quantum technology with cold atoms in ring shaped optical lattices},
	school       = {National University of Singapore},
	year         = 2015,
}
@phdthesis{aghamalyan2015atomtronics:,
	author       = {Aghamalyan, Davit},
	title        = {Atomtronics: Quantum technology with cold atoms in ring shaped optical lattices},
	school       = {National University of Singapore},
	year         = 2015,
}
@article{Aharonov-Bohm,
	author       = {Aharonov, Y. and Bohm, D.},
	title        = {Significance of Electromagnetic Potentials in the Quantum Theory},
	journal      = {Phys. Rev.},
	year         = 1959,
	volume       = 115,
	pages        = {485--491},
	month        = {Aug},
}
@article{aharonov1959significance,
	author       = {Aharonov, Y. and Bohm, D.},
	title        = {Significance of Electromagnetic Potentials in the Quantum Theory},
	journal      = {Phys. Rev.},
	year         = 1959,
	volume       = 115,
	pages        = {485--491},
	month        = {Aug},
}
@article{Akatsuka2017APE,
	author       = {Akatsuka, Tomoya and Takahashi, Tadahiro and Katori, Hidetoshi},
	title        = {Optically guided atom interferometer tuned to magic wavelength},
	journal      = {Applied Physics Express},
	year         = 2017,
	volume       = 10,
	number       = 11,
	pages        = 112501,
	month        = {Oct},
}
@article{akatsuka2017optically,
	author       = {Akatsuka, Tomoya and Takahashi, Tadahiro and Katori, Hidetoshi},
	title        = {Optically guided atom interferometer tuned to magic wavelength},
	journal      = {Applied Physics Express},
	year         = 2017,
	volume       = 10,
	number       = 11,
	pages        = 112501,
	month        = {Oct},
}

@article{franke2007optical,
  title={Optical ferris wheel for ultracold atoms},
  author={Franke-Arnold, Sonja and Leach, Jonathan and Padgett, Miles J and Lembessis, Vassilis E and Ellinas, Demos and Wright, Amanda J and Girkin, John M and {\"O}hberg, P and Arnold, Aidan S},
  journal={Optics Express},
  volume={15},
  number={14},
  pages={8619--8625},
  year={2007},
  publisher={Optical Society of America}
}


@article{gauthier2016direct,
  title={Direct imaging of a digital-micromirror device for configurable microscopic optical potentials},
  author={Gauthier, G and Lenton, I and Parry, N McKay and Baker, M and Davis, MJ and Rubinsztein-Dunlop, H and Neely, TW},
  journal={Optica},
  volume={3},
  number={10},
  pages={1136--1143},
  year={2016},
  publisher={Optical Society of America}
}


@article{Albiez:2005aa,
	author       = {Albiez, Michael and Gati, Rudolf and F\"olling, Jonas and Hunsmann, Stefan and Cristiani, Matteo and Oberthaler, Markus K.},
	title        = {Direct Observation of Tunneling and Nonlinear Self-Trapping in a Single Bosonic Josephson Junction},
	journal      = {Phys. Rev. Lett.},
	year         = 2005,
	volume       = 95,
	number       = 1,
	pages        = {010402},
	month        = {Jun},
}
@article{albiez2005direct,
	author       = {Albiez, Michael and Gati, Rudolf and F\"olling, Jonas and Hunsmann, Stefan and Cristiani, Matteo and Oberthaler, Markus K.},
	title        = {Direct Observation of Tunneling and Nonlinear Self-Trapping in a Single Bosonic Josephson Junction},
	journal      = {Phys. Rev. Lett.},
	year         = 2005,
	volume       = 95,
	number       = 1,
	pages        = {010402},
	month        = {Jun},
}

@article{amico2020state,
	author       = {Amico, L and Boshier, M and Birkl, G and Minguzzi, A and Miniatura, C and Kwek, LC and Aghamalyan, D and Ahufinger, V and Anderson, D and Andrei, N and others},
	title        = {State of the art and perspective on atomtronics (2020)},
	journal      = {arXiv preprint arXiv:2008.04439},
}
@article{surace2021scattering,
  title={Scattering of mesons in quantum simulators},
  author={Surace, Federica Maria and Lerose, Alessio},
  journal={New Journal of Physics},
  volume={23},
  number={6},
  pages={062001},
  year={2021},
  publisher={IOP Publishing}
}



@article{clark2017collective,
  title={Collective emission of matter-wave jets from driven Bose--Einstein condensates},
  author={Clark, Logan W and Gaj, Anita and Feng, Lei and Chin, Cheng},
  journal={Nature},
  volume={551},
  number={7680},
  pages={356--359},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{fu2020jet,
  title={Jet Substructure in Fireworks Emission from Nonuniform and Rotating Bose-Einstein Condensates},
  author={Fu, Han and Zhang, Zhendong and Yao, Kai-Xuan and Feng, Lei and Yoo, Jooheon and Clark, Logan W and Levin, K and Chin, Cheng},
  journal={Physical Review Letters},
  volume={125},
  number={18},
  pages={183003},
  year={2020},
  publisher={APS}
}


@article{amicostate,
	author       = {Amico, L and Boshier, M and Birkl, G and Minguzzi, A and Miniatura, C and Kwek, LC and Aghamalyan, D and Ahufinger, V and Anderson, D and Andrei, N and others},
	title        = {State of the art and perspective on atomtronics (2020)},
	journal      = {arXiv preprint arXiv:2008.04439},
}
@article{amico2014superfluid,
	author       = {Amico, Luigi and Aghamalyan, Davit and Auksztol, Filip and Crepaz, Herbert and Dumke, Rainer and Kwek, Leong Chuan},
	title        = {Superfluid qubit systems with ring shaped optical lattices},
	journal      = {Sci. Rep.},
	year         = 2014,
	volume       = 4,
	pages        = 4298,
	month        = {Mar},
}
@article{amico2017focus,
	author       = {Amico, Luigi and Birkl, Gerhard and Boshier, Malcolm and Kwek, Leong-Chuan},
	title        = {Focus on atomtronics-enabled quantum technologies},
	journal      = {New Journal of Physics},
	year         = 2017,
	volume       = 19,
	number       = 2,
	pages        = {020201},
	month        = {feb},
}

@article{bongs2019taking,
  title={Taking atom interferometric quantum sensors from the laboratory to real-world applications},
  author={Bongs, Kai and Holynski, Michael and Vovrosh, Jamie and Bouyer, Philippe and Condon, Gabriel and Rasel, Ernst and Schubert, Christian and Schleich, Wolfgang P and Roura, Albert},
  journal={Nature Reviews Physics},
  volume={1},
  number={12},
  pages={731--739},
  year={2019},
  publisher={Nature Publishing Group}
}



@article{degen2017quantum,
  title={Quantum sensing},
  author={Degen, Christian L and Reinhard, F and Cappellaro, Paola},
  journal={Reviews of modern physics},
  volume={89},
  number={3},
  pages={035002},
  year={2017},
  publisher={APS}
}

@article{amico2004universality,
	author       = {Amico, Luigi and Korepin, Vladimir},
	title        = {Universality of the one-dimensional Bose gas with delta interaction},
	journal      = {Annals of Physics},
	year         = 2004,
	volume       = 314,
	number       = 2,
	pages        = {496--507},
}
@article{amico2005quantum,
	author       = {Amico, Luigi and Osterloh, Andreas and Cataliotti, Francesco},
	title        = {Quantum many particle systems in ring-shaped optical lattices},
	journal      = {Phys. Rev. Lett.},
	year         = 2005,
	volume       = 95,
	number       = 6,
	pages        = {063201},
}
@article{amico2000time,
	author       = {Amico, Luigi and Penna, Vittorio},
	title        = {Time-dependent mean-field theory of the superfluid-insulator phase transition},
	journal      = {Physical Review B},
	year         = 2000,
	volume       = 62,
	number       = 2,
	pages        = 1224,
}
@article{amico2000time-dependent,
	author       = {Amico, Luigi and Penna, Vittorio},
	title        = {Time-dependent mean-field theory of the superfluid-insulator phase transition},
	journal      = {Physical Review B},
	year         = 2000,
	volume       = 62,
	number       = 2,
	pages        = 1224,
}
@article{amico2000algebraic,
	author       = {Amico, Luigi},
	title        = {Algebraic equivalence between certain models for superfluid--insulator transition},
	journal      = {Modern Physics Letters B},
	year         = 2000,
	volume       = 14,
	number       = 21,
	pages        = {759--766},
}
@article{Amico_qubit,
	title        = {Superfluid qubit systems with ring shaped optical lattices},
	author       = {Amico, Luigi and Aghamalyan, Davit and Auksztol, Filip and Crepaz, Herbert and Dumke, Rainer and Kwek, Leong Chuan},
	year         = 2014,
	journal      = {Scientific reports},
	publisher    = {Nature Publishing Group},
	volume       = 4
}
@article{an2018engineering,
	author       = {An, Fangzhao Alex and Meier, Eric J. and Gadway, Bryce},
	title        = {Engineering a Flux-Dependent Mobility Edge in Disordered Zigzag Chains},
	journal      = {Phys. Rev. X},
	year         = 2018,
	volume       = 8,
	pages        = {031045},
	month        = {Aug},
}
@article{PhysRevX.8.031045,
	author       = {An, Fangzhao Alex and Meier, Eric J. and Gadway, Bryce},
	title        = {Engineering a Flux-Dependent Mobility Edge in Disordered Zigzag Chains},
	journal      = {Phys. Rev. X},
	year         = 2018,
	volume       = 8,
	pages        = {031045},
	month        = {Aug},
}
@article{andersson2002multimode,
	author       = {Andersson, E. and Calarco, T. and Folman, R. and Andersson, M. and Hessmo, B. and Schmiedmayer, J.},
	title        = {Multimode Interferometer for Guided Matter Waves},
	journal      = {Phys. Rev. Lett.},
	year         = 2002,
	volume       = 88,
	number       = 10,
	pages        = 100401,
	month        = 3,
}
@article{Andersson2002PRL,
	author       = {Andersson, E. and Calarco, T. and Folman, R. and Andersson, M. and Hessmo, B. and Schmiedmayer, J.},
	title        = {Multimode Interferometer for Guided Matter Waves},
	journal      = {Phys. Rev. Lett.},
	year         = 2002,
	volume       = 88,
	number       = 10,
	pages        = 100401,
	month        = 3,
}
@article{Ando.1987,
	author       = {Ando, Yuji and Itoh, Tomohiro},
	title        = {Calculation of transmission tunneling current across arbitrary potential barriers},
	journal      = {Journal of Applied Physics},
	year         = 1987,
	volume       = 61,
	number       = 4,
	pages        = {1497--1502},
}
@article{ando1987calculation,
	author       = {Ando, Yuji and Itoh, Tomohiro},
	title        = {Calculation of transmission tunneling current across arbitrary potential barriers},
	journal      = {Journal of Applied Physics},
	year         = 1987,
	volume       = 61,
	number       = 4,
	pages        = {1497--1502},
}
@article{andrei1995integrable,
	author       = {Andrei, Natan},
	title        = {Integrable models in condensed matter physics},
	journal      = {Low-Dimensional Quantum Field Theories for Condensed Matter Physicists (World Scientific Publishing Co, 2013) pp},
	year         = 1995,
	pages        = {457--551},
}

@article{ketterle2002nobel,
  title={Nobel lecture: When atoms behave as waves: Bose-Einstein condensation and the atom laser},
  author={Ketterle, Wolfgang},
  journal={Reviews of Modern Physics},
  volume={74},
  number={4},
  pages={1131},
  year={2002},
  publisher={APS}
}

@article{cornell2002nobel,
  title={Nobel Lecture: Bose-Einstein condensation in a dilute gas, the first 70 years and some recent experiments},
  author={Cornell, Eric A and Wieman, Carl E},
  journal={Reviews of Modern Physics},
  volume={74},
  number={3},
  pages={875},
  year={2002},
  publisher={APS}
}

@article{Andrews:1997ab,
	author       = {Andrews, M. R. and Townsend, C. G. and Miesner, H.-J. and Durfee, D. S. and Kurn, D. M. and Ketterle, W.},
	title        = {Observation of Interference Between Two Bose Condensates},
	journal      = {Science},
	year         = 1997,
	volume       = 275,
	number       = 5300,
	pages        = {637--641},
}
@article{andrews1997observation,
	author       = {Andrews, M. R. and Townsend, C. G. and Miesner, H.-J. and Durfee, D. S. and Kurn, D. M. and Ketterle, W.},
	title        = {Observation of Interference Between Two Bose Condensates},
	journal      = {Science},
	year         = 1997,
	volume       = 275,
	number       = 5300,
	pages        = {637--641},
}

@article{anoshkin2012persistent,
  title = {Persistent currents in a bosonic mixture in the ring geometry},
  author = {Anoshkin, K. and Wu, Z. and Zaremba, E.},
  journal = {Phys. Rev. A},
  volume = {88},
  issue = {1},
  pages = {013609},
  numpages = {14},
  year = {2013},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.88.013609},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.88.013609}
}


@article{arabahmadi2021universal,
	author       = {Arabahmadi, Ehsan and Schumayer, Daniel and Hutchinson, David A. W.},
	title        = {Universal nomogram for the atomtronic quantum rotation sensor},
	journal      = {Phys. Rev. A},
	year         = 2021,
	volume       = 103,
	pages        = {043319},
	month        = {Apr},
}
@article{arabamahdi2021universal,
	author       = {Arabahmadi, Ehsan and Schumayer, Daniel and Hutchinson, David A. W.},
	title        = {Universal nomogram for the atomtronic quantum rotation sensor},
	journal      = {Phys. Rev. A},
	year         = 2021,
	volume       = 103,
	pages        = {043319},
	month        = {Apr},
}
@book{arimondo2009atom,
	title        = {Atom Optics and Space Physics: Proceedings of the International School of Physics" Enrico Fermi", Course CLXVIII, Varenna on Lake Como, Villa Monastero, 3-13 July 2007},
	publisher    = {IOS Press},
	year         = 2009,
	author       = {Arimondo, Ennio and Ertmer, Wolfgang and Schleich, Wolfgang and Rasel, EM},
	volume       = 168,
}
@article{arnold2006large,
	author       = {Arnold, Aidan S and Garvie, Craig S and Riis, Erling},
	title        = {Large magnetic storage ring for Bose-Einstein condensates},
	journal      = {Physical Review A},
	year         = 2006,
	volume       = 73,
	number       = 4,
	pages        = {041606},
	month        = {Apr},
}
@article{aubin2006rapid,
	author       = {Aubin, S and Myrskog, S and Extavour, MHT and LeBlanc, LJ and McKay, D and Stummer, A and Thywissen, JH},
	title        = {Rapid sympathetic cooling to Fermi degeneracy on a chip},
	journal      = {Nature Physics},
	year         = 2006,
	volume       = 2,
	number       = 6,
	pages        = {384--387},
}
@article{Averin:1995aa,
	author       = {Averin, D. and Bardas, A.},
	title        = {ac Josephson Effect in a Single Quantum Channel},
	journal      = {Phys. Rev. Lett.},
	year         = 1995,
	volume       = 75,
	pages        = {1831--1834},
	month        = {Aug},
}
@article{averin1995josephson,
	author       = {Averin, D. and Bardas, A.},
	title        = {ac Josephson Effect in a Single Quantum Channel},
	journal      = {Phys. Rev. Lett.},
	year         = 1995,
	volume       = 75,
	pages        = {1831--1834},
	month        = {Aug},
}
@article{buttiker1984quantum,
	author       = {B\"{u}ttiker, M and Imry, Y and Azbel, M Ya},
	title        = {Quantum oscillations in one-dimensional normal-metal rings},
	journal      = {Phys. Rev. A},
	year         = 1984,
	volume       = 30,
	number       = 4,
	pages        = 1982,
}
@article{buttiker1983josephson,
	author       = {B\"{u}ttiker, M. and Imry, Y. and Landauer, R.},
	title        = {Josephson behavior in small normal one-dimensional rings},
	journal      = {Physics Letters A},
	year         = 1983,
	volume       = 96,
	number       = 7,
	pages        = {365--367},
}
@book{baeriswyl2013hubbard,
	title        = {The Hubbard model: its physics and mathematical physics},
	publisher    = {Springer Science \& Business Media},
	year         = 2013,
	author       = {Baeriswyl, Dionys and Campbell, David K and Carmelo, Jose MP and Guinea, Francisco and Louis, Enrique},
	volume       = 343,
}
@book{baeriswyl2013the,
	title        = {The Hubbard model: its physics and mathematical physics},
	publisher    = {Springer Science \& Business Media},
	year         = 2013,
	author       = {Baeriswyl, Dionys and Campbell, David K and Carmelo, Jose MP and Guinea, Francisco and Louis, Enrique},
	volume       = 343,
}
@article{baiborodov1963adiabatic,
	author       = {Baiborodov, Yu T and Ioffe, M S and Petrov, V M and Sobolev, R I},
	title        = {An adiabatic trap with combined magnetic field},
	journal      = {Journal of Nuclear Energy. Part C},
	year         = 1963,
	volume       = 5,
	number       = 6,
	pages        = 409,
}
@article{Baiborodov1963JONEPC,
	author       = {Baiborodov, Yu T and Ioffe, M S and Petrov, V M and Sobolev, R I},
	title        = {An adiabatic trap with combined magnetic field},
	journal      = {Journal of Nuclear Energy. Part C},
	year         = 1963,
	volume       = 5,
	number       = 6,
	pages        = 409,
}
@article{Barontini:2013aa,
	author       = {Barontini, G. and Labouvie, R. and Stubenrauch, F. and Vogler, A. and Guarrera, V. and Ott, H.},
	title        = {Controlling the Dynamics of an Open Many-Body Quantum System with Localized Dissipation},
	journal      = {Phys. Rev. Lett.},
	year         = 2013,
	volume       = 110,
	pages        = {035302},
	month        = {Jan},
}
@article{barontini2013controlling,
	author       = {Barontini, G. and Labouvie, R. and Stubenrauch, F. and Vogler, A. and Guarrera, V. and Ott, H.},
	title        = {Controlling the Dynamics of an Open Many-Body Quantum System with Localized Dissipation},
	journal      = {Phys. Rev. Lett.},
	year         = 2013,
	volume       = 110,
	pages        = {035302},
	month        = {Jan},
}
@article{barrett2014sagnac,
	author       = {Barrett, Brynle and Geiger, R\'{e}my and Dutta, Indranil and Meunier, Matthieu and Canuel, Benjamin and Gauguet, Alexandre and Bouyer, Philippe and Landragin, Arnaud},
	title        = {The Sagnac effect: 20 years of development in matter-wave interferometry},
	journal      = {Comptes Rendus Physique},
	year         = 2014,
	volume       = 15,
	number       = 10,
	pages        = {875--883},
	month        = dec,
}
@article{barrett2014the,
	author       = {Barrett, Brynle and Geiger, R\'{e}my and Dutta, Indranil and Meunier, Matthieu and Canuel, Benjamin and Gauguet, Alexandre and Bouyer, Philippe and Landragin, Arnaud},
	title        = {The Sagnac effect: 20 years of development in matter-wave interferometry},
	journal      = {Comptes Rendus Physique},
	year         = 2014,
	volume       = 15,
	number       = 10,
	pages        = {875--883},
	month        = dec,
}
@article{beattie2013persistent,
	author       = {Beattie, Scott and Moulder, Stuart and Fletcher, Richard J. and Hadzibabic, Zoran},
	title        = {Persistent Currents in Spinor Condensates},
	journal      = {Phys. Rev. Lett.},
	year         = 2013,
	volume       = 110,
	number       = 2,
	month        = jan,
}
@article{bell2016bose,
	author       = {Bell, Thomas A and Glidden, Jake A P and Humbert, Leif and Bromley, Michael W J and Haine, Simon A and Davis, Matthew J and Neely, Tyler W and Baker, Mark A and Rubinsztein-Dunlop, Halina},
	title        = {Bose{\textendash}Einstein condensation in large time-averaged optical ring potentials},
	journal      = {New Journal of Physics},
	year         = 2016,
	volume       = 18,
	number       = 3,
	pages        = {035003},
	month        = {mar},
}
@article{bell2016bosetextendasheinstein,
	author       = {Bell, Thomas A and Glidden, Jake A P and Humbert, Leif and Bromley, Michael W J and Haine, Simon A and Davis, Matthew J and Neely, Tyler W and Baker, Mark A and Rubinsztein-Dunlop, Halina},
	title        = {Bose{\textendash}Einstein condensation in large time-averaged optical ring potentials},
	journal      = {New Journal of Physics},
	year         = 2016,
	volume       = 18,
	number       = 3,
	pages        = {035003},
	month        = {mar},
}
@article{bell2018phase,
	author       = {Bell, Thomas A. and Gauthier, Guillaume and Neely, Tyler W. and Rubinsztein-Dunlop, Halina and Davis, Matthew J. and Baker, Mark A.},
	title        = {Phase and micromotion of Bose-Einstein condensates in a time-averaged ring trap},
	journal      = {Physical Review A},
	year         = 2018,
	volume       = 98,
	number       = 1,
	pages        = {013604},
	month        = {Jul},
}
@article{Bentine2017Species,
	author       = {Bentine, E and Harte, T L and Luksch, K and Barker, A J and Mur-Petit, J and Yuen, B and Foot, C J},
	title        = {Species-selective confinement of atoms dressed with multiple radiofrequencies},
	journal      = {Journal of Physics B},
	year         = 2017,
	volume       = 50,
	number       = 9,
	pages        = {094002},
	month        = {apr},
}
@article{bentine2017species-selective,
	author       = {Bentine, E and Harte, T L and Luksch, K and Barker, A J and Mur-Petit, J and Yuen, B and Foot, C J},
	title        = {Species-selective confinement of atoms dressed with multiple radiofrequencies},
	journal      = {Journal of Physics B},
	year         = 2017,
	volume       = 50,
	number       = 9,
	pages        = {094002},
	month        = {apr},
}
@book{berman1997atom,
	title        = {Atom interferometry},
	publisher    = {Academic press},
	year         = 1997,
	author       = {Berman, Paul R},
}
@article{bernon2013manipulation,
	author       = {Bernon, Simon and Hattermann, Helge and Bothner, Daniel and Knufinke, Martin and Weiss, Patrizia and Jessen, Florian and Cano, Daniel and Kemmler, Matthias and Kleiner, Reinhold and Koelle, Dieter and others},
	title        = {Manipulation and coherence of ultra-cold atoms on a superconducting atom chip},
	journal      = {Nature communications},
	year         = 2013,
	volume       = 4,
	number       = 1,
	pages        = {1--8},
}
@article{Betz:2011aa,
	author       = {Betz, T. and Manz, S. and B\"ucker, R. and Berrada, T. and Koller, Ch. and Kazakov, G. and Mazets, I. E. and Stimming, H.-P. and Perrin, A. and Schumm, T. and Schmiedmayer, J.},
	title        = {Two-Point Phase Correlations of a One-Dimensional Bosonic Josephson Junction},
	journal      = {Phys. Rev. Lett.},
	year         = 2011,
	volume       = 106,
	pages        = {020407},
	month        = {Jan},
}
@article{betz2011two-point,
	author       = {Betz, T. and Manz, S. and B\"ucker, R. and Berrada, T. and Koller, Ch. and Kazakov, G. and Mazets, I. E. and Stimming, H.-P. and Perrin, A. and Schumm, T. and Schmiedmayer, J.},
	title        = {Two-Point Phase Correlations of a One-Dimensional Bosonic Josephson Junction},
	journal      = {Phys. Rev. Lett.},
	year         = 2011,
	volume       = 106,
	pages        = {020407},
	month        = {Jan},
}
@article{binanti2021dissipation,
  title={Dissipation and fluctuations in elongated bosonic Josephson junctions},
  author={Binanti, F and Furutani, K and Salasnich, L},
  journal={arXiv preprint arXiv:2104.11259},
  year={2021}
}

@article{birkl2001atom,
	author       = {Birkl, G and Buchkremer, FBJ and Dumke, Rainer and Ertmer, Wolfgang},
	title        = {Atom optics with microfabricated optical elements},
	journal      = {Optics Communications},
	year         = 2001,
	volume       = 191,
	number       = {1-2},
	pages        = {67--81},
}
@article{bleszynski-jayich2009persistent,
	author       = {Bleszynski-Jayich, AC and Shanks, WE and Peaudecerf, B and Ginossar, E and Von Oppen, F and Glazman, L and Harris, JGE},
	title        = {Persistent currents in normal metal rings},
	journal      = {Science},
	year         = 2009,
	volume       = 326,
	number       = 5950,
	pages        = {272--275},
}
@article{bleszynski2009persistent,
	author       = {Bleszynski-Jayich, AC and Shanks, WE and Peaudecerf, B and Ginossar, E and Von Oppen, F and Glazman, L and Harris, JGE},
	title        = {Persistent currents in normal metal rings},
	journal      = {Science},
	year         = 2009,
	volume       = 326,
	number       = 5950,
	pages        = {272--275},
}
@article{bloch2008many,
	author       = {Bloch, I. and Dalibard, J. and Zwerger, W.},
	title        = {Many-body physics with ultracold gases},
	journal      = {Rev. Mod. Phys.},
	year         = 2008,
	volume       = 80,
	number       = 3,
	pages        = {885--964},
}
@article{bloch2008many-body,
	author       = {Bloch, I. and Dalibard, J. and Zwerger, W.},
	title        = {Many-body physics with ultracold gases},
	journal      = {Rev. Mod. Phys.},
	year         = 2008,
	volume       = 80,
	number       = 3,
	pages        = {885--964},
}
@article{bloch2005ultracold,
	author       = {Bloch, Immanuel},
	title        = {Ultracold quantum gases in optical lattices},
	journal      = {Nat. Phys.},
	year         = 2005,
	volume       = 1,
	number       = 1,
	pages        = {23--30},
}

@book{lewenstein2012ultracold,
  title={Ultracold Atoms in Optical Lattices: Simulating quantum many-body systems},
  author={Lewenstein, Maciej and Sanpera, Anna and Ahufinger, Veronica},
  year={2012},
  publisher={Oxford University Press}
}


@article{boada2012quantum,
	author       = {Boada, O. and Celi, A. and Latorre, J. I. and Lewenstein, M.},
	title        = {Quantum Simulation of an Extra Dimension},
	journal      = {Phys. Rev. Lett.},
	year         = 2012,
	volume       = 108,
	pages        = 133001,
	month        = {Mar},
}
@article{PhysRevLett.108.133001,
	author       = {Boada, O. and Celi, A. and Latorre, J. I. and Lewenstein, M.},
	title        = {Quantum Simulation of an Extra Dimension},
	journal      = {Phys. Rev. Lett.},
	year         = 2012,
	volume       = 108,
	pages        = 133001,
	month        = {Mar},
}
@article{bongs2001waveguide,
	author       = {Bongs, K. and Burger, S. and Dettmer, S. and Hellweg, D. and Arlt, J. and Ertmer, W. and Sengstock, K.},
	title        = {Waveguide for Bose-Einstein condensates},
	journal      = {Physical Review A - Atomic, Molecular, and Optical Physics},
	year         = 2001,
	volume       = 63,
	pages        = {031602(R)},
}
@article{boyer2004dynamic,
	author       = {Boyer, V. and Chandrashekar, C. M. and Foot, C. J. and Laczik, Z. J.},
	title        = {Dynamic optical trap generation using FLC SLMs for the manipulation of cold atoms Wave-Optical Engineering},
	journal      = {Journal of Modern Optics},
	year         = 2004,
	volume       = 51,
	number       = 14,
	pages        = {2235--2240},
}
@article{boyer2006dynamic,
	author       = {Boyer, V. and Godun, R. M. and Smirne, G. and Cassettari, D. and Chandrashekar, C. M. and Deb, A. B. and Laczik, Z. J. and Foot, C. J.},
	title        = {Dynamic manipulation of Bose-Einstein condensates with a spatial light modulator},
	journal      = {Physical Review A (Atomic, Molecular, and Optical Physics)},
	year         = 2006,
	volume       = 73,
	number       = 3,
	pages        = {031402},
}
@article{Brantut:2013aa,
	author       = {Brantut, Jean-Philippe and Grenier, Charles and Meineke, Jakob and Stadler, David and Krinner, Sebastian and Kollath, Corinna and Esslinger, Tilman and Georges, Antoine},
	title        = {A Thermoelectric Heat Engine with Ultracold Atoms},
	journal      = {Science},
	year         = 2013,
	volume       = 342,
	number       = 6159,
	pages        = {713--715},
}
@article{brantut2013thermoelectric,
	author       = {Brantut, Jean-Philippe and Grenier, Charles and Meineke, Jakob and Stadler, David and Krinner, Sebastian and Kollath, Corinna and Esslinger, Tilman and Georges, Antoine},
	title        = {A Thermoelectric Heat Engine with Ultracold Atoms},
	journal      = {Science},
	year         = 2013,
	volume       = 342,
	number       = 6159,
	pages        = {713--715},
}
@article{Brantut:2012aa,
	author       = {Brantut, Jean-Philippe and Meineke, Jakob and Stadler, David and Krinner, Sebastian and Esslinger, Tilman},
	title        = {Conduction of Ultracold Fermions Through a Mesoscopic Channel},
	journal      = {Science},
	year         = 2012,
	volume       = 337,
	number       = 6098,
	pages        = {1069--1071},
}
@article{brantut2012conduction,
	author       = {Brantut, Jean-Philippe and Meineke, Jakob and Stadler, David and Krinner, Sebastian and Esslinger, Tilman},
	title        = {Conduction of Ultracold Fermions Through a Mesoscopic Channel},
	journal      = {Science},
	year         = 2012,
	volume       = 337,
	number       = 6098,
	pages        = {1069--1071},
}
@book{breuer2002the,
	title        = {The theory of open quantum systems},
	publisher    = {Oxford University Press on Demand},
	year         = 2002,
	author       = {Breuer, Heinz-Peter and Petruccione, Francesco},
}
@book{breuer2002theory,
	title        = {The theory of open quantum systems},
	publisher    = {Oxford University Press on Demand},
	year         = 2002,
	author       = {Breuer, Heinz-Peter and Petruccione, Francesco},
}
@article{Bruderer:2012aa,
	author       = {Bruderer, M. and Belzig, W.},
	title        = {Mesoscopic transport of fermions through an engineered optical lattice connecting two reservoirs},
	journal      = {Phys. Rev. A},
	year         = 2012,
	volume       = 85,
	pages        = {013623},
	month        = {Jan},
}
@article{bruderer2012mesoscopic,
	author       = {Bruderer, M. and Belzig, W.},
	title        = {Mesoscopic transport of fermions through an engineered optical lattice connecting two reservoirs},
	journal      = {Phys. Rev. A},
	year         = 2012,
	volume       = 85,
	pages        = {013623},
	month        = {Jan},
}
@article{Bucker2011NP,
	author       = {Bucker, R. and Grond, J. and Manz, S. and Berrada, T. and Betz, T. and Koller, C. and Hohenester, U. and Schumm, T. and Perrin, A. and Schmiedmayer, J.},
	title        = {Twin-atom beams},
	journal      = {Nature Physics},
	year         = 2011,
	volume       = 7,
	number       = 8,
	pages        = {608--611},
	month        = {Aug},
}
@article{bucker2011twin-atom,
	author       = {Bucker, R. and Grond, J. and Manz, S. and Berrada, T. and Betz, T. and Koller, C. and Hohenester, U. and Schumm, T. and Perrin, A. and Schmiedmayer, J.},
	title        = {Twin-atom beams},
	journal      = {Nature Physics},
	year         = 2011,
	volume       = 7,
	number       = 8,
	pages        = {608--611},
	month        = {Aug},
}
@article{buluta2009quantum,
	author       = {Buluta, Iulia and Nori, Franco},
	title        = {Quantum simulators},
	journal      = {Science},
	year         = 2009,
	volume       = 326,
	number       = 5949,
	pages        = {108--111},
}
@article{Burchianti:2018aa,
	author       = {Burchianti, A. and Scazza, F. and Amico, A. and Valtolina, G. and Seman, J. A. and Fort, C. and Zaccanti, M. and Inguscio, M. and Roati, G.},
	title        = {Connecting Dissipation and Phase Slips in a Josephson Junction between Fermionic Superfluids},
	journal      = {Phys. Rev. Lett.},
	year         = 2018,
	volume       = 120,
	pages        = {025302},
	month        = {Jan},
}

@article{Burchianti2018,
	author       = {Burchianti, A. and Scazza, F. and Amico, A. and Valtolina, G. and Seman, J. A. and Fort, C. and Zaccanti, M. and Inguscio, M. and Roati, G.},
	title        = {Connecting Dissipation and Phase Slips in a Josephson Junction between Fermionic Superfluids},
	journal      = {Phys. Rev. Lett.},
	year         = 2018,
	volume       = 120,
	pages        = {025302},
	month        = {Jan},
}
@article{burchianti2018connecting,
	author       = {Burchianti, A. and Scazza, F. and Amico, A. and Valtolina, G. and Seman, J. A. and Fort, C. and Zaccanti, M. and Inguscio, M. and Roati, G.},
	title        = {Connecting Dissipation and Phase Slips in a Josephson Junction between Fermionic Superfluids},
	journal      = {Phys. Rev. Lett.},
	year         = 2018,
	volume       = 120,
	pages        = {025302},
	month        = {Jan},
}
@article{buser2020interacting,
	author       = {Buser, Maximilian and Hubig, Claudius and Schollw\"{o}ck, Ulrich and Tarruell, Leticia and Heidrich-Meisner, Fabian},
	title        = {Interacting bosonic flux ladders with a synthetic dimension: Ground-state phases and quantum quench dynamics},
	journal      = {Physical Review A},
	year         = 2020,
	volume       = 102,
	number       = 5,
	pages        = {053314},
}
@article{byers1961theoretical,
	author       = {Byers, N and Yang, CN},
	title        = {Theoretical considerations concerning quantized magnetic flux in superconducting cylinders},
	journal      = {Phys. Rev. Lett.},
	year         = 1961,
	volume       = 7,
	number       = 2,
	pages        = 46,
}
@article{cai2021persistent,
	author       = {Cai, Yanping and Allman, Daniel G and Sabharwal, Parth and Wright, Kevin C},
	title        = {Persistent currents in rings of ultracold fermionic atoms},
	journal      = {arXiv preprint arXiv:2104.02218},
	year         = 2021,
}
@article{Caliga.2012,
	author       = {Caliga, Seth C and Straatsma, Cameron J E and Zozulya, Alex A and Anderson, Dana Z},
	title        = {A Matterwave Transistor Oscillator},
	journal      = {arXiv.org},
	year         = 2012,
	month        = {08},
}
@article{caliga2012matterwave,
	author       = {Caliga, Seth C and Straatsma, Cameron J E and Zozulya, Alex A and Anderson, Dana Z},
	title        = {A Matterwave Transistor Oscillator},
	journal      = {arXiv.org},
	year         = 2012,
	month        = {08},
}
@article{caliga2016transport,
	author       = {Caliga, Seth C and Straatsma, Cameron JE and Anderson, Dana Z},
	title        = {Transport dynamics of ultracold atoms in a triple-well transistor-like potential},
	journal      = {New Journal of Physics},
	year         = 2016,
	volume       = 18,
	number       = 2,
	pages        = {025010},
	month        = feb,
}
@article{caliga2017experimental,
	author       = {Caliga, Seth C and Straatsma, Cameron JE and Anderson, Dana Z},
	title        = {Experimental demonstration of an atomtronic battery},
	journal      = {New Journal of Physics},
	year         = 2017,
	volume       = 19,
	number       = 1,
	pages        = {013036},
	month        = {jan},
}
@article{caliga2016principles,
	author       = {Caliga, Seth C and Straatsma, Cameron JE and Zozulya, Alex A and Anderson, Dana Z},
	title        = {Principles of an atomtronic transistor},
	journal      = {New Journal of Physics},
	year         = 2016,
	volume       = 18,
	number       = 1,
	pages        = {015012},
	month        = {jan},
}
@article{Calogero_1975,
	author       = {Calogero, F. and Degasperis, A.},
	title        = {Comparison between the exact and Hartree solutions of a one-dimensional many-body problem},
	journal      = {Phys. Rev. A},
	year         = 1975,
	volume       = 11,
	pages        = {265--269},
	month        = {Jan},
}
@article{calogero1975comparison,
	author       = {Calogero, F. and Degasperis, A.},
	title        = {Comparison between the exact and Hartree solutions of a one-dimensional many-body problem},
	journal      = {Phys. Rev. A},
	year         = 1975,
	volume       = 11,
	pages        = {265--269},
	month        = {Jan},
}
@article{cano2008meissner,
	author       = {Cano, D. and Kasch, B. and Hattermann, H. and Kleiner, R. and Zimmermann, C. and Koelle, D. and Fort\'agh, J.},
	title        = {Meissner Effect in Superconducting Microtraps},
	journal      = {Phys. Rev. Lett.},
	year         = 2008,
	volume       = 101,
	pages        = 183006,
	month        = {Oct},
}
@article{PhysRevLett.101.183006,
	author       = {Cano, D. and Kasch, B. and Hattermann, H. and Kleiner, R. and Zimmermann, C. and Koelle, D. and Fort\'agh, J.},
	title        = {Meissner Effect in Superconducting Microtraps},
	journal      = {Phys. Rev. Lett.},
	year         = 2008,
	volume       = 101,
	pages        = 183006,
	month        = {Oct},
}
@article{cappellini2014direct,
	author       = {Cappellini, Giacomo and Mancini, Marco and Pagano, Guido and Lombardi, Pietro and Livi, Lorenzo and de Cumis, M Siciliani and Cancio, Pablo and Pizzocaro, Marco and Calonico, Davide and Levi, Filippo and others},
	title        = {Direct observation of coherent interorbital spin-exchange dynamics},
	journal      = {Phys. Rev. Lett.},
	year         = 2014,
	volume       = 113,
	number       = 12,
	pages        = 120402,
}
@article{capponi2016phases,
	author       = {Capponi, Sylvain and Lecheminant, Philippe and Totsuka, Keisuke},
	title        = {Phases of one-dimensional SU (N) cold atomic Fermi gases---From molecular Luttinger liquids to topological phases},
	journal      = {Annals of Physics},
	year         = 2016,
	volume       = 367,
	pages        = {50--95},
}
@article{cazalilla2014ultracold,
	author       = {Cazalilla, Miguel A and Rey, Ana Maria},
	title        = {Ultracold Fermi gases with emergent SU (N) symmetry},
	journal      = {Reports on Progress in Physics},
	year         = 2014,
	volume       = 77,
	number       = 12,
	pages        = 124401,
}
@article{celi2014synthetic,
	author       = {Celi, A. and Massignan, P. and Ruseckas, J. and Goldman, N. and Spielman, I. B. and Juzeli\ifmmode \bar{u}\else \={u}\fi{}nas, G. and Lewenstein, M.},
	title        = {Synthetic Gauge Fields in Synthetic Dimensions},
	journal      = {Phys. Rev. Lett.},
	year         = 2014,
	volume       = 112,
	pages        = {043001},
	month        = {Jan},
}
@article{chakraborty1994electron,
	author       = {Chakraborty, Tapash and Pietil\"{a}inen, Pekka},
	title        = {Electron-electron interaction and the persistent current in a quantum ring},
	journal      = {Physical Review B},
	year         = 1994,
	volume       = 50,
	number       = 12,
	pages        = 8460,
}
@article{chakraborty1994electron-electron,
	author       = {Chakraborty, Tapash and Pietil\"{a}inen, Pekka},
	title        = {Electron-electron interaction and the persistent current in a quantum ring},
	journal      = {Physical Review B},
	year         = 1994,
	volume       = 50,
	number       = 12,
	pages        = 8460,
}
@article{chetcuti2020persistent,
	author       = {Chetcuti, Wayne J. and Haug, Tobias and Kwek, Leong-Chuan and Amico, Luigi},
	title        = {Persistent Current of SU(N) Fermions},
}
@article{chetcutipersistent,
	author       = {Chetcuti, Wayne J. and Haug, Tobias and Kwek, Leong-Chuan and Amico, Luigi},
	title        = {Persistent Current of SU(N) Fermions},
}
@article{Chien:2014aa,
	author       = {Chien, Chih-Chun and Di Ventra, Massimiliano and Zwolak, Michael},
	title        = {Landauer, Kubo, and microcanonical approaches to quantum transport and noise: A comparison and implications for cold-atom dynamics},
	journal      = {Phys. Rev. A},
	year         = 2014,
	volume       = 90,
	pages        = {023624},
	month        = {Aug},
}
@article{chien2014landauer,
	author       = {Chien, Chih-Chun and Di Ventra, Massimiliano and Zwolak, Michael},
	title        = {Landauer, Kubo, and microcanonical approaches to quantum transport and noise: A comparison and implications for cold-atom dynamics},
	journal      = {Phys. Rev. A},
	year         = 2014,
	volume       = 90,
	pages        = {023624},
	month        = {Aug},
}
@article{cirac2012goals,
	author       = {Cirac, J. Ignacio and Zoller, Peter},
	title        = {Goals and opportunities in quantum simulation},
	journal      = {Nat Phys},
	year         = 2012,
	volume       = 8,
	number       = 4,
	pages        = {264--266},
	month        = {04},
}
@article{cohen-tannoudji1977dressed-atom,
	author       = {Cohen-Tannoudji, C and Reynaud, S},
	title        = {Dressed-atom description of resonance fluorescence and absorption spectra of a multi-level atom in an intense laser beam},
	journal      = {Journal of Physics B: Atomic and Molecular Physics},
	year         = 1977,
	volume       = 10,
	number       = 3,
	pages        = {345--363},
	month        = {feb},
}
@article{Tannoudji1977Dressed,
	author       = {Cohen-Tannoudji, C and Reynaud, S},
	title        = {Dressed-atom description of resonance fluorescence and absorption spectra of a multi-level atom in an intense laser beam},
	journal      = {Journal of Physics B: Atomic and Molecular Physics},
	year         = 1977,
	volume       = 10,
	number       = 3,
	pages        = {345--363},
	month        = {feb},
}
@article{Colombe2004EL,
	author       = {Colombe, Y. and Knyazchyan, E. and Morizot, O. and Mercier, Brigitte and Lorent, V. and Perrin, H\'{e}l\`{e}ne},
	title        = {Ultracold atoms confined in rf-induced two-dimensional trapping potentials},
	journal      = {Europhysics Letters},
	year         = 2004,
	volume       = 467,
	pages        = {593--599},
	month        = 8,
}
@article{colombe2004ultracold,
	author       = {Colombe, Y. and Knyazchyan, E. and Morizot, O. and Mercier, Brigitte and Lorent, V. and Perrin, H\'{e}l\`{e}ne},
	title        = {Ultracold atoms confined in rf-induced two-dimensional trapping potentials},
	journal      = {Europhysics Letters},
	year         = 2004,
	volume       = 467,
	pages        = {593--599},
	month        = 8,
}
@article{cominotti2015optimal,
	author       = {Cominotti, Marco and Rizzi, Matteo and Rossini, Davide and Aghamalyan, Davit and Amico, Luigi and Kwek, Leon C and Hekking, Frank and Minguzzi, Anna},
	title        = {Optimal scaling of persistent currents for interacting bosons on a ring},
	journal      = {The European Physical Journal Special Topics},
	year         = 2015,
	volume       = 224,
	number       = 3,
	pages        = {519--524},
}
@article{cominotti2015scaling,
	author       = {Cominotti, Marco and Rizzi, Matteo and Rossini, Davide and Aghamalyan, Davit and Amico, Luigi and Kwek, Leon C and Hekking, Frank and Minguzzi, Anna},
	title        = {Optimal scaling of persistent currents for interacting bosons on a ring},
	journal      = {The European Physical Journal Special Topics},
	year         = 2015,
	volume       = 224,
	number       = 3,
	pages        = {519--524},
}
@article{cominotti2014optimal,
	author       = {Cominotti, Marco and Rossini, Davide and Rizzi, Matteo and Hekking, Frank and Minguzzi, Anna},
	title        = {Optimal persistent currents for interacting bosons on a ring with a gauge field},
	journal      = {Phys. Rev. Lett.},
	year         = 2014,
	volume       = 113,
	number       = 2,
	pages        = {025301},
	month        = {jul},
}
@article{corman2014quench,
	author       = {Corman, Laura and Chomaz, Lauriane and Bienaim\'{e}, Tom and Desbuquois, R\'{e}mi and Weitenberg, Christof and Nascimbene, Sylvain and Dalibard, Jean and Beugnon, J\'{e}r\^{o}me},
	title        = {Quench-induced supercurrents in an annular Bose gas},
	journal      = {Phys. Rev. Lett.},
	year         = 2014,
	volume       = 113,
	number       = 13,
	pages        = 135302,
	month        = {Sep},
}
@article{corman2014quench-induced,
	author       = {Corman, Laura and Chomaz, Lauriane and Bienaim\'{e}, Tom and Desbuquois, R\'{e}mi and Weitenberg, Christof and Nascimbene, Sylvain and Dalibard, Jean and Beugnon, J\'{e}r\^{o}me},
	title        = {Quench-induced supercurrents in an annular Bose gas},
	journal      = {Phys. Rev. Lett.},
	year         = 2014,
	volume       = 113,
	number       = 13,
	pages        = 135302,
	month        = {Sep},
}
@article{Corman:2019aa,
	author       = {Corman, Laura and Fabritius, Philipp and H\"ausler, Samuel and Mohan, Jeffrey and Dogra, Lena H. and Husmann, Dominik and Lebrat, Martin and Esslinger, Tilman},
	title        = {Quantized conductance through a dissipative atomic point contact},
	journal      = {Phys. Rev. A},
	year         = 2019,
	volume       = 100,
	pages        = {053605},
	month        = {Nov},
}
@article{corman2019quantized,
	author       = {Corman, Laura and Fabritius, Philipp and H\"ausler, Samuel and Mohan, Jeffrey and Dogra, Lena H. and Husmann, Dominik and Lebrat, Martin and Esslinger, Tilman},
	title        = {Quantized conductance through a dissipative atomic point contact},
	journal      = {Phys. Rev. A},
	year         = 2019,
	volume       = 100,
	pages        = {053605},
	month        = {Nov},
}
@article{Couvert:2008mh,
	author       = {Couvert and Couvert, A. and Jeppesen, M. and Kawalec, T. and Reinaudi, G. and Mathevet, R. and Gu\'{e}ry-Odelin, D.},
	title        = {A quasi-monomode guided atom laser from an all-optical Bose-Einstein condensate},
	journal      = {EPL},
	year         = 2008,
	volume       = 83,
	number       = 5,
	pages        = {6 pages},
}
@article{couvert2008quasi-monomode,
	author       = {Couvert and Couvert, A. and Jeppesen, M. and Kawalec, T. and Reinaudi, G. and Mathevet, R. and Gu\'{e}ry-Odelin, D.},
	title        = {A quasi-monomode guided atom laser from an all-optical Bose-Einstein condensate},
	journal      = {EPL},
	year         = 2008,
	volume       = 83,
	number       = 5,
	pages        = {6 pages},
}
@article{cronin2009optics,
	author       = {Cronin, Alexander D and Schmiedmayer, J\"{o}rg and Pritchard, David E},
	title        = {Optics and interferometry with atoms and molecules},
	journal      = {Reviews of Modern Physics},
	year         = 2009,
	volume       = 81,
	number       = 3,
	pages        = 1051,
}
@book{Cuevas:2017wb,
	title        = {Molecular Electronics},
	publisher    = {WORLD SCIENTIFIC},
	year         = 2017,
	author       = {Cuevas, Juan Carlos and Scheer, Elke},
	volume       = {Volume 15},
	month        = {2021/05/19},
}
@book{cuevas2017molecular,
	title        = {Molecular Electronics},
	publisher    = {WORLD SCIENTIFIC},
	year         = 2017,
	author       = {Cuevas, Juan Carlos and Scheer, Elke},
	volume       = {Volume 15},
	month        = {2021/05/19},
}
@article{curtis2002dynamic,
	author       = {Curtis, Jennifer E. and Koss, Brian A. and Grier, David G.},
	title        = {Dynamic holographic optical tweezers},
	journal      = {Optics Communications},
	year         = 2002,
	volume       = 207,
	number       = 1,
	pages        = {169--175},
}
@article{daley2008andreev,
	author       = {Daley, AJ and Zoller, P and Trauzettel, B},
	title        = {Andreev-like reflections with cold atoms},
	journal      = {Phys. Rev. Lett.},
	year         = 2008,
	volume       = 100,
	number       = 11,
	pages        = 110404,
}
@article{daley2008andreev-like,
	author       = {Daley, AJ and Zoller, P and Trauzettel, B},
	title        = {Andreev-like reflections with cold atoms},
	journal      = {Phys. Rev. Lett.},
	year         = 2008,
	volume       = 100,
	number       = 11,
	pages        = 110404,
}

@article{giorgini2008theory,
  title={Theory of ultracold atomic Fermi gases},
  author={Giorgini, Stefano and Pitaevskii, Lev P and Stringari, Sandro},
  journal={Reviews of Modern Physics},
  volume={80},
  number={4},
  pages={1215},
  year={2008},
  publisher={APS}
}
@article{Dalfovo:1999aa,
	author       = {Dalfovo, Franco and Giorgini, Stefano and Pitaevskii, Lev P. and Stringari, Sandro},
	title        = {Theory of Bose-Einstein condensation in trapped gases},
	journal      = {Rev. Mod. Phys.},
	year         = 1999,
	volume       = 71,
	number       = 3,
	pages        = {463--512},
	month        = {Apr},
}
@article{dalfovo1999theory,
	author       = {Dalfovo, Franco and Giorgini, Stefano and Pitaevskii, Lev P. and Stringari, Sandro},
	title        = {Theory of Bose-Einstein condensation in trapped gases},
	journal      = {Rev. Mod. Phys.},
	year         = 1999,
	volume       = 71,
	number       = 3,
	pages        = {463--512},
	month        = {Apr},
}
@article{dalibard2011colloquium,
	author       = {Dalibard, Jean and Gerbier, Fabrice and Juzeli\={u}nas, Gediminas and \"{O}hberg, Patrik},
	title        = {Colloquium: Artificial gauge potentials for neutral atoms},
	journal      = {Rev. Mod. Phys.},
	year         = 2011,
	volume       = 83,
	number       = 4,
	pages        = 1523,
}
@article{dalibard2011colloquium:,
	author       = {Dalibard, Jean and Gerbier, Fabrice and Juzeli\={u}nas, Gediminas and \"{O}hberg, Patrik},
	title        = {Colloquium: Artificial gauge potentials for neutral atoms},
	journal      = {Rev. Mod. Phys.},
	year         = 2011,
	volume       = 83,
	number       = 4,
	pages        = 1523,
}
@article{dall2010transverse,
	author       = {Dall, R. G. and Hodgman, S. S. and Johnsson, M. T. and Baldwin, K. G. H. and Truscott, A. G.},
	title        = {Transverse mode imaging of guided matter waves},
	journal      = {Physical Review A},
	year         = 2010,
	volume       = 81,
	number       = 1,
	pages        = {011602},
}
@article{damanet2019reservoir,
	author       = {Damanet, Fran{\c{c}}ois and Mascarenhas, Eduardo and Pekker, David and Daley, Andrew J},
	title        = {Reservoir engineering of Cooper-pair-assisted transport with cold atoms},
	journal      = {arXiv preprint arXiv:1908.02061},
	year         = 2019,
}
@article{damanet2019controlling,
	author       = {Damanet, Fran\ifmmode \mbox{\c{c}}\else \c{c}\fi{}ois and Mascarenhas, Eduardo and Pekker, David and Daley, Andrew J.},
	title        = {Controlling Quantum Transport via Dissipation Engineering},
	journal      = {Phys. Rev. Lett.},
	year         = 2019,
	volume       = 123,
	pages        = 180402,
	month        = {Oct},
}
@article{danshita2012quantum,
	author       = {Danshita, Ippei and Polkovnikov, Anatoli},
	title        = {Quantum phase slips in one-dimensional superfluids in a periodic potential},
	journal      = {Phys. Rev. A},
	year         = 2012,
	volume       = 85,
	pages        = {023638},
	month        = {Feb},
}
@article{david2008magnetic,
	author       = {David, T and Japha, Y and Dikovsky, V and Salem, R and Henkel, C and Folman, R},
	title        = {Magnetic interactions of cold atoms with anisotropic conductors},
	journal      = {The European Physical Journal D},
	year         = 2008,
	volume       = 48,
	number       = 3,
	pages        = {321--332},
}
@article{davis1999atomic,
	author       = {Davis, T J},
	title        = {Atomic de Broglie waveguides and integrated atom-optics using permanent magnets},
	journal      = {Journal of Optics B:},
	year         = 1999,
	volume       = 1,
	number       = 4,
	pages        = {408--414},
	month        = {Aug},
}
@article{Davis1999JOOB,
	author       = {Davis, T J},
	title        = {Atomic de Broglie waveguides and integrated atom-optics using permanent magnets},
	journal      = {Journal of Optics B:},
	year         = 1999,
	volume       = 1,
	number       = 4,
	pages        = {408--414},
	month        = {Aug},
}

@article{hafele1972around-the-world,
	Author = {Hafele, J. C. and Keating, Richard E.},
	Title = {Around-the-World Atomic Clocks: Observed Relativistic Time Gains},
	Journal = {Science},
	Year = {1972},
	Volume = {177},
	Number = {4044},
	Pages = {168-170},
	Month = {},
	URL = {http://www.sciencemag.org/content/177/4044/168.abstract},
	DOI = {10.1126/science.177.4044.168},
}


@article{amit2019stern-gerlach,
	Author = {O. Amit and Y. Margalit and O. Dobkowski and Z. Zhou and Y. Japha and M. Zimmermann and M.{\hspace{0.167em}}A. Efremov and F.{\hspace{0.167em}}A. Narducci and E.{\hspace{0.167em}}M. Rasel and W.{\hspace{0.167em}}P. Schleich and R. Folman},
	Title = {T3 Stern-Gerlach Matter-Wave Interferometer},
	Journal = {Physical Review Letters},
	Year = 2019,
	Volume = {123},
	Number = {8},
	Pages = {},
	Month = {aug},
	URL = {https://doi.org/10.1103/PhysRevLett.123.083601},
	DOI = {10.1103/PhysRevLett.123.083601},
}


@article{machluf2013coherent,
	Author = {Machluf, S. and Japha, Y. and Folman, R.},
	Title = {Coherent Stern-Gerlach momentum splitting on an atom chip},
	Journal = {Nature Communications},
	Year = {2013},
	Volume = {4},
	Number = {},
	Pages = {2424},
	Month = {Sep},
	URL = {},
	DOI = {10.1038/ncomms3424},
}


@article{deaver1961experimental,
	author       = {Deaver, Bascom S. and Fairbank, William M.},
	title        = {Experimental Evidence for Quantized Flux in Superconducting Cylinders},
	journal      = {Phys. Rev. Lett.},
	year         = 1961,
	volume       = 7,
	pages        = {43--46},
	month        = {Jul},
}
@article{deaver1991experimental,
	author       = {Deaver, Bascom S. and Fairbank, William M.},
	title        = {Experimental Evidence for Quantized Flux in Superconducting Cylinders},
	journal      = {Phys. Rev. Lett.},
	year         = 1961,
	volume       = 7,
	pages        = {43--46},
	month        = {Jul},
}
@article{burke2009scalable,
	Author = {Burke, J. H. T. and Sackett, C. A.},
	Title = {Scalable Bose-Einstein-condensate Sagnac interferometer in a linear trap},
	Journal = {Physical Review A},
	Year = {2009},
	Volume = {80},
	Number = {},
	Pages = {061603},
	Month = {Dec},
	URL = {http://link.aps.org/doi/10.1103/PhysRevA.80.061603},
	DOI = {10.1103/PhysRevA.80.061603},
}


@article{burke2008confinement,
	Author = {J. H. T. Burke and B. Deissler and K. J. Hughes and C. A. Sackett},
	Title = {Confinement effects in a guided-wave atom interferometer with millimeter-scale arm separation},
	Journal = {Physical Review A},
	Year = 2008,
	Volume = {78},
	Number = {2},
	Pages = {},
	Month = {aug},
	URL = {https://doi.org/10.1103/PhysRevA.78.023619},
	DOI = {10.1103/PhysRevA.78.023619},
}


@article{deissler2008measurement,
	author       = {Deissler, B and Hughes, KJ and Burke, JHT and Sackett, CA},
	title        = {Measurement of the ac Stark shift with a guided matter-wave interferometer},
	journal      = {Physical Review A},
	year         = 2008,
	volume       = 77,
	number       = 3,
	pages        = {031604},
	month        = {Mar},
}
@article{Deissler2008PRA,
	author       = {Deissler, B and Hughes, KJ and Burke, JHT and Sackett, CA},
	title        = {Measurement of the ac Stark shift with a guided matter-wave interferometer},
	journal      = {Physical Review A},
	year         = 2008,
	volume       = 77,
	number       = 3,
	pages        = {031604},
	month        = {Mar},
}
@article{Del-Pace:2021ti,
	author       = {Del Pace, G. and Kwon, W. J. and Zaccanti, M. and Roati, G. and Scazza, F.},
	title        = {Tunneling Transport of Unitary Fermions across the Superfluid Transition},
	journal      = {Phys. Rev. Lett.},
	year         = 2021,
	volume       = 126,
	pages        = {055301},
	month        = {Feb},
}
@article{del-pace2021tunneling,
	author       = {Del Pace, G. and Kwon, W. J. and Zaccanti, M. and Roati, G. and Scazza, F.},
	title        = {Tunneling Transport of Unitary Fermions across the Superfluid Transition},
	journal      = {Phys. Rev. Lett.},
	year         = 2021,
	volume       = 126,
	pages        = {055301},
	month        = {Feb},
}
@article{majorana1932atomi,
	author       = {Ettore Majorana},
	title        = {Atomi orientati in campo magnetico variabile},
	journal      = {Il Nuovo Cimento},
	year         = 1932,
	volume       = 9,
	pages        = {43--50},
}
@article{ettore-majorana1932atomi,
	author       = {di Ettore Majorana, Nota},
	title        = {Atomi orientati in campo magnetico variabile},
	journal      = {Il Nuovo Cimento},
	year         = 1932,
	volume       = 9,
	pages        = {43--50},
}
@article{dikovsky2005reduction,
	author       = {Dikovsky, V and Japha, Y and Henkel, Carsten and Folman, R},
	title        = {Reduction of magnetic noise in atom chips by material optimization},
	journal      = {The European Physical Journal D-Atomic, Molecular, Optical and Plasma Physics},
	year         = 2005,
	volume       = 35,
	number       = 1,
	pages        = {87--95},
}
@article{dikovsky2009superconducting,
	author       = {Dikovsky, Valery and Sokolovsky, Vladimir and Zhang, Bin and Henkel, Carsten and Folman, Ron},
	title        = {Superconducting atom chips: advantages and challenges},
	journal      = {The European Physical Journal D},
	year         = 2009,
	volume       = 51,
	number       = 2,
	pages        = {247--259},
}
@article{dowling2003quantum,
	author       = {Dowling, Jonathan P and Milburn, Gerard J},
	title        = {Quantum technology: the second quantum revolution},
	journal      = {Philosophical Transactions of the Royal Society of London A: Mathematical, Physical and Engineering Sciences},
	year         = 2003,
	volume       = 361,
	number       = 1809,
	pages        = {1655--1674},
}
@article{dubessy2012critical,
	author       = {Dubessy, R. and Liennard, T. and Pedri, P. and Perrin, H.},
	title        = {Critical rotation of an annular superfluid Bose-Einstein condensate},
	journal      = {Phys. Rev. A},
	year         = 2012,
	volume       = 86,
	pages        = {011602},
	month        = {Jul},
}
@article{dubessy2021universal,
	author       = {Dubessy, Romain and Polo, Juan and Perrin, H\'el\`ene and Minguzzi, Anna and Olshanii, Maxim},
	title        = {Universal shock-wave propagation in one-dimensional Bose fluids},
	journal      = {Phys. Rev. Research},
	year         = 2021,
	volume       = 3,
	pages        = {013098},
	month        = {Jan},
}
@article{dumke2002interferometer,
	author       = {Dumke, R. and M\"{u}ther, T. and Volk, M. and Ertmer, W. and Birkl, G.},
	title        = {Interferometer-Type Structures for Guided Atoms},
	journal      = {Physical Review Letters},
	year         = 2002,
	volume       = 89,
	number       = 22,
	pages        = 220402,
	month        = {Nov},
}
@article{dumke2002interferometer-type,
	author       = {Dumke, R. and M\"{u}ther, T. and Volk, M. and Ertmer, W. and Birkl, G.},
	title        = {Interferometer-Type Structures for Guided Atoms},
	journal      = {Physical Review Letters},
	year         = 2002,
	volume       = 89,
	number       = 22,
	pages        = 220402,
	month        = {Nov},
}
@article{dutta2015non,
	author       = {Dutta, Omjyoti and Gajda, Mariusz and Hauke, Philipp and Lewenstein, Maciej and L\"{u}hmann, Dirk-S\"{o}ren and Malomed, Boris A and Sowi\'{n}ski, Tomasz and Zakrzewski, Jakub},
	title        = {Non-standard Hubbard models in optical lattices: a review},
	journal      = {Reports on Progress in Physics},
	year         = 2015,
	volume       = 78,
	number       = 6,
	pages        = {066001},
}
@article{dutta2015non-standard,
	author       = {Dutta, Omjyoti and Gajda, Mariusz and Hauke, Philipp and Lewenstein, Maciej and L\"{u}hmann, Dirk-S\"{o}ren and Malomed, Boris A and Sowi\'{n}ski, Tomasz and Zakrzewski, Jakub},
	title        = {Non-standard Hubbard models in optical lattices: a review},
	journal      = {Reports on Progress in Physics},
	year         = 2015,
	volume       = 78,
	number       = 6,
	pages        = {066001},
}
@article{eckel2014interferometric,
	author       = {Eckel, S. and Jendrzejewski, F. and Kumar, A. and Lobb, C. J. and Campbell, G. K.},
	title        = {Interferometric Measurement of the Current-Phase Relationship of a Superfluid Weak Link},
	journal      = {Phys. Rev. X},
	year         = 2014,
	volume       = 4,
	number       = 3,
	pages        = {031052},
	month        = {Sep},
}
@article{eckel2018rapidly,
	author       = {Eckel, S. and Kumar, A. and Jacobson, T. and Spielman, I. B. and Campbell, G. K.},
	title        = {A Rapidly Expanding Bose-Einstein Condensate: An Expanding Universe in the Lab},
	journal      = {Phys. Rev. X},
	year         = 2018,
	volume       = 8,
	pages        = {021021},
	month        = {Apr},
}
@article{Eckel:2016aa,
	author       = {Eckel, S. and Lee, Jeffrey G. and Jendrzejewski, F. and Lobb, C. J. and Campbell, G. K. and Hill, W. T.},
	title        = {Contact resistance and phase slips in mesoscopic superfluid-atom transport},
	journal      = {Phys. Rev. A},
	year         = 2016,
	volume       = 93,
	pages        = {063619},
	month        = {Jun},
}
@article{eckel2016contact,
	author       = {Eckel, S. and Lee, Jeffrey G. and Jendrzejewski, F. and Lobb, C. J. and Campbell, G. K. and Hill, W. T.},
	title        = {Contact resistance and phase slips in mesoscopic superfluid-atom transport},
	journal      = {Phys. Rev. A},
	year         = 2016,
	volume       = 93,
	pages        = {063619},
	month        = {Jun},
}
@article{eckel2014hysteresis,
	author       = {Eckel, Stephen and Lee, Jeffrey G. and Jendrzejewski, Fred and Murray, Noel and Clark, Charles W. and Lobb, Christopher J. and Phillips, William D. and Edwards, Mark and Campbell, Gretchen K.},
	title        = {Hysteresis in a quantized superfluid {\textquoteleft}atomtronic{\textquoteright} circuit},
	journal      = {Nature},
	year         = 2014,
	volume       = 506,
	number       = 7487,
	pages        = {200{\textendash}203},
}
@book{essler2005one,
	title        = {The one-dimensional Hubbard model},
	publisher    = {Cambridge University Press},
	year         = 2005,
	author       = {Essler, Fabian HL and Frahm, Holger and G\"{o}hmann, Frank and Kl\"{u}mper, Andreas and Korepin, Vladimir E},
}
@book{essler2005the,
	title        = {The one-dimensional Hubbard model},
	publisher    = {Cambridge University Press},
	year         = 2005,
	author       = {Essler, Fabian HL and Frahm, Holger and G\"{o}hmann, Frank and Kl\"{u}mper, Andreas and Korepin, Vladimir E},
}
@article{fabre2011realization,
	author       = {Fabre, C. M. and Cheiney, P. and Gattobigio, G. L. and Vermersch, F. and Faure, S. and Mathevet, R. and Lahaye, T. and Gu\'{e}ry-Odelin, D.},
	title        = {Realization of a Distributed Bragg Reflector for Propagating Guided Matter Waves},
	journal      = {Physical Review Letters},
	year         = 2011,
	volume       = 107,
	number       = 23,
	pages        = 230401,
}
@book{faddeev2007hamiltonian,
	title        = {Hamiltonian methods in the theory of solitons},
	publisher    = {Springer Science \& Business Media},
	year         = 2007,
	author       = {Faddeev, Ludwig and Takhtajan, Leon},
}
@article{fazio2001quantum,
	author       = {Fazio, Rosario and Van Der Zant, Herre},
	title        = {Quantum phase transitions and vortex dynamics in superconducting networks},
	journal      = {Physics Reports},
	year         = 2001,
	volume       = 355,
	number       = 4,
	pages        = {235--334},
}
@article{fernholz2008fully,
	author       = {Fernholz, T. and Gerritsma, R. and Whitlock, S. and Barb, I. and Spreeuw, R. J. C.},
	title        = {Fully permanent magnet atom chip for Bose-Einstein condensation},
	journal      = {Physical Review A},
	year         = 2008,
	volume       = 77,
	number       = 3,
	month        = {Mar},
}
@article{Fernholz2008PRA,
	author       = {Fernholz, T. and Gerritsma, R. and Whitlock, S. and Barb, I. and Spreeuw, R. J. C.},
	title        = {Fully permanent magnet atom chip for Bose-Einstein condensation},
	journal      = {Physical Review A},
	year         = 2008,
	volume       = 77,
	number       = 3,
	month        = {Mar},
}
@article{Filippone:2016aa,
	author       = {Filippone, Michele and Hekking, Frank and Minguzzi, Anna},
	title        = {Violation of the Wiedemann-Franz law for one-dimensional ultracold atomic gases},
	journal      = {Phys. Rev. A},
	year         = 2016,
	volume       = 93,
	pages        = {011602},
	month        = {Jan},
}
@article{filippone2016violation,
	author       = {Filippone, Michele and Hekking, Frank and Minguzzi, Anna},
	title        = {Violation of the Wiedemann-Franz law for one-dimensional ultracold atomic gases},
	journal      = {Phys. Rev. A},
	year         = 2016,
	volume       = 93,
	pages        = {011602},
	month        = {Jan},
}
@article{fleischhauer2005electromagnetically,
	author       = {Fleischhauer, Michael and Imamoglu, Atac and Marangos, Jonathan P},
	title        = {Electromagnetically induced transparency: Optics in coherent media},
	journal      = {Reviews of modern physics},
	year         = 2005,
	volume       = 77,
	number       = 2,
	pages        = 633,
}
@article{Folman2000PRL,
	author       = {Folman, R. and Kruger, P. and Cassettari, D. and Hessmo, B. and Maier, T. and Schmiedmayer, J.},
	title        = {Controlling cold atoms using nanofabricated surfaces: Atom chips},
	journal      = {Phys. Rev. Lett.},
	year         = 2000,
	volume       = {84 20},
	pages        = {4749--4752},
	month        = 5,
}
@article{folman2000controlling,
	author       = {Folman, Ron and Kr\"{u}ger, Peter and Cassettari, Donatella and Hessmo, Bj\"{o}rn and Maier, Thomas and Schmiedmayer, J\"{o}rg},
	title        = {Controlling cold atoms using nanofabricated surfaces: atom chips},
	journal      = {Physical Review Letters},
	year         = 2000,
	volume       = 84,
	number       = 20,
	pages        = 4749,
	month        = 5,
}
@article{folman2008microscopic,
	author       = {Folman, Ron and Kruger, Peter and Schmiedmayer, J\"{o}rg and Denschlag, Johannes and Henkel, Carsten},
	title        = {Microscopic atom optics: from wires to an atom chip},
	journal      = {arXiv preprint arXiv:0805.2613},
	year         = 2008,
}
@article{fortagh2007magnetic,
	author       = {Fort\'{a}gh, J\'{o}zsef and Zimmermann, Claus},
	title        = {Magnetic microtraps for ultracold atoms},
	journal      = {Reviews of Modern Physics},
	year         = 2007,
	volume       = 79,
	number       = 1,
	pages        = {235--289},
	month        = feb,
}
@article{friedman2001observation,
	author       = {Friedman, Nir and Kaplan, Ariel and Carasso, Dina and Davidson, Nir},
	title        = {Observation of chaotic and regular dynamics in atom-optics billiards},
	journal      = {Physical Review Letters},
	year         = 2001,
	volume       = 86,
	number       = 8,
	pages        = {1518--1521},
}
@article{Frye2021EQT,
	author       = {Frye, Kai and Abend, Sven and Bartosch, Wolfgang and Bawamia, Ahmad and Becker, Dennis and Blume, Holger and Braxmaier, Claus and Chiow, Sheng-Wey and Efremov, Maxim A. and Ertmer, Wolfgang and Fierlinger, Peter and Franz, Tobias and Gaaloul, Naceur and Grosse, Jens and Grzeschik, Christoph and Hellmig, Ortwin and Henderson, Victoria A. and Herr, Waldemar and Israelsson, Ulf and Kohel, James and Krutzik, Markus and K\"{u}rbis, Christian and L\"{a}mmerzahl, Claus and List, Meike and L\"{u}dtke, Daniel and Lundblad, Nathan and Marburger, J. Pierre and Meister, Matthias and Mihm, Moritz and M\"{u}ller, Holger and M\"{u}ntinga, Hauke and Nepal, Ayush M. and Oberschulte, Tim and Papakonstantinou, Alexandros and Perovs\uek, Jaka and Peters, Achim and Prat, Arnau and Rasel, Ernst M. and Roura, Albert and Sbroscia, Matteo and Schleich, Wolfgang P. and Schubert, Christian and Seidel, Stephan T. and Sommer, Jan and Spindeldreier, Christian and Stamper-Kurn, Dan and Stuhl, Benjamin K. and Warner, Marvin and Wendrich, Thijs and Wenzlawski, Andr\'{e} and Wicht, Andreas and Windpassinger, Patrick and Yu, Nan and W\"{o}rner, Lisa},
	title        = {The Bose-Einstein Condensate and Cold Atom Laboratory},
	journal      = {EPJ Quantum Technology},
	year         = 2021,
	volume       = 8,
	number       = 1,
	pages        = 1,
}
@article{frye2021the,
	author       = {Frye, Kai and Abend, Sven and Bartosch, Wolfgang and Bawamia, Ahmad and Becker, Dennis and Blume, Holger and Braxmaier, Claus and Chiow, Sheng-Wey and Efremov, Maxim A. and Ertmer, Wolfgang and Fierlinger, Peter and Franz, Tobias and Gaaloul, Naceur and Grosse, Jens and Grzeschik, Christoph and Hellmig, Ortwin and Henderson, Victoria A. and Herr, Waldemar and Israelsson, Ulf and Kohel, James and Krutzik, Markus and K\"{u}rbis, Christian and L\"{a}mmerzahl, Claus and List, Meike and L\"{u}dtke, Daniel and Lundblad, Nathan and Marburger, J. Pierre and Meister, Matthias and Mihm, Moritz and M\"{u}ller, Holger and M\"{u}ntinga, Hauke and Nepal, Ayush M. and Oberschulte, Tim and Papakonstantinou, Alexandros and Perovs\uek, Jaka and Peters, Achim and Prat, Arnau and Rasel, Ernst M. and Roura, Albert and Sbroscia, Matteo and Schleich, Wolfgang P. and Schubert, Christian and Seidel, Stephan T. and Sommer, Jan and Spindeldreier, Christian and Stamper-Kurn, Dan and Stuhl, Benjamin K. and Warner, Marvin and Wendrich, Thijs and Wenzlawski, Andr\'{e} and Wicht, Andreas and Windpassinger, Patrick and Yu, Nan and W\"{o}rner, Lisa},
	title        = {The Bose-Einstein Condensate and Cold Atom Laboratory},
	journal      = {EPJ Quantum Technology},
	year         = 2021,
	volume       = 8,
	number       = 1,
	pages        = 1,
}
@article{Gallego-Marcos:2014aa,
	author       = {Gallego-Marcos, Fernando and Platero, Gloria and Nietner, Christian and Schaller, Gernot and Brandes, Tobias},
	title        = {Nonequilibrium relaxation transport of ultracold atoms},
	journal      = {Phys. Rev. A},
	year         = 2014,
	volume       = 90,
	pages        = {033614},
	month        = {Sep},
}

@article{gallemi2018interaction,
  title = {Interaction-enhanced flow of a polariton superfluid current in a ring},
  author = {Gallem\'{\i}, A. and Guilleumas, M. and Richard, M. and Minguzzi, A.},
  journal = {Phys. Rev. B},
  volume = {98},
  issue = {10},
  pages = {104502},
  numpages = {7},
  year = {2018},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.98.104502},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.98.104502}
}


@article{gallego-marcos2014nonequilibrium,
	author       = {Gallego-Marcos, Fernando and Platero, Gloria and Nietner, Christian and Schaller, Gernot and Brandes, Tobias},
	title        = {Nonequilibrium relaxation transport of ultracold atoms},
	journal      = {Phys. Rev. A},
	year         = 2014,
	volume       = 90,
	pages        = {033614},
	month        = {Sep},
}
@article{Garraway2016JOPB,
	author       = {Garraway, Barry M and Perrin, H\'{e}l\`{e}ne},
	title        = {Recent developments in trapping and manipulation of atoms with adiabatic potentials},
	journal      = {Journal of Physics B},
	year         = 2016,
	volume       = 49,
	number       = 17,
	pages        = 172001,
	month        = {Aug},
}
@article{garraway2016recent,
	author       = {Garraway, Barry M and Perrin, H\'{e}l\`{e}ne},
	title        = {Recent developments in trapping and manipulation of atoms with adiabatic potentials},
	journal      = {Journal of Physics B},
	year         = 2016,
	volume       = 49,
	number       = 17,
	pages        = 172001,
	month        = {Aug},
}
@article{Gati:2006aa,
	author       = {Gati, Rudolf and Hemmerling, B\"{o}rge and F\"{o}lling, Jonas and Albiez, Michael and Oberthaler, Markus K.},
	title        = {Noise Thermometry with Two Weakly Coupled Bose-Einstein Condensates},
	journal      = {Physical Review Letters},
	year         = 2006,
	volume       = 96,
	number       = 13,
	pages        = 130404,
}
@article{gati2006noise,
	author       = {Gati, Rudolf and Hemmerling, B\"{o}rge and F\"{o}lling, Jonas and Albiez, Michael and Oberthaler, Markus K.},
	title        = {Noise Thermometry with Two Weakly Coupled Bose-Einstein Condensates},
	journal      = {Physical Review Letters},
	year         = 2006,
	volume       = 96,
	number       = 13,
	pages        = 130404,
}
@article{gattobigio2012optically,
	author       = {Gattobigio, G. L. and Couvert, A. and Reinaudi, G. and Georgeot, B. and Gu\'{e}ry-Odelin, D.},
	title        = {Optically Guided Beam Splitter for Propagating Matter Waves},
	journal      = {Physical Review Letters},
	year         = 2012,
	volume       = 109,
	number       = 3,
	pages        = {030403},
}
@article{gaunt2012robust,
	author       = {Gaunt, Alexander L. and Hadzibabic, Zoran},
	title        = {Robust Digital Holography For Ultracold Atom Trapping},
	journal      = {Scientific Reports},
	year         = 2012,
	volume       = 2,
	pages        = 721,
	month        = 10,
}
@article{gauthier2016direct,
	author       = {Gauthier, G and Lenton, I and Parry, N McKay and Baker, M and Davis, MJ and Rubinsztein-Dunlop, H and Neely, TW},
	title        = {Direct imaging of a digital-micromirror device for configurable microscopic optical potentials},
	journal      = {Optica},
	year         = 2016,
	volume       = 3,
	number       = 10,
	pages        = {1136--1143},
	month        = {Oct},
}
@article{gauthier2021dynamic,
	author       = {Gauthier, Guillaume and Bell, Thomas A and Stilgoe, Alexander B and Baker, Mark and Rubinsztein-Dunlop, Halina and Neely, Tyler W},
	title        = {Dynamic high-resolution optical trapping of ultracold atoms},
	journal      = {arXiv preprint arXiv:2103.10020},
	year         = 2021,
}
@article{Gauthier:2019aa,
	author       = {Gauthier, Guillaume and Szigeti, Stuart S. and Reeves, Matthew T. and Baker, Mark and Bell, Thomas A. and Rubinsztein-Dunlop, Halina and Davis, Matthew J. and Neely, Tyler W.},
	title        = {Quantitative Acoustic Models for Superfluid Circuits},
	journal      = {Phys. Rev. Lett.},
	year         = 2019,
	volume       = 123,
	pages        = 260402,
	month        = {Dec},
}
@article{gauthier2019quantitative,
	author       = {Gauthier, Guillaume and Szigeti, Stuart S. and Reeves, Matthew T. and Baker, Mark and Bell, Thomas A. and Rubinsztein-Dunlop, Halina and Davis, Matthew J. and Neely, Tyler W.},
	title        = {Quantitative Acoustic Models for Superfluid Circuits},
	journal      = {Phys. Rev. Lett.},
	year         = 2019,
	volume       = 123,
	pages        = 260402,
	month        = {Dec},
}
@article{gefen1984quantum,
	author       = {Gefen, Yuval and Imry, Yoseph and Azbel, M Ya},
	title        = {Quantum oscillations and the Aharonov-Bohm effect for parallel resistors},
	journal      = {Phys. Rev. Lett.},
	year         = 1984,
	volume       = 52,
	number       = 2,
	pages        = 129,
}
@article{Gehr2010Cavity,
	author       = {Gehr, Roger and Volz, Juegen and Dubois, Guilhem and Steinmetz, Tilo and Colombe, Yves and Lev, Benjamin L. and Long, Romain and Esteve, Jerome and Reichel, Jakob},
	title        = {Cavity-Based Single Atom Preparation and High-Fidelity Hyperfine State Readout},
	journal      = {Phys. Rev. Lett.},
	year         = 2010,
	volume       = 104,
	number       = 20,
	pages        = 203602,
	month        = {May},
}
@article{gehr2010cavity-based,
	author       = {Gehr, Roger and Volz, Juegen and Dubois, Guilhem and Steinmetz, Tilo and Colombe, Yves and Lev, Benjamin L. and Long, Romain and Esteve, Jerome and Reichel, Jakob},
	title        = {Cavity-Based Single Atom Preparation and High-Fidelity Hyperfine State Readout},
	journal      = {Phys. Rev. Lett.},
	year         = 2010,
	volume       = 104,
	number       = 20,
	pages        = 203602,
	month        = {May},
}
@article{geiger2011detecting,
	author       = {Geiger, Remi and M\'{e}noret, Vincent and Stern, Guillaume and Zahzam, Nassim and Cheinet, Patrick and Battelier, Baptiste and Villing, Andr\'{e} and Moron, Fr\'{e}d\'{e}ric and Lours, Michel and Bidel, Yannick and others},
	title        = {Detecting inertial effects with airborne matter-wave interferometry},
	journal      = {Nature communications},
	year         = 2011,
	volume       = 2,
	number       = 1,
	pages        = {1--7},
}
@book{Giamarchi:2003aa,
	title        = {Quantum Physics in One Dimension},
	publisher    = {Clarendon Press},
	year         = 2003,
	author       = {Giamarchi, T.},
	series       = {International Series of Monographs on Physics},
}
@book{giamarchi2003quantum,
	title        = {Quantum Physics in One Dimension},
	publisher    = {Clarendon Press},
	year         = 2003,
	author       = {Giamarchi, T.},
	series       = {International Series of Monographs on Physics},
}
@article{Giovanazzi:2008aa,
	author       = {Giovanazzi, S and Esteve, J and Oberthaler, M K},
	title        = {Effective parameters for weakly coupled Bose--Einstein condensates},
	year         = 2008,
	volume       = 10,
	number       = 4,
	pages        = {045009},
}
@article{giovanazzi2008effective,
	author       = {Giovanazzi, S and Esteve, J and Oberthaler, M K},
	title        = {Effective parameters for weakly coupled Bose--Einstein condensates},
	year         = 2008,
	volume       = 10,
	number       = 4,
	pages        = {045009},
}
@article{goldman2014light-induced,
	author       = {Goldman, N and Juzeli{\={u}}nas, G and \"{O}hberg, P and Spielman, I B},
	title        = {Light-induced gauge fields for ultracold atoms},
	journal      = {Reports on Progress in Physics},
	year         = 2014,
	volume       = 77,
	number       = 12, 
	pages        = 126401,
	month        = {nov},
}
@article{Grenier:2014aa,
	author       = {Grenier, Ch. and Georges, A. and Kollath, C.},
	title        = {Peltier Cooling of Fermionic Quantum Gases},
	journal      = {Phys. Rev. Lett.},
	year         = 2014,
	volume       = 113,
	pages        = 200601,
	month        = {Nov},
}
@article{grenier2014peltier,
	author       = {Grenier, Ch. and Georges, A. and Kollath, C.},
	title        = {Peltier Cooling of Fermionic Quantum Gases},
	journal      = {Phys. Rev. Lett.},
	year         = 2014,
	volume       = 113,
	pages        = 200601,
	month        = {Nov},
}
@article{Grenier:aa,
	author       = {Grenier, Charles and Kollath, Corinna and Georges, Antoine},
	title        = {Thermoelectric transport and Peltier cooling of cold atomic gases},
	journal      = {Comptes Rendus Physique},
	year         = 2016,
	volume       = 17,
	pages        = {1161--1174},
}
@article{grenier2016thermoelectric,
	author       = {Grenier, Charles and Kollath, Corinna and Georges, Antoine},
	title        = {Thermoelectric transport and Peltier cooling of cold atomic gases},
	journal      = {Comptes Rendus Physique},
	year         = 2016,
	volume       = 17,
	pages        = {1161--1174},
}
@inbook{grimm2000optical,
	title        = {Optical Dipole Traps for Neutral Atoms},
	publisher    = {Academic Press},
	year         = 2000,
	editor       = {Bederson, Benjamin and Walther, Herbert},
	author       = {Grimm, Rudolf and Weidem\"{u}ller, Matthias and Ovchinnikov, Yurii B.},
	volume       = 42,
	type         = {Book Section},
	pages        = {95--170},
}
@article{Gring:2012aa,
	author       = {Gring, M. and Kuhnert, M. and Langen, T. and Kitagawa, T. and Rauer, B. and Schreitl, M. and Mazets, I. and Smith, D. Adu and Demler, E. and Schmiedmayer, J.},
	title        = {Relaxation and Prethermalization in an Isolated Quantum System},
	journal      = {Science},
	year         = 2012,
	volume       = 337,
	number       = 6100,
	pages        = {1318--1322},
}
@article{gring2012relaxation,
	author       = {Gring, M. and Kuhnert, M. and Langen, T. and Kitagawa, T. and Rauer, B. and Schreitl, M. and Mazets, I. and Smith, D. Adu and Demler, E. and Schmiedmayer, J.},
	title        = {Relaxation and Prethermalization in an Isolated Quantum System},
	journal      = {Science},
	year         = 2012,
	volume       = 337,
	number       = 6100,
	pages        = {1318--1322},
}
@article{guan2013fermi,
	author       = {Guan, Xi-Wen and Batchelor, Murray T and Lee, Chaohong},
	title        = {Fermi gases in one dimension: From Bethe ansatz to experiments},
	journal      = {Reviews of Modern Physics},
	year         = 2013,
	volume       = 85,
	number       = 4,
	pages        = 1633,
}
@article{Guerin:2006aa,
	author       = {Guerin, W. and Riou, J.-F. and Gaebler, J. P. and Josse, V. and Bouyer, P. and Aspect, A.},
	title        = {Guided Quasicontinuous Atom Laser},
	journal      = {Phys. Rev. Lett.},
	year         = 2006,
	volume       = 97,
	pages        = 200402,
	month        = {Nov},
}
@article{guerin2006guided,
	author       = {Guerin, W. and Riou, J.-F. and Gaebler, J. P. and Josse, V. and Bouyer, P. and Aspect, A.},
	title        = {Guided Quasicontinuous Atom Laser},
	journal      = {Phys. Rev. Lett.},
	year         = 2006,
	volume       = 97,
	pages        = 200402,
	month        = {Nov},
}
@article{guo2020supersonic,
	author       = {Guo, Yanliang and Dubessy, Romain and de Herve, Mathieu de Go\"er and Kumar, Avinash and Badr, Thomas and Perrin, Aur\'elien and Longchambon, Laurent and Perrin, H\'el\`ene},
	title        = {Supersonic Rotation of a Superfluid: A Long-Lived Dynamical Ring},
	journal      = {Phys. Rev. Lett.},
	year         = 2020,
	volume       = 124,
	number       = 2,
	pages        = {025301},
	month        = {Jan},
}
@article{gupta2005bose,
	author       = {Gupta, S and Murch, KW and Moore, KL and Purdy, TP and Stamper-Kurn, DM},
	title        = {Bose-Einstein condensation in a circular waveguide},
	journal      = {Phys. Rev. Lett.},
	year         = 2005,
	volume       = 95,
	number       = 14,
	pages        = 143201,
	month        = sep,
}
@article{gupta2005bose-einstein,
	author       = {Gupta, S and Murch, KW and Moore, KL and Purdy, TP and Stamper-Kurn, DM},
	title        = {Bose-Einstein condensation in a circular waveguide},
	journal      = {Phys. Rev. Lett.},
	year         = 2005,
	volume       = 95,
	number       = 14,
	pages        = 143201,
	month        = sep,
}
@article{Gutman:2012aa,
	author       = {Gutman, D. B. and Gefen, Yuval and Mirlin, A. D.},
	title        = {Cold bosons in the Landauer setup},
	journal      = {Phys. Rev. B},
	year         = 2012,
	volume       = 85,
	pages        = 125102,
	month        = {Mar},
}
@article{gutman2012cold,
	author       = {Gutman, D. B. and Gefen, Yuval and Mirlin, A. D.},
	title        = {Cold bosons in the Landauer setup},
	journal      = {Phys. Rev. B},
	year         = 2012,
	volume       = 85,
	pages        = 125102,
	month        = {Mar},
}
@article{gutzwiller1963effect,
	author       = {Gutzwiller, Martin C},
	title        = {Effect of correlation on the ferromagnetism of transition metals},
	journal      = {Phys. Rev. Lett.},
	year         = 1963,
	volume       = 10,
	number       = 5,
	pages        = 159,
}
@article{hansel2001bose,
	author       = {H\"{a}nsel, Wolfgang and Hommelhoff, Peter and H\"{a}nsch, TW and Reichel, Jakob},
	title        = {Bose--Einstein condensation on a microelectronic chip},
	journal      = {Nature},
	year         = 2001,
	volume       = 413,
	number       = 6855,
	pages        = {498--501},
}
@article{hansel2001bose--einstein,
	author       = {H\"{a}nsel, Wolfgang and Hommelhoff, Peter and H\"{a}nsch, TW and Reichel, Jakob},
	title        = {Bose--Einstein condensation on a microelectronic chip},
	journal      = {Nature},
	year         = 2001,
	volume       = 413,
	number       = 6855,
	pages        = {498--501},
}
@article{Hausler:2017ab,
	author       = {H\"ausler, Samuel and Nakajima, Shuta and Lebrat, Martin and Husmann, Dominik and Krinner, Sebastian and Esslinger, Tilman and Brantut, Jean-Philippe},
	title        = {Scanning Gate Microscope for Cold Atomic Gases},
	journal      = {Phys. Rev. Lett.},
	year         = 2017,
	volume       = 119,
	pages        = {030403},
	month        = {Jul},
}
@article{hausler2017scanning,
	author       = {H\"ausler, Samuel and Nakajima, Shuta and Lebrat, Martin and Husmann, Dominik and Krinner, Sebastian and Esslinger, Tilman and Brantut, Jean-Philippe},
	title        = {Scanning Gate Microscope for Cold Atomic Gases},
	journal      = {Phys. Rev. Lett.},
	year         = 2017,
	volume       = 119,
	pages        = {030403},
	month        = {Jul},
}
@article{Ha:2015vu,
	author       = {Ha, Li-Chung and Clark, Logan W. and Parker, Colin V. and Anderson, Brandon M. and Chin, Cheng},
	title        = {Roton-Maxon Excitation Spectrum of Bose Condensates in a Shaken Optical Lattice},
	journal      = {Phys. Rev. Lett.},
	year         = 2015,
	volume       = 114,
	pages        = {055301},
	month        = {Feb},
}
@article{ha2015roton-maxon,
	author       = {Ha, Li-Chung and Clark, Logan W. and Parker, Colin V. and Anderson, Brandon M. and Chin, Cheng},
	title        = {Roton-Maxon Excitation Spectrum of Bose Condensates in a Shaken Optical Lattice},
	journal      = {Phys. Rev. Lett.},
	year         = 2015,
	volume       = 114,
	pages        = {055301},
	month        = {Feb},
}
@article{haine2018quantum,
	author       = {Haine, Simon A},
	title        = {Quantum noise in bright soliton matterwave interferometry},
	journal      = {New Journal of Physics},
	year         = 2018,
	volume       = 20,
	number       = 3,
	pages        = {033009},
	month        = {mar},
}
@article{haldane1980solidification,
	author       = {Haldane, FDM},
	title        = {Solidification'' in a soluble model of bosons on a one-dimensional lattice: The ``Boson-Hubbard chain},
	journal      = {Physics Letters A},
	year         = 1980,
	volume       = 80,
	number       = 4,
	pages        = {281--283},
}
@article{hallwood_delta,
	author       = {Hallwood, D. W. and Burnett, K. and Dunningham, J.},
	title        = {The barriers to producing multiparticle superposition states in rotating Bose--Einstein condensates},
	journal      = {Journal of Modern Optics},
	year         = 2007,
	volume       = 54,
	number       = {13-15},
	pages        = {2129--2148},
}
@article{hallwood2007the,
	author       = {Hallwood, D. W. and Burnett, K. and Dunningham, J.},
	title        = {The barriers to producing multiparticle superposition states in rotating Bose--Einstein condensates},
	journal      = {Journal of Modern Optics},
	year         = 2007,
	volume       = 54,
	number       = {13-15},
	pages        = {2129--2148},
}
@article{hallwood2006macroscopic,
	author       = {Hallwood, David W and Burnett, Keith and Dunningham, Jacob},
	title        = {Macroscopic superpositions of superfluid flows},
	journal      = {New journal of Physics},
	year         = 2006,
	volume       = 8,
	number       = 9,
	pages        = 180,
}
@article{hallwood2010robust,
	author       = {Hallwood, David W and Ernst, Thomas and Brand, Joachim},
	title        = {Robust mesoscopic superposition of strongly correlated ultracold atoms},
	journal      = {Physical Review A},
	year         = 2010,
	volume       = 82,
	number       = 6,
	pages        = {063623},
}
@article{hammerer2010quantum,
	author       = {Hammerer, Klemens and S\o{}rensen, Anders S and Polzik, Eugene S},
	title        = {Quantum interface between light and atomic ensembles},
	journal      = {Reviews of Modern Physics},
	year         = 2010,
	volume       = 82,
	number       = 2,
	pages        = 1041,
}
@article{harber2005measurement,
	author       = {Harber, DM and Obrecht, JM and McGuirk, JM and Cornell, EA},
	title        = {Measurement of the Casimir-Polder force through center-of-mass oscillations of a Bose-Einstein condensate},
	journal      = {Physical Review A},
	year         = 2005,
	volume       = 72,
	number       = 3,
	pages        = 33610,
}
@article{Harber2005PRA,
	author       = {Harber, DM and Obrecht, JM and McGuirk, JM and Cornell, EA},
	title        = {Measurement of the Casimir-Polder force through center-of-mass oscillations of a Bose-Einstein condensate},
	journal      = {Physical Review A},
	year         = 2005,
	volume       = 72,
	number       = 3,
	pages        = 33610,
}
@book{hariharan2010basics,
	title        = {Basics of interferometry},
	publisher    = {Elsevier},
	year         = 2010,
	author       = {Hariharan, Parameswaran},
}
@book{Haroche:2006aa,
	title        = {Exploring the quantum: atoms, cavities, and photons},
	publisher    = {Oxford university press},
	year         = 2006,
	author       = {Haroche, Serge and Raimond, Jean-Marie},
}
@book{haroche2006exploring,
	title        = {Exploring the quantum: atoms, cavities, and photons},
	publisher    = {Oxford university press},
	year         = 2006,
	author       = {Haroche, Serge and Raimond, Jean-Marie},
}
@article{hattermann2017coupling,
	author       = {Hattermann, H and Bothner, D and Ley, LY and Ferdinand, B and Wiedmaier, D and S\'{a}rk\'{a}ny, L and Kleiner, Reinhold and Koelle, Dieter and Fort\'{a}gh, J},
	title        = {Coupling ultracold atoms to a superconducting coplanar waveguide resonator},
	journal      = {Nature communications},
	year         = 2017,
	volume       = 8,
	number       = 1,
	pages        = {1--7},
}
@article{haug2019topological,
	author       = {Haug, T and Amico, L and Kwek, L-C and Munro, WJ and Bastidas, VM},
	title        = {Topological pumping of quantum correlations},
	journal      = {Phys. Rev. Res.},
	year         = 2020,
	volume       = 2,
	number       = 1,
	pages        = {013135},
}
@article{haug2020topological,
	author       = {Haug, T and Amico, L and Kwek, L-C and Munro, WJ and Bastidas, VM},
	title        = {Topological pumping of quantum correlations},
	journal      = {Phys. Rev. Res.},
	year         = 2020,
	volume       = 2,
	number       = 1,
	pages        = {013135},
}
@article{haug2018mesoscopic,
	author       = {Haug, Tobias and Amico, Luigi and Dumke, Rainer and Kwek, Leong-Chuan},
	title        = {Mesoscopic Vortex--Meissner currents in ring ladders},
	journal      = {Quantum Science and Technology},
	year         = 2018,
	volume       = 3,
	number       = 3,
	pages        = {035006},
}
@article{haug2019andreev,
	author       = {Haug, Tobias and Dumke, Rainer and Kwek, Leong-Chuan and Amico, Luigi},
	title        = {Andreev-reflection and Aharonov--Bohm dynamics in atomtronic circuits},
	journal      = {Quantum Sci. Technol.},
	year         = 2019,
	volume       = 4,
	number       = 4,
	pages        = {045001},
}
@article{haug2019andreev-reflection,
	author       = {Haug, Tobias and Dumke, Rainer and Kwek, Leong-Chuan and Amico, Luigi},
	title        = {Andreev-reflection and Aharonov--Bohm dynamics in atomtronic circuits},
	journal      = {Quantum Sci. Technol.},
	year         = 2019,
	volume       = 4,
	number       = 4,
	pages        = {045001},
}
@article{haug2019engineering,
	author       = {Haug, Tobias and Dumke, Rainer and Kwek, Leong-Chuan and Miniatura, Christian and Amico, Luigi},
	title        = {Engineering quantum current states with machine learning},
	journal      = {arXiv:1911.09578},
	year         = 2019,
}
@article{haug2019aharonov,
	author       = {Haug, Tobias and Heimonen, Hermanni and Dumke, Rainer and Kwek, Leong-Chuan and Amico, Luigi},
	title        = {Aharonov-Bohm effect in mesoscopic Bose-Einstein condensates},
	journal      = {Physical Review A},
	year         = 2019,
	volume       = 100,
	number       = 4,
	pages        = {041601},
}
@article{haug2019aharonov-bohm,
	author       = {Haug, Tobias and Heimonen, Hermanni and Dumke, Rainer and Kwek, Leong-Chuan and Amico, Luigi},
	title        = {Aharonov-Bohm effect in mesoscopic Bose-Einstein condensates},
	journal      = {Physical Review A},
	year         = 2019,
	volume       = 100,
	number       = 4,
	pages        = {041601},
}
@article{haug2018readout,
	author       = {Haug, Tobias and Tan, Joel and Theng, Mark and Dumke, Rainer and Kwek, Leong-Chuan and Amico, Luigi},
	title        = {Readout of the atomtronic quantum interference device},
	journal      = {Phys. Rev. A},
	year         = 2018,
	volume       = 97,
	number       = 1,
	pages        = {013633},
}
@article{hekking1997quantum,
	author       = {Hekking, FWJ and Glazman, LI},
	title        = {Quantum fluctuations in the equilibrium state of a thin superconducting loop},
	journal      = {Physical Review B},
	year         = 1997,
	volume       = 55,
	number       = 10,
	pages        = 6551,
}
@article{helm2012bright,
	author       = {Helm, J. L. and Billam, T. P. and Gardiner, S. A.},
	title        = {Bright matter-wave soliton collisions at narrow barriers},
	journal      = {Phys. Rev. A},
	year         = 2012,
	volume       = 85,
	pages        = {053621},
	month        = {May},
}
@article{helm2015sagnac,
	author       = {Helm, JL and Cornish, SL and Gardiner, SA},
	title        = {Sagnac interferometry using bright matter-wave solitons},
	journal      = {Phys. Rev. Lett.},
	year         = 2015,
	volume       = 114,
	number       = 13,
	pages        = 134101,
	month        = {Apr},
}
@article{helm2014splitting,
	author       = {Helm, JL and Rooney, SJ and Weiss, Christoph and Gardiner, SA},
	title        = {Splitting bright matter-wave solitons on narrow potential barriers: Quantum to classical transition and applications to interferometry},
	journal      = {Physical Review A},
	year         = 2014,
	volume       = 89,
	number       = 3,
	pages        = {033610},
	month        = {Mar},
}
@article{henderson2009experimental,
	author       = {Henderson, K. and Ryu, C. and MacCormick, C. and Boshier, M. G.},
	title        = {Experimental demonstration of painting arbitrary and dynamic potentials for Bose-Einstein condensates},
	journal      = {New Journal of Physics},
	year         = 2009,
	volume       = 11,
	number       = 4,
	pages        = {043030},
	month        = {apr},
}
@article{hod2006inelastic,
	author       = {Hod, Oded and Baer, Roi and Rabani, Eran},
	title        = {Inelastic effects in Aharonov-Bohm molecular interferometers},
	journal      = {Phys. Rev. Lett.},
	year         = 2006,
	volume       = 97,
	number       = 26,
	pages        = 266803,
}
@article{Hofferberth:2007ab,
	author       = {Hofferberth, S. and Lesanovsky, I. and Fischer, B. and Schumm, T. and Schmiedmayer, J.},
	title        = {Non-equilibrium coherence dynamics in one-dimensional Bose gases},
	journal      = {Nature},
	year         = 2007,
	volume       = 449,
	number       = 7160,
	pages        = {324--327},
	month        = {09},
}
@article{hofferberth2007non-equilibrium,
	author       = {Hofferberth, S. and Lesanovsky, I. and Fischer, B. and Schumm, T. and Schmiedmayer, J.},
	title        = {Non-equilibrium coherence dynamics in one-dimensional Bose gases},
	journal      = {Nature},
	year         = 2007,
	volume       = 449,
	number       = 7160,
	pages        = {324--327},
	month        = {09},
}
@article{Hofferberth:2008aa,
	author       = {Hofferberth, S. and Lesanovsky, I. and Schumm, T. and Imambekov, A. and Gritsev, V. and Demler, E. and Schmiedmayer, J.},
	title        = {Probing quantum and thermal noise in an interacting many-body system},
	journal      = {Nature Physics},
	year         = 2008,
	volume       = 4,
	number       = 6,
	pages        = {489--495},
}
@article{hofferberth2008probing,
	author       = {Hofferberth, S. and Lesanovsky, I. and Schumm, T. and Imambekov, A. and Gritsev, V. and Demler, E. and Schmiedmayer, J.},
	title        = {Probing quantum and thermal noise in an interacting many-body system},
	journal      = {Nature Physics},
	year         = 2008,
	volume       = 4,
	number       = 6,
	pages        = {489--495},
}
@article{hopkins2004proposed,
	author       = {Hopkins, Asa and Lev, Benjamin and Mabuchi, Hideo},
	title        = {Proposed magnetoelectrostatic ring trap for neutral atoms},
	journal      = {Physical Review A},
	year         = 2004,
	volume       = 70,
	number       = 5,
	pages        = {053616},
}
@article{houde2000cold,
	author       = {Houde, Olivier and Kadio, Demascoth and Pruvost, Laurence},
	title        = {Cold Atom Beam Splitter Realized with Two Crossing Dipole Guides},
	journal      = {Physical Review Letters},
	year         = 2000,
	volume       = 85,
	number       = 26,
	pages        = {5543--5546},
}
@article{hubbard1963electron,
	author       = {Hubbard, John},
	title        = {Electron correlations in narrow energy bands},
	journal      = {Proceedings of the Royal Society of London. Series A. Mathematical and Physical Sciences},
	year         = 1963,
	volume       = 276,
	number       = 1365,
	pages        = {238--257},
}
@article{Hueck:2017tv,
	author       = {Hueck, Klaus and Mazurenko, Anton and Luick, Niclas and Lompe, Thomas and Moritz, Henning},
	title        = {Note: Suppression of kHz-frequency switching noise in digital micro-mirror devices},
	journal      = {Review of Scientific Instruments},
	year         = 2017,
	volume       = 88,
	number       = 1,
	pages        = {016103},
	month        = {2021/05/20},
}
@article{hueck2017note:,
	author       = {Hueck, Klaus and Mazurenko, Anton and Luick, Niclas and Lompe, Thomas and Moritz, Henning},
	title        = {Note: Suppression of kHz-frequency switching noise in digital micro-mirror devices},
	journal      = {Review of Scientific Instruments},
	year         = 2017,
	volume       = 88,
	number       = 1,
	pages        = {016103},
	month        = {2021/05/20},
}
@article{Husmann:2018aa,
	author       = {Husmann, Dominik and Lebrat, Martin and H\"{a}usler, Samuel and Brantut, Jean-Philippe and Corman, Laura and Esslinger, Tilman},
	title        = {Breakdown of the Wiedemann{\textendash}Franz law in a unitary Fermi gas},
	journal      = {Proceedings of the National Academy of Sciences},
	year         = 2018,
}
@article{husmann2018breakdown,
	author       = {Husmann, Dominik and Lebrat, Martin and H\"{a}usler, Samuel and Brantut, Jean-Philippe and Corman, Laura and Esslinger, Tilman},
	title        = {Breakdown of the Wiedemann{\textendash}Franz law in a unitary Fermi gas},
	journal      = {Proceedings of the National Academy of Sciences},
	year         = 2018,
}
@article{Husmann:2015aa,
	author       = {Husmann, Dominik and Uchino, Shun and Krinner, Sebastian and Lebrat, Martin and Giamarchi, Thierry and Esslinger, Tilman and Brantut, Jean-Philippe},
	title        = {Connecting strongly correlated superfluids by a quantum point contact},
	year         = 2015,
	month        = {08},
}
@article{husmann2015connecting,
	author       = {Husmann, Dominik and Uchino, Shun and Krinner, Sebastian and Lebrat, Martin and Giamarchi, Thierry and Esslinger, Tilman and Brantut, Jean-Philippe},
	title        = {Connecting strongly correlated superfluids by a quantum point contact},
	journal      = {Science},
	year         = 2015,
	volume       = 350,
	number       = 6267,
	pages        = {1498--1501},
}
@article{Imry:1999aa,
	author       = {Imry, Yoseph and Landauer, Rolf},
	title        = {Conductance viewed as transmission},
	journal      = {Rev. Mod. Phys.},
	year         = 1999,
	volume       = 71,
	pages        = {S306--S312},
	month        = {Mar},
}
@article{imry1999conductance,
	author       = {Imry, Yoseph and Landauer, Rolf},
	title        = {Conductance viewed as transmission},
	journal      = {Rev. Mod. Phys.},
	year         = 1999,
	volume       = 71,
	pages        = {S306--S312},
	month        = {Mar},
}
@book{Imry:2002aa,
	title        = {Introduction to mesoscopic physics},
	publisher    = {Oxford University Press},
	year         = 2002,
	author       = {Imry, Yoseph},
}
@book{imry2002introduction,
	title        = {Introduction to mesoscopic physics},
	publisher    = {Oxford University Press},
	year         = 2002,
	author       = {Imry, Yoseph},
}
@article{Ivanov:2013aa,
	author       = {Ivanov, Anton and Kordas, Georgios and Komnik, Andreas and Wimberger, Sandro},
	title        = {Bosonic transport through a chain of quantum dots},
	journal      = {The European Physical Journal B},
	year         = 2013,
	volume       = 86,
	number       = 8,
	pages        = 345,
}
@article{ivanov2013bosonic,
	author       = {Ivanov, Anton and Kordas, Georgios and Komnik, Andreas and Wimberger, Sandro},
	title        = {Bosonic transport through a chain of quantum dots},
	journal      = {The European Physical Journal B},
	year         = 2013,
	volume       = 86,
	number       = 8,
	pages        = 345,
}
@article{jordens2008mott,
	author       = {J\"{o}rdens, Robert and Strohmaier, Niels and G\"{u}nter, Kenneth and Moritz, Henning and Esslinger, Tilman},
	title        = {A Mott insulator of fermionic atoms in an optical lattice},
	journal      = {Nature},
	year         = 2008,
	volume       = 455,
	number       = 7210,
	pages        = {204--207},
}
@article{jagla1993electron,
	author       = {Jagla, EA and Balseiro, CA},
	title        = {Electron-electron correlations and the Aharonov-Bohm effect in mesoscopic rings},
	journal      = {Phys. Rev. Lett.},
	year         = 1993,
	volume       = 70,
	number       = 5,
	pages        = 639,
}
@article{jagla1993electron-electron,
	author       = {Jagla, EA and Balseiro, CA},
	title        = {Electron-electron correlations and the Aharonov-Bohm effect in mesoscopic rings},
	journal      = {Phys. Rev. Lett.},
	year         = 1993,
	volume       = 70,
	number       = 5,
	pages        = 639,
}
@article{jaksch1998cold,
	author       = {Jaksch, Dieter and Bruder, Ch and Cirac, Juan Ignacio and Gardiner, Crispin W and Zoller, Peter},
	title        = {Cold bosonic atoms in optical lattices},
	journal      = {Phys. Rev. Lett.},
	year         = 1998,
	volume       = 81,
	number       = 15,
	pages        = 3108,
}
@article{japha2007using,
	author       = {Japha, Y and Arzouan, O and Avishai, Y and Folman, R},
	title        = {Using time-reversal symmetry for sensitive incoherent matter-wave Sagnac interferometry},
	journal      = {Physical review letters},
	year         = 2007,
	volume       = 99,
	number       = 6,
	pages        = {060402},
}
@article{jaroszewicz2016review,
	author       = {Jaroszewicz, Leszek R and Kurzych, Anna and Krajewski, Zbigniew and Mar\'{c}, Pawe\l{} and Kowalski, Jerzy K and Bobra, Piotr and Zembaty, Zbigniew and Sakowicz, Bartosz and Jankowski, Robert},
	title        = {Review of the usefulness of various rotational seismometers with laboratory results of fibre-optic ones tested for engineering applications},
	journal      = {Sensors},
	year         = 2016,
	volume       = 16,
	number       = 12,
	pages        = 2161,
}
@article{Jendrzejewski:2014aa,
	author       = {Jendrzejewski, F. and Eckel, S. and Murray, N. and Lanier, C. and Edwards, M. and Lobb, C. J. and Campbell, G. K.},
	title        = {Resistive Flow in a Weakly Interacting Bose-Einstein Condensate},
	journal      = {Phys. Rev. Lett.},
	year         = 2014,
	volume       = 113,
	pages        = {045305},
	month        = {Jul},
}
@article{jendrzejewski2014resistive,
	author       = {Jendrzejewski, F. and Eckel, S. and Murray, N. and Lanier, C. and Edwards, M. and Lobb, C. J. and Campbell, G. K.},
	title        = {Resistive Flow in a Weakly Interacting Bose-Einstein Condensate},
	journal      = {Phys. Rev. Lett.},
	year         = 2014,
	volume       = 113,
	number       = 4,
	pages        = {045305},
	month        = {Jul},
}
@article{jones2004cold,
	author       = {Jones, M P A and Vale, C J and Sahagun, Daniel and Hall, B V and Eberlein, C C and Sauer, Ben and Furusawa, K and Richardson, D and Hinds, E A},
	title        = {Cold atoms probe the magnetic field near a wire},
	journal      = {Journal of Physics B},
	year         = 2004,
	volume       = 37,
	number       = 2,
	pages        = {L15},
}
@article{Jones2004JOPB,
	author       = {Jones, M P A and Vale, C J and Sahagun, Daniel and Hall, B V and Eberlein, C C and Sauer, Ben and Furusawa, K and Richardson, D and Hinds, E A},
	title        = {Cold atoms probe the magnetic field near a wire},
	journal      = {Journal of Physics B},
	year         = 2004,
	volume       = 37,
	number       = 2,
	pages        = {L15},
}
@article{Kanasz-Nagy:2016ab,
	author       = {Kan\'asz-Nagy, M. and Glazman, L. and Esslinger, T. and Demler, E. A.},
	title        = {Anomalous Conductances in an Ultracold Quantum Wire},
	journal      = {Phys. Rev. Lett.},
	year         = 2016,
	volume       = 117,
	pages        = 255302,
	month        = {Dec},
}
@article{kanasz-nagy2016anomalous,
	author       = {Kan\'asz-Nagy, M. and Glazman, L. and Esslinger, T. and Demler, E. A.},
	title        = {Anomalous Conductances in an Ultracold Quantum Wire},
	journal      = {Phys. Rev. Lett.},
	year         = 2016,
	volume       = 117,
	pages        = 255302,
	month        = {Dec},
}
@article{kanamori1963electron,
	author       = {Kanamori, Junjiro},
	title        = {Electron correlation and ferromagnetism of transition metals},
	journal      = {Progress of Theoretical Physics},
	year         = 1963,
	volume       = 30,
	number       = 3,
	pages        = {275--289},
}
@article{kasch2010cold,
	author       = {Kasch, B and Hattermann, H and Cano, D and Judd, TE and Scheel, S and Zimmermann, C and Kleiner, R and Koelle, D and Fort\'{a}gh, J},
	title        = {Cold atoms near superconductors: atomic spin coherence beyond the Johnson noise limit},
	journal      = {New Journal of Physics},
	year         = 2010,
	volume       = 12,
	number       = 6,
	pages        = {065024},
}
@article{keck2018persistent,
	author       = {Keck, Maximilian and Rossini, Davide and Fazio, Rosario},
	title        = {Persistent currents by reservoir engineering},
	journal      = {Physical Review A},
	year         = 2018,
	volume       = 98,
	number       = 5,
	pages        = {053812},
}
@article{keil2016fifteen,
	author       = {Keil, Mark and Amit, Omer and Zhou, Shuyu and Groswasser, David and Japha, Yonathan and Folman, Ron},
	title        = {Fifteen years of cold matter on the atom chip: promise, realizations, and prospects},
	journal      = {Journal of modern optics},
	year         = 2016,
	volume       = 63,
	number       = 18,
	pages        = {1840--1885},
}
@article{KHONDKER.1988,
	author       = {Khonker, A N and Khan, M R and Anwar, AFM},
	title        = {Transmission-Line Analogy of Resonance Tunneling Phenomena - the Generalized Impedance Concept},
	journal      = {Journal of Applied Physics},
	year         = 1988,
	volume       = 63,
	number       = 10,
	pages        = {5191 5193},
}
@article{khonker1988transmission-line,
	author       = {Khonker, A N and Khan, M R and Anwar, AFM},
	title        = {Transmission-Line Analogy of Resonance Tunneling Phenomena - the Generalized Impedance Concept},
	journal      = {Journal of Applied Physics},
	year         = 1988,
	volume       = 63,
	number       = 10,
	pages        = {5191 5193},
}
@article{kitching2011atomic,
	author       = {Kitching, John and Knappe, Svenja and Donley, Elizabeth A},
	title        = {Atomic sensors--a review},
	journal      = {IEEE Sensors Journal},
	year         = 2011,
	volume       = 11,
	number       = 9,
	pages        = {1749--1758},
}
@article{Kolovsky:2018aa,
	author       = {Kolovsky, Andrey R. and Denis, Zakari and Wimberger, Sandro},
	title        = {Landauer-B\"uttiker equation for bosonic carriers},
	journal      = {Phys. Rev. A},
	year         = 2018,
	volume       = 98,
	pages        = {043623},
	month        = {Oct},
}
@article{Kolovsky:2017ab,
	author = {Kolovsky, Andrey R.},
	journal = {Phys. Rev. A},
	month = {Jul},
	pages = {011601},
	title = {Microscopic models of source and sink for atomtronics},
	volume = {96},
	year = {2017}
}
@article{kolovsky2018landauer-buttiker,
	author       = {Kolovsky, Andrey R. and Denis, Zakari and Wimberger, Sandro},
	title        = {Landauer-B\"uttiker equation for bosonic carriers},
	journal      = {Phys. Rev. A},
	year         = 2018,
	volume       = 98,
	pages        = {043623},
	month        = {Oct},
}
@book{korepin1997quantum,
	title        = {Quantum inverse scattering method and correlation functions},
	publisher    = {Cambridge university press},
	year         = 1997,
	author       = {Korepin, Vladimir E and Bogoliubov, Nicholay M and Izergin, Anatoli G},
	volume       = 3,
}
@article{kovachy2015matter,
	author       = {Kovachy, Tim and Hogan, Jason M. and Sugarbaker, Alex and Dickerson, Susannah M. and Donnelly, Christine A. and Overstreet, Chris and Kasevich, Mark A.},
	title        = {Matter Wave Lensing to Picokelvin Temperatures},
	journal      = {Phys. Rev. Lett.},
	year         = 2015,
	volume       = 114,
	pages        = 143004,
	month        = {Apr},
}
@article{Kovachy2015PRL,
	author       = {Kovachy, Tim and Hogan, Jason M. and Sugarbaker, Alex and Dickerson, Susannah M. and Donnelly, Christine A. and Overstreet, Chris and Kasevich, Mark A.},
	title        = {Matter Wave Lensing to Picokelvin Temperatures},
	journal      = {Phys. Rev. Lett.},
	year         = 2015,
	volume       = 114,
	pages        = 143004,
	month        = {Apr},
}
@article{kraft2002anomalous,
	author       = {Kraft, S and G\"{u}nther, A and Ott, H and Wharam, D and Zimmermann, C and Fort\'{a}gh, J},
	title        = {Anomalous longitudinal magnetic field near the surface of copper conductors},
	journal      = {Journal of Physics B: Atomic, Molecular and Optical Physics},
	year         = 2002,
	volume       = 35,
	number       = 21,
	pages        = {L469},
}
@article{kreutzmann2004coherence,
	author       = {Kreutzmann, H. and Poulsen, U. V. and Lewenstein, M. and Dumke, R. and Ertmer, W. and Birkl, G. and Sanpera, A.},
	title        = {Coherence Properties of Guided-Atom Interferometers},
	journal      = {Phys. Rev. Lett.},
	year         = 2004,
	volume       = 92,
	number       = 16,
	month        = {Apr},
}
@article{Kreutzmann2004PRL,
	author       = {Kreutzmann, H. and Poulsen, U. V. and Lewenstein, M. and Dumke, R. and Ertmer, W. and Birkl, G. and Sanpera, A.},
	title        = {Coherence Properties of Guided-Atom Interferometers},
	journal      = {Phys. Rev. Lett.},
	year         = 2004,
	volume       = 92,
	number       = 16,
	month        = {Apr},
}
@article{Krinner:2017aa,
	author       = {Krinner, Sebastian and Esslinger, Tilman and Brantut, Jean-Philippe},
	title        = {Two-terminal transport measurements with cold atoms},
	journal      = {Journal of Physics: Condensed Matter},
	year         = 2017,
	volume       = 29,
	number       = 34,
	pages        = 343003,
}
@article{krinner2017two-terminal,
	author       = {Krinner, Sebastian and Esslinger, Tilman and Brantut, Jean-Philippe},
	title        = {Two-terminal transport measurements with cold atoms},
	journal      = {Journal of Physics: Condensed Matter},
	year         = 2017,
	volume       = 29,
	number       = 34,
	pages        = 343003,
}
@article{Krinner:2016ab,
	author       = {Krinner, Sebastian and Lebrat, Martin and Husmann, Dominik and Grenier, Charles and Brantut, Jean-Philippe and Esslinger, Tilman},
	title        = {Mapping out spin and particle conductances in a quantum point contact},
	journal      = {Proceedings of the National Academy of Sciences},
	year         = 2016,
	volume       = 113,
	number       = 29,
	pages        = {8144--8149},
	month        = {07},
}
@article{krinner2016mapping,
	author       = {Krinner, Sebastian and Lebrat, Martin and Husmann, Dominik and Grenier, Charles and Brantut, Jean-Philippe and Esslinger, Tilman},
	title        = {Mapping out spin and particle conductances in a quantum point contact},
	journal      = {Proc. Nat. Acad. Sci.},
	year         = 2016,
	volume       = 113,
	number       = 29,
	pages        = {8144--8149},
}
@article{Krinner:2015aa,
	author       = {Krinner, Sebastian and Stadler, David and Husmann, Dominik and Brantut, Jean-Philippe and Esslinger, Tilman},
	title        = {Observation of quantized conductance in neutral matter},
	journal      = {Nature},
	year         = 2015,
	volume       = 517,
	number       = 7532,
	pages        = {64--67},
	month        = {01},
}
@article{Krinner:2013aa,
	author       = {Krinner, Sebastian and Stadler, David and Meineke, Jakob and Brantut, Jean-Philippe and Esslinger, Tilman},
	title        = {Superfluidity with disorder in a thin film of quantum gas},
	journal      = {Phys. Rev. Lett.},
	year         = 2013,
	volume       = 110,
	pages        = 100601,
	month        = {Mar},
}
@article{krinner2013superfluidity,
	author       = {Krinner, Sebastian and Stadler, David and Meineke, Jakob and Brantut, Jean-Philippe and Esslinger, Tilman},
	title        = {Superfluidity with disorder in a thin film of quantum gas},
	journal      = {Phys. Rev. Lett.},
	year         = 2013,
	volume       = 110,
	pages        = 100601,
	month        = {Mar},
}
@article{Krinner:2015ac,
	author       = {Krinner, Sebastian and Stadler, David and Meineke, Jakob and Brantut, Jean-Philippe and Esslinger, Tilman},
	title        = {Observation of a Fragmented, Strongly Interacting Fermi Gas},
	journal      = {Phys. Rev. Lett.},
	year         = 2015,
	volume       = 115,
	pages        = {045302},
	month        = {Jul},
}
@article{krinner2015observation,
	author       = {Krinner, Sebastian and Stadler, David and Meineke, Jakob and Brantut, Jean-Philippe and Esslinger, Tilman},
	title        = {Observation of a Fragmented, Strongly Interacting Fermi Gas},
	journal      = {Phys. Rev. Lett.},
	year         = 2015,
	volume       = 115,
	pages        = {045302},
	month        = {Jul},
}
@article{kuga1997novel,
	author       = {Kuga, Takahiro and Torii, Yoshio and Shiokawa, Noritsugu and Hirano, Takuya and Shimizu, Yukiko and Sasada, Hiroyuki},
	title        = {Novel Optical Trap of Atoms with a Doughnut Beam},
	journal      = {Physical Review Letters},
	year         = 1997,
	volume       = 78,
	number       = 25,
	pages        = {4713--4716},
}
@article{kumar2017temperature,
	author       = {Kumar, A. and Eckel, S. and Jendrzejewski, F. and Campbell, G. K.},
	title        = {Temperature-induced decay of persistent currents in a superfluid ultracold gas},
	journal      = {Phys. Rev. A},
	year         = 2017,
	volume       = 95,
	number       = 2,
	pages        = {021602},
	month        = {Feb},
}
@article{kumar2017temperature-induced,
	author       = {Kumar, A. and Eckel, S. and Jendrzejewski, F. and Campbell, G. K.},
	title        = {Temperature-induced decay of persistent currents in a superfluid ultracold gas},
	journal      = {Phys. Rev. A},
	year         = 2017,
	volume       = 95,
	number       = 2,
	pages        = {021602},
	month        = {Feb},
}
@article{kunimi2017thermally,
	author       = {Kunimi, Masaya and Danshita, Ippei},
	title        = {Thermally activated phase slips of one-dimensional Bose gases in shallow optical lattices},
	journal      = {Phys. Rev. A},
	year         = 2017,
	volume       = 95,
	pages        = {033637},
	month        = {Mar},
}
@article{Kwon:2020aa,
	author       = {Kwon, W. J. and Del Pace, G. and Panza, R. and Inguscio, M. and Zwerger, W. and Zaccanti, M. and Scazza, F. and Roati, G.},
	title        = {Strongly correlated superfluid order parameters from dc Josephson supercurrents},
	journal      = {Science},
	year         = 2020,
	volume       = 369,
	number       = 6499,
	pages        = 84,
	month        = {07},
}
@article{kwon2020strongly,
	author       = {Kwon, W. J. and Del Pace, G. and Panza, R. and Inguscio, M. and Zwerger, W. and Zaccanti, M. and Scazza, F. and Roati, G.},
	title        = {Strongly correlated superfluid order parameters from dc Josephson supercurrents},
	journal      = {Science},
	year         = 2020,
	volume       = 369,
	number       = 6499,
	pages        = 84,
	month        = {07},
}
@article{levy1990magnetization,
	author       = {L\'evy, L. P. and Dolan, G. and Dunsmuir, J. and Bouchiat, H.},
	title        = {Magnetization of mesoscopic copper rings: Evidence for persistent currents},
	journal      = {Phys. Rev. Lett.},
	year         = 1990,
	volume       = 64,
	pages        = {2074--2077},
	month        = {Apr},
}
@article{Labouvie:2015aa,
	author       = {Labouvie, Ralf and Santra, Bodhaditya and Heun, Simon and Wimberger, Sandro and Ott, Herwig},
	title        = {Negative Differential Conductivity in an Interacting Quantum Gas},
	journal      = {Phys. Rev. Lett.},
	year         = 2015,
	volume       = 115,
	pages        = {050601},
	month        = {Jul},
}
@article{labouvie2015negative,
	author       = {Labouvie, Ralf and Santra, Bodhaditya and Heun, Simon and Wimberger, Sandro and Ott, Herwig},
	title        = {Negative Differential Conductivity in an Interacting Quantum Gas},
	journal      = {Phys. Rev. Lett.},
	year         = 2015,
	volume       = 115,
	pages        = {050601},
	month        = {Jul},
}
@article{lamata2014epj,
	author       = {Lamata, Lucas and Mezzacapo, Antonio and Casanova, Jorge and Solano, Enrique and Johnson, Tomi H and Clark, Stephen R and Jaksch, Dieter and Krutitsky, Konstantin V and Navez, Patrick and Queisser, Friedemann and others},
	title        = {EPJ Quantum Technology},
	journal      = {Quantum},
	year         = 2014,
	volume       = 1,
	number       = 1,
}
@article{Langen:2015ab,
	author       = {Langen, Tim and Geiger, Remi and Schmiedmayer, J\"{o}rg},
	title        = {Ultracold Atoms Out of Equilibrium},
	journal      = {Annual Review of Condensed Matter Physics},
	year         = 2015,
	volume       = 6,
	number       = 1,
	pages        = {201--217},
	month        = {2020/09/14},
}
@article{langen2015ultracold,
	author       = {Langen, Tim and Geiger, Remi and Schmiedmayer, J\"{o}rg},
	title        = {Ultracold Atoms Out of Equilibrium},
	journal      = {Annual Review of Condensed Matter Physics},
	year         = 2015,
	volume       = 6,
	number       = 1,
	pages        = {201--217},
	month        = {2020/09/14},
}
@article{leanhardt2002propagation,
	author       = {Leanhardt, AE and Chikkatur, AP and Kielpinski, D and Shin, Y and Gustavson, TL and Ketterle, W and Pritchard, DE},
	title        = {Propagation of Bose-Einstein condensates in a magnetic waveguide},
	journal      = {Phys. Rev. Lett.},
	year         = 2002,
	volume       = 89,
	number       = 4,
	pages        = {040401},
}
@article{LeBlanc:2011aa,
	author       = {LeBlanc, L. J. and Bardon, A. B. and McKeever, J. and Extavour, M. H. T. and Jervis, D. and Thywissen, J. H. and Piazza, F. and Smerzi, A.},
	title        = {Dynamics of a Tunable Superfluid Junction},
	journal      = {Phys. Rev. Lett.},
	year         = 2011,
	volume       = 106,
	pages        = {025302},
	month        = {Jan},
}
@article{leblanc2011dynamics,
	author       = {LeBlanc, L. J. and Bardon, A. B. and McKeever, J. and Extavour, M. H. T. and Jervis, D. and Thywissen, J. H. and Piazza, F. and Smerzi, A.},
	title        = {Dynamics of a Tunable Superfluid Junction},
	journal      = {Phys. Rev. Lett.},
	year         = 2011,
	volume       = 106,
	pages        = {025302},
	month        = {Jan},
}
@article{Lebrat:2018aa,
	author       = {Lebrat, Martin and Gri\ifmmode \check{s}\else \v{s}\fi{}ins, Pjotrs and Husmann, Dominik and H\"ausler, Samuel and Corman, Laura and Giamarchi, Thierry and Brantut, Jean-Philippe and Esslinger, Tilman},
	title        = {Band and Correlated Insulators of Cold Fermions in a Mesoscopic Lattice},
	journal      = {Phys. Rev. X},
	year         = 2018,
	volume       = 8,
	pages        = {011053},
	month        = {Mar},
}
@article{lebrat2018band,
	author       = {Lebrat, Martin and Gri\ifmmode \check{s}\else \v{s}\fi{}ins, Pjotrs and Husmann, Dominik and H\"ausler, Samuel and Corman, Laura and Giamarchi, Thierry and Brantut, Jean-Philippe and Esslinger, Tilman},
	title        = {Band and Correlated Insulators of Cold Fermions in a Mesoscopic Lattice},
	journal      = {Phys. Rev. X},
	year         = 2018,
	volume       = 8,
	pages        = {011053},
	month        = {Mar},
}
@article{Lebrat:2019aa,
	author       = {Lebrat, Martin and H\"ausler, Samuel and Fabritius, Philipp and Husmann, Dominik and Corman, Laura and Esslinger, Tilman},
	title        = {Quantized Conductance through a Spin-Selective Atomic Point Contact},
	journal      = {Phys. Rev. Lett.},
	year         = 2019,
	volume       = 123,
	pages        = 193605,
	month        = {Nov},
}
@article{lebrat2019quantized,
	author       = {Lebrat, Martin and H\"ausler, Samuel and Fabritius, Philipp and Husmann, Dominik and Corman, Laura and Esslinger, Tilman},
	title        = {Quantized Conductance through a Spin-Selective Atomic Point Contact},
	journal      = {Phys. Rev. Lett.},
	year         = 2019,
	volume       = 123,
	pages        = 193605,
	month        = {Nov},
}
@article{lee1957eigenvalues,
	author       = {Lee, T. D. and Huang, Kerson and Yang, C. N.},
	title        = {Eigenvalues and Eigenfunctions of a Bose System of Hard Spheres and Its Low-Temperature Properties},
	journal      = {Phys. Rev.},
	year         = 1957,
	volume       = 106,
	pages        = {1135--1145},
	month        = {Jun},
}
@article{leggett1991granular,
	author       = {Leggett, AJ},
	title        = {Granular Nanoelectronics},
	journal      = {NATO ASI Ser. B, 251Plenum, New York},
	year         = 1991,
	pages        = 297,
}
@book{leggett2006quantum,
	title        = {Quantum Fluids},
	publisher    = {Oxford University Press Oxford},
	year         = 2006,
	author       = {Leggett, AJ},
}
@article{leggett1980macroscopic,
	author       = {Leggett, Anthony J},
	title        = {Macroscopic quantum systems and the quantum theory of measurement},
	journal      = {Progr. Theoret. Phys. Suppl.},
	year         = 1980,
	volume       = 69,
	pages        = {80--100},
}
@article{Lesanovsky2007PRL,
	author       = {Lesanovsky, Igor and von Klitzing, Wolf},
	title        = {Time-Averaged Adiabatic Potentials: Versatile Matter-Wave Guides and Atom Traps},
	journal      = {Phys. Rev. Lett.},
	year         = 2007,
	volume       = 99,
	number       = 8,
	pages        = {083001},
}
@article{lesanovsky2007time,
	author       = {Lesanovsky, Igor and von Klitzing, Wolf},
	title        = {Time-Averaged Adiabatic Potentials: Versatile Matter-Wave Guides and Atom Traps},
	journal      = {Phys. Rev. Lett.},
	year         = 2007,
	volume       = 99,
	number       = 8,
	pages        = {083001},
	month        = {Aug},
}
@article{lesanovsky2007time-averaged,
	author       = {Lesanovsky, Igor and von Klitzing, Wolf},
	title        = {Time-Averaged Adiabatic Potentials: Versatile Matter-Wave Guides and Atom Traps},
	journal      = {Phys. Rev. Lett.},
	year         = 2007,
	volume       = 99,
	number       = 8,
	pages        = {083001},
	month        = {Aug},
}
@article{Levy:2007fk,
	author       = {Levy, S. and Lahoud, E. and Shomroni, I. and Steinhauer, J.},
	title        = {The a.c. and d.c. Josephson effects in a Bose-Einstein condensate},
	journal      = {Nature},
	year         = 2007,
	volume       = 449,
	number       = 7162,
	pages        = {579--583},
	month        = 10,
}
@article{levy2007the,
	author       = {Levy, S. and Lahoud, E. and Shomroni, I. and Steinhauer, J.},
	title        = {The a.c. and d.c. Josephson effects in a Bose-Einstein condensate},
	journal      = {Nature},
	year         = 2007,
	volume       = 449,
	number       = 7162,
	pages        = {579--583},
	month        = 10,
}
@article{lieb1963exact,
	author       = {Lieb, Elliott H and Liniger, Werner},
	title        = {Exact analysis of an interacting Bose gas. I. The general solution and the ground state},
	journal      = {Physical Review},
	year         = 1963,
	volume       = 130,
	number       = 4,
	pages        = 1605,
}
@article{LiebLiniger,
	author       = {Lieb, Elliott H and Liniger, Werner},
	title        = {Exact analysis of an interacting Bose gas. I. The general solution and the ground state},
	journal      = {Physical Review},
	year         = 1963,
	volume       = 130,
	number       = 4,
	pages        = 1605,
}
@article{lieb1968absence,
	author       = {Lieb, Elliott H and Wu, FY},
	title        = {Absence of Mott Transition in an Exact Solution of the Short-Range, One-Band Model in One Dimension},
	journal      = {Phys. Rev. Lett.},
	year         = 1968,
	volume       = 21,
	number       = 3,
	pages        = 192,
}
@article{Liu:2017aa,
	author       = {Liu, Boyang and Zhai, Hui and Zhang, Shizhong},
	title        = {Anomalous conductance of a strongly interacting Fermi gas through a quantum point contact},
	journal      = {Phys. Rev. A},
	year         = 2017,
	volume       = 95,
	pages        = {013623},
	month        = {Jan},
}
@article{liu2017anomalous,
	author       = {Liu, Boyang and Zhai, Hui and Zhang, Shizhong},
	title        = {Anomalous conductance of a strongly interacting Fermi gas through a quantum point contact},
	journal      = {Phys. Rev. A},
	year         = 2017,
	volume       = 95,
	pages        = {013623},
	month        = {Jan},
}
@article{lobos2008effects,
	author       = {Lobos, AM and Aligia, AA},
	title        = {Effects of interactions in transport through Aharonov-Bohm-Casher interferometers},
	journal      = {Phys. Rev. Lett.},
	year         = 2008,
	volume       = 100,
	number       = 1,
	pages        = {016803},
}
@article{Long2005EPJD,
	author       = {Long, R. and Rom, T. and Hansel, W. and Hansch, T. W. and Reichel, J.},
	title        = {Long distance magnetic conveyor for precise positioning of ultracold atoms},
	journal      = {European Physical Journal D},
	year         = 2005,
	volume       = 35,
	pages        = {125--133},
	month        = 8,
}
@article{long2005long,
	author       = {Long, R. and Rom, T. and Hansel, W. and Hansch, T. W. and Reichel, J.},
	title        = {Long distance magnetic conveyor for precise positioning of ultracold atoms},
	journal      = {European Physical Journal D},
	year         = 2005,
	volume       = 35,
	pages        = {125--133},
	month        = 8,
}
@article{loss1992parity,
	author       = {Loss, Daniel},
	title        = {Parity effects in a Luttinger liquid: Diamagnetic and paramagnetic ground states},
	journal      = {Phys. Rev. Lett.},
	year         = 1992,
	volume       = 69,
	number       = 2,
	pages        = 343,
}

@article{lukoshkin2018persistent,
  title = {Persistent circular currents of exciton-polaritons in cylindrical pillar microcavities},
  author = {Lukoshkin, V. A. and Kalevich, V. K. and Afanasiev, M. M. and Kavokin, K. V. and Hatzopoulos, Z. and Savvidis, P. G. and Sedov, E. S. and Kavokin, A. V.},
  journal = {Phys. Rev. B},
  volume = {97},
  issue = {19},
  pages = {195149},
  numpages = {6},
  year = {2018},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.97.195149},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.97.195149}
}

@article{Lui.1986,
	author       = {Lui, Wayne W and Fukuma, Masao},
	title        = {Exact solution of the Schrodinger equation across an arbitrary one-dimensional piecewise-linear potential barrier},
	journal      = {Journal of Applied Physics},
	year         = 1986,
	volume       = 60,
	number       = 5,
	pages        = {1555--1559},
}
@article{lui1986exact,
	author       = {Lui, Wayne W and Fukuma, Masao},
	title        = {Exact solution of the Schrodinger equation across an arbitrary one-dimensional piecewise-linear potential barrier},
	journal      = {Journal of Applied Physics},
	year         = 1986,
	volume       = 60,
	number       = 5,
	pages        = {1555--1559},
}
@article{Luick:2020aa,
	author       = {Luick, Niclas and Sobirey, Lennart and Bohlen, Markus and Singh, Vijay Pal and Mathey, Ludwig and Lompe, Thomas and Moritz, Henning},
	title        = {An ideal Josephson junction in an ultracold two-dimensional Fermi gas},
	journal      = {Science},
	year         = 2020,
	volume       = 369,
	number       = 6499,
	pages        = 89,
	month        = {07},
}
@article{luick2020ideal,
	author       = {Luick, Niclas and Sobirey, Lennart and Bohlen, Markus and Singh, Vijay Pal and Mathey, Ludwig and Lompe, Thomas and Moritz, Henning},
	title        = {An ideal Josephson junction in an ultracold two-dimensional Fermi gas},
	journal      = {Science},
	year         = 2020,
	volume       = 369,
	number       = 6499,
	pages        = 89,
	month        = {07},
}
@article{muller2000guiding,
	author       = {M\"{u}ller, Dirk and Cornell, Eric A. and Anderson, Dana Z. and Abraham, Eric R. I.},
	title        = {Guiding laser-cooled atoms in hollow-core fibers},
	journal      = {Physical Review A},
	year         = 2000,
	volume       = 61,
	number       = 3,
	pages        = {033411},
}
@article{muller2008atom,
	author       = {M\"{u}ller, Holger and Chiow, Sheng-wey and Long, Quan and Herrmann, Sven and Chu, Steven},
	title        = {Atom interferometry with up to 24-photon-momentum-transfer beam splitters},
	journal      = {Phys. Rev. lett},
	year         = 2008,
	volume       = 100,
	number       = 18,
	pages        = 180405,
}
@article{muller2010programmable,
	author       = {M\"{u}ller, T and Zhang, B and Fermani, R and Chan, KS and Lim, MJ and Dumke, R},
	title        = {Programmable trap geometries with superconducting atom chips},
	journal      = {Physical Review A},
	year         = 2010,
	volume       = 81,
	number       = 5,
	pages        = {053624},
	month        = {May},
}
@article{muller2010trapping,
	author       = {M\"{u}ller, T and Zhang, B and Fermani, R and Chan, KS and Wang, ZW and Zhang, CB and Lim, MJ and Dumke, R},
	title        = {Trapping of ultra-cold atoms with the magnetic field of vortices in a thin-film superconducting micro-structure},
	journal      = {New Journal of Physics},
	year         = 2010,
	volume       = 12,
	number       = 4,
	pages        = {043016},
	month        = {apr},
}
@article{Mullers:2018aa,
	author       = {M\"{u}llers, Andreas and Santra, Bodhaditya and Baals, Christian and Jiang, Jian and Benary, Jens and Labouvie, Ralf and Zezyulin, Dmitry A. and Konotop, Vladimir V. and Ott, Herwig},
	title        = {Coherent perfect absorption of nonlinear matter waves},
	journal      = {Science Advances},
	year         = 2018,
	volume       = 4,
	number       = 8,
	pages        = {eaat6539},
	month        = {08},
}
@article{mullers2018coherent,
	author       = {M\"{u}llers, Andreas and Santra, Bodhaditya and Baals, Christian and Jiang, Jian and Benary, Jens and Labouvie, Ralf and Zezyulin, Dmitry A. and Konotop, Vladimir V. and Ott, Herwig},
	title        = {Coherent perfect absorption of nonlinear matter waves},
	journal      = {Science Advances},
	year         = 2018,
	volume       = 4,
	number       = 8,
	pages        = {eaat6539},
	month        = {08},
}
@book{mahan2013many,
	title        = {Many-particle physics},
	publisher    = {Springer Science \& Business Media},
	year         = 2013,
	author       = {Mahan, Gerald D},
}
@book{mahan2013many-particle,
	title        = {Many-particle physics},
	publisher    = {Springer Science \& Business Media},
	year         = 2013,
	author       = {Mahan, Gerald D},
}
@article{manmana2011magnetism,
	author       = {Manmana, Salvatore R and Hazzard, Kaden RA and Chen, Gang and Feiguin, Adrian E and Rey, Ana Maria},
	title        = {SU (N) magnetism in chains of ultracold alkaline-earth-metal atoms: Mott transitions and quantum correlations},
	journal      = {Physical Review A},
	year         = 2011,
	volume       = 84,
	number       = 4,
	pages        = {043601},
}
@article{manmana2011n,
	author       = {Manmana, Salvatore R and Hazzard, Kaden RA and Chen, Gang and Feiguin, Adrian E and Rey, Ana Maria},
	title        = {SU (N) magnetism in chains of ultracold alkaline-earth-metal atoms: Mott transitions and quantum correlations},
	journal      = {Physical Review A},
	year         = 2011,
	volume       = 84,
	number       = 4,
	pages        = {043601},
}
@misc{2018_marchukov_preprint,
	title        = {A model of splitting an NLS breather by an emerging localized linear or nonlinear potential},
	author       = {Marchukov, Olexandr and Olshanii, Maxim and Malomed, Boris},
	year         = 2018,
}
@misc{marchukov2018model,
	title        = {A model of splitting an NLS breather by an emerging localized linear or nonlinear potential},
	author       = {Marchukov, Olexandr and Olshanii, Maxim and Malomed, Boris},
	year         = 2018,
}
@article{Marino:1999aa,
	author       = {Marino, I. and Raghavan, S. and Fantoni, S. and Shenoy, S. R. and Smerzi, A.},
	title        = {Bose-condensate tunneling dynamics: Momentum-shortened pendulum with damping},
	journal      = {Phys. Rev. A},
	year         = 1999,
	volume       = 60,
	pages        = {487--493},
	month        = {Jul},
}
@article{marino1999bose-condensate,
	author       = {Marino, I. and Raghavan, S. and Fantoni, S. and Shenoy, S. R. and Smerzi, A.},
	title        = {Bose-condensate tunneling dynamics: Momentum-shortened pendulum with damping},
	journal      = {Phys. Rev. A},
	year         = 1999,
	volume       = 60,
	pages        = {487--493},
	month        = {Jul},
}
@article{marquardt2002aharonov,
	author       = {Marquardt, Florian and Bruder, C},
	title        = {Aharonov-Bohm ring with fluctuating flux},
	journal      = {Phys. Rev. B},
	year         = 2002,
	volume       = 65,
	number       = 12,
	pages        = 125315,
}
@article{marquardt2002aharonov-bohm,
	author       = {Marquardt, Florian and Bruder, C},
	title        = {Aharonov-Bohm ring with fluctuating flux},
	journal      = {Phys. Rev. B},
	year         = 2002,
	volume       = 65,
	number       = 12,
	pages        = 125315,
}
@article{mas2019bi-chromatic,
	author       = {Mas, H\`{e}ctor and Pandey, Saurabh and Vasilakis, Georgios and von Klitzing, Wolf},
	title        = {Bi-chromatic adiabatic shells for atom interferometry},
	journal      = {New Journal of Physics},
	year         = 2019,
	volume       = 21,
	pages        = 123039,
}
@article{Mas2019NJOP,
	author       = {Mas, H\`{e}ctor and Pandey, Saurabh and Vasilakis, Georgios and von Klitzing, Wolf},
	title        = {Bi-chromatic adiabatic shells for atom interferometry},
	journal      = {New Journal of Physics},
	year         = 2019,
	volume       = 21,
	pages        = 123039,
}
@article{mathew2015self-heterodyne,
	author       = {Mathew, R. and Kumar, A. and Eckel, S. and Jendrzejewski, F. and Campbell, G. K. and Edwards, Mark and Tiesinga, E.},
	title        = {Self-heterodyne detection of the in situ phase of an atomic superconducting quantum interference device},
	journal      = {Phys. Rev. A},
	year         = 2015,
	volume       = 92,
	pages        = {033602},
	month        = {Sep},
}
@article{matthew2015self-heterodyne,
	author       = {Mathew, R. and Kumar, A. and Eckel, S. and Jendrzejewski, F. and Campbell, G. K. and Edwards, Mark and Tiesinga, E.},
	title        = {Self-heterodyne detection of the in situ phase of an atomic superconducting quantum interference device},
	journal      = {Phys. Rev. A},
	year         = 2015,
	volume       = 92,
	pages        = {033602},
	month        = {Sep},
}
@article{mathey2014decay,
	author       = {Mathey, Amy C. and Clark, Charles W. and Mathey, L.},
	title        = {Decay of a superfluid current of ultracold atoms in a toroidal trap},
	journal      = {Phys. Rev. A},
	year         = 2014,
	volume       = 90,
	number       = 2,
	pages        = {023604},
	month        = {Aug},
}
@article{matveev2002persistent,
	author       = {Matveev, KA and Larkin, AI and Glazman, LI},
	title        = {Persistent current in superconducting nanorings},
	journal      = {Phys. Rev. Lett.},
	year         = 2002,
	volume       = 89,
	number       = 9,
	pages        = {096802},
}
@article{mcdonald201380hk,
	author       = {McDonald, G D and Kuhn, C C N and Bennetts, S and Debs, J E and Hardman, K S and Johnsson, M and Close, J D and Robins, N P},
	title        = {80hk momentum separation with Bloch oscillations in an optically guided atom interferometer},
	journal      = {Physical Review A},
	year         = 2013,
	volume       = 88,
	number       = 5,
	pages        = {053620},
	month        = {Nov},
}
@article{mcdonald2013optically,
	author       = {McDonald, G. D. and Keal, H. and Altin, P. A. and Debs, J. E. and Bennetts, S. and Kuhn, C. C. N. and Hardman, K. S. and Johnsson, M. T. and Close, J. D. and Robins, N. P.},
	title        = {Optically guided linear Mach-Zehnder atom interferometer},
	journal      = {Physical Review A},
	year         = 2013,
	volume       = 87,
	number       = 1,
	pages        = {013632},
	month        = {Jan},
}
@article{mcdonald2014bright,
	author       = {McDonald, Gordon D and Kuhn, Carlos CN and Hardman, Kyle S and Bennetts, Shayne and Everitt, Patrick J and Altin, Paul A and Debs, John E and Close, John D and Robins, Nicholas P},
	title        = {Bright solitonic matter-wave interferometer},
	journal      = {Phys. Rev. Lett.},
	year         = 2014,
	volume       = 113,
	number       = 1,
	pages        = {013002},
	month        = {Jul},
}
@article{mcgloin2003applications,
	author       = {McGloin, David and Spalding, Gabriel C and Melville, H and Sibbett, Wilson and Dholakia, Kishan},
	title        = {Applications of spatial light modulators in atom optics},
	journal      = {Opt. Express},
	year         = 2003,
	volume       = 11,
	number       = 2,
	pages        = {158--166},
}
@article{meek2008trapping,
	author       = {Meek, Samuel A and Bethlem, Hendrick L and Conrad, Horst and Meijer, Gerard},
	title        = {Trapping molecules on a chip in traveling potential wells},
	journal      = {Phys. Rev. Lett.},
	year         = 2008,
	volume       = 100,
	number       = 15,
	pages        = 153003,
}
@article{meek2009trapping,
	author       = {Meek, Samuel A and Conrad, Horst and Meijer, Gerard},
	title        = {Trapping molecules on a chip},
	journal      = {Science},
	year         = 2009,
	volume       = 324,
	number       = 5935,
	pages        = {1699--1702},
}
@article{Meier:2001aa,
	author       = {Meier, F. and Zwerger, W.},
	title        = {Josephson tunneling between weakly interacting Bose-Einstein condensates},
	journal      = {Phys. Rev. A},
	year         = 2001,
	volume       = 64,
	pages        = {033610},
	month        = {Aug},
}
@article{meier2001josephson,
	author       = {Meier, F. and Zwerger, W.},
	title        = {Josephson tunneling between weakly interacting Bose-Einstein condensates},
	journal      = {Phys. Rev. A},
	year         = 2001,
	volume       = 64,
	pages        = {033610},
	month        = {Aug},
}
@article{mielke2015hubbard,
	author       = {Mielke, Andreas},
	title        = {The Hubbard model and its properties},
	journal      = {Many Body Physics: From Kondo to Hubbard. Modeling and Simulation},
	year         = 2015,
	volume       = 5,
}
@article{mielke2015the,
	author       = {Mielke, Andreas},
	title        = {The Hubbard model and its properties},
	journal      = {Many Body Physics: From Kondo to Hubbard. Modeling and Simulation},
	year         = 2015,
	volume       = 5,
}
@article{milburn1997quantum,
	author       = {Milburn, GJ and Corney, J and Wright, Ewan M and Walls, DF},
	title        = {Quantum dynamics of an atomic Bose-Einstein condensate in a double-well potential},
	journal      = {Physical Review A},
	year         = 1997,
	volume       = 55,
	number       = 6,
	pages        = 4318,
}
@article{milner2001optical,
	author       = {Milner, V. and Hanssen, J. L. and Campbell, W. C. and Raizen, M. G.},
	title        = {Optical billiards for atoms},
	journal      = {Physical Review Letters},
	year         = 2001,
	volume       = 86,
	number       = 8,
	pages        = {1514--17},
}
@article{Moan2020PRL,
	author       = {Moan, E. R. and Horne, R. A. and Arpornthip, T. and Luo, Z. and Fallon, A. J. and Berl, S. J. and Sackett, C. A.},
	title        = {Quantum Rotation Sensing with Dual Sagnac Interferometers in an Atom-Optical Waveguide},
	journal      = {Phys. Rev. Lett.},
	year         = 2020,
	volume       = 124,
	number       = 12,
	month        = {Mar},
}
@article{moan2020quantum,
	author       = {Moan, E. R. and Horne, R. A. and Arpornthip, T. and Luo, Z. and Fallon, A. J. and Berl, S. J. and Sackett, C. A.},
	title        = {Quantum Rotation Sensing with Dual Sagnac Interferometers in an Atom-Optical Waveguide},
	journal      = {Phys. Rev. Lett.},
	year         = 2020,
	volume       = 124,
	number       = 12,
	month        = {Mar},
}
@article{mohanty1999persistent,
	author       = {Mohanty, Pritiraj},
	title        = {Persistent current in normal metals},
	journal      = {Annalen der Physik},
	year         = 1999,
	volume       = 8,
	number       = {7-9},
	pages        = {549--558},
}
@article{Mokhov.2008kun,
	author       = {Mokhov, Sergiy and Zeldovich, Boris Ya},
	title        = {{Strength of electromagnetic, acoustic, and Schr\"{o}dinger reflections}},
	journal      = {Proc. Royal Society A},
	year         = 2008,
	volume       = 464,
	number       = 2099,
	pages        = {3071 3080},
}
@article{mokhov2008strength,
	author       = {Mokhov, Sergiy and Zeldovich, Boris Ya},
	title        = {{Strength of electromagnetic, acoustic, and Schr\"{o}dinger reflections}},
	journal      = {Proc. Royal Society A},
	year         = 2008,
	volume       = 464,
	number       = 2099,
	pages        = {3071 3080},
}
@article{morizot2006ring,
	author       = {Morizot, O. and Colombe, Y. and Lorent, V. and Perrin, H. and Garraway, B. M.},
	title        = {Ring trap for ultracold atoms},
	journal      = {Phys. Rev. A},
	year         = 2006,
	volume       = 74,
	number       = 2,
	pages        = {023617},
	month        = aug,
}


@article{moulder2012quantized,
	author       = {Moulder, Stuart and Beattie, Scott and Smith, Robert P and Tammuz, Naaman and Hadzibabic, Zoran},
	title        = {Quantized supercurrent decay in an annular Bose-Einstein condensate},
	journal      = {Phys. Rev. A},
	year         = 2012,
	volume       = 86,
	number       = 1,
	pages        = {013629},
	month        = {Jul},
}
@article{PhysRevLett.98.260407,
	author       = {Mukai, T. and Hufnagel, C. and Kasper, A. and Meno, T. and Tsukada, A. and Semba, K. and Shimizu, F.},
	title        = {Persistent Supercurrent Atom Chip},
	journal      = {Phys. Rev. Lett.},
	year         = 2007,
	volume       = 98,
	pages        = 260407,
	month        = {Jun},
}
@article{mukai2007persistent,
	author       = {Mukai, Tetsuya and Hufnagel, Christoph and Kasper, A and Meno, T and Tsukada, A and Semba, K and Shimizu, F},
	title        = {Persistent supercurrent atom chip},
	journal      = {Phys. Rev. Lett.},
	year         = 2007,
	volume       = 98,
	number       = 26,
	pages        = 260407,
	month        = {Jun},
}
@article{muntinga2013interferometry,
	author       = {Muntinga, H. and Ahlers, H. and Krutzik, Markus and Wenzlawski, Andr\'{e} and Arnold, Stefan and Becker, D. and Bongs, Kai and Dittus, H. and Duncker, H. and Gaaloul, Naceur and Gherasim, C. and Giese, E. and Grzeschik, Christoph and H\"ansch, T. W. and Hellmig, Ortwin and Herr, Waldemar and Herrmann, S. and Kajari, E. and Kleinert, S. and Lammerzahl, C. and Lewoczko-Adamczyk, W. and Malcolm, J. and Meyer, N. and Nolte, R. and Peters, Achim and Popp, M. and Reichel, Jakob and Roura, Albert and Rudolph, J. and Schiemangk, Max and Schneider, M. and Seidel, S. T. and Sengstock, Klaus and Tamma, V. and Valenzuela, Tristan and Vogel, A. and Walser, R. and Wendrich, T. and Windpassinger, P. and Zeller, W. and van Zoest, T. and Ertmer, W. and Schleich, Wolfgang P. and Rasel, E. M.},
	title        = {Interferometry with Bose-Einstein Condensates in Microgravity},
	journal      = {Phys. Rev. Lett.},
	year         = 2013,
	volume       = 110,
	pages        = {093602},
	month        = {Feb},
}
@article{Muntinga2013PRL,
	author       = {Muntinga, H. and Ahlers, H. and Krutzik, Markus and Wenzlawski, Andr\'{e} and Arnold, Stefan and Becker, D. and Bongs, Kai and Dittus, H. and Duncker, H. and Gaaloul, Naceur and Gherasim, C. and Giese, E. and Grzeschik, Christoph and H\"ansch, T. W. and Hellmig, Ortwin and Herr, Waldemar and Herrmann, S. and Kajari, E. and Kleinert, S. and Lammerzahl, C. and Lewoczko-Adamczyk, W. and Malcolm, J. and Meyer, N. and Nolte, R. and Peters, Achim and Popp, M. and Reichel, Jakob and Roura, Albert and Rudolph, J. and Schiemangk, Max and Schneider, M. and Seidel, S. T. and Sengstock, Klaus and Tamma, V. and Valenzuela, Tristan and Vogel, A. and Walser, R. and Wendrich, T. and Windpassinger, P. and Zeller, W. and van Zoest, T. and Ertmer, W. and Schleich, Wolfgang P. and Rasel, E. M.},
	title        = {Interferometry with Bose-Einstein Condensates in Microgravity},
	journal      = {Phys. Rev. Lett.},
	year         = 2013,
	volume       = 110,
	pages        = {093602},
	month        = {Feb},
}
@article{Murmann:2015aa,
	author       = {Murmann, Simon and Bergschneider, Andrea and Klinkhamer, Vincent M. and Z\"urn, Gerhard and Lompe, Thomas and Jochim, Selim},
	title        = {Two Fermions in a Double Well: Exploring a Fundamental Building Block of the Hubbard Model},
	journal      = {Phys. Rev. Lett.},
	year         = 2015,
	volume       = 114,
	pages        = {080402},
	month        = {Feb},
}
@article{murmann2015two,
	author       = {Murmann, Simon and Bergschneider, Andrea and Klinkhamer, Vincent M. and Z\"urn, Gerhard and Lompe, Thomas and Jochim, Selim},
	title        = {Two Fermions in a Double Well: Exploring a Fundamental Building Block of the Hubbard Model},
	journal      = {Phys. Rev. Lett.},
	year         = 2015,
	volume       = 114,
	pages        = {080402},
	month        = {Feb},
}
@article{murray2013probing,
	author       = {Murray, Noel and Krygier, Michael and Edwards, Mark and Wright, K. C. and Campbell, G. K. and Clark, Charles W.},
	title        = {Probing the circulation of ring-shaped Bose-Einstein condensates},
	journal      = {Phys. Rev. A},
	year         = 2013,
	volume       = 88,
	pages        = {053615},
	month        = {Nov},
}
@article{naber2016adsorbate,
	author       = {Naber, J and Machluf, S and Torralbo-Campo, L and Soudijn, ML and Van Druten, NJ and Van Den Heuvell, HB Van Linden and Spreeuw, RJC},
	title        = {Adsorbate dynamics on a silica-coated gold surface measured by Rydberg Stark spectroscopy},
	journal      = {Journal of Physics B: Atomic, Molecular and Optical Physics},
	year         = 2016,
	volume       = 49,
	number       = 9,
	pages        = {094005},
}
@article{naldesi2019angular,
	author       = {Naldesi, Piero and Gomez, Juan Polo and Dunjko, Vanja and Perrin, H\'{e}l\`{e}ne and Olshanii, Maxim and Amico, Luigi and Minguzzi, Anna},
	title        = {Angular momentum fractionalization: the quantum advantage of entangled bosons},
	journal      = {arXiv preprint arXiv:1901.09398},
	year         = 2019,
	pages        = {arXiv:1901.09398},
	month        = {Jan},
}
@article{naldesi2018rise,
	author       = {Naldesi, Piero and Gomez, Juan Polo and Malomed, Boris and Olshanii, Maxim and Minguzzi, Anna and Amico, Luigi},
	title        = {Rise and Fall of a Bright Soliton in an Optical Lattice},
	journal      = {Phys. Rev. Lett.},
	year         = 2019,
	volume       = 122,
	pages        = {053001},
	month        = {Feb},
}
@article{naldesi2019rise,
	author       = {Naldesi, Piero and Gomez, Juan Polo and Malomed, Boris and Olshanii, Maxim and Minguzzi, Anna and Amico, Luigi},
	title        = {Rise and Fall of a Bright Soliton in an Optical Lattice},
	journal      = {Phys. Rev. Lett.},
	year         = 2019,
	volume       = 122,
	pages        = {053001},
	month        = {Feb},
}
@article{navez2016matter-wave,
	author       = {Navez, P and Pandey, S and Mas, H and Poulios, K and Fernholz, T and von Klitzing, W},
	title        = {Matter-wave interferometers using TAAP rings},
	journal      = {New Journal of Physics},
	year         = 2016,
	volume       = 18,
	number       = 7,
	pages        = {075014},
}
@article{Navez2016NJOP,
	author       = {Navez, P and Pandey, S and Mas, H and Poulios, K and Fernholz, T and von Klitzing, W},
	title        = {Matter-wave interferometers using TAAP rings},
	journal      = {New Journal of Physics},
	year         = 2016,
	volume       = 18,
	number       = 7,
	pages        = {075014},
}
@article{navez2016matter,
	author       = {Navez, Patrick and Pandey, Saurabh and Mas, Hector and Poulios, Konstantinos and Fernholz, Thomas and von Klitzing, Wolf},
	title        = {Matter-wave interferometers using TAAP rings},
	journal      = {New Journal of Physics},
	year         = 2016,
	volume       = 18,
	number       = 7,
	pages        = {075014},
}

@book{nazarov_blanter_2009,
	title        = {Quantum Transport: Introduction to Nanoscience},
	publisher    = {Cambridge University Press},
	year         = 2009,
	author       = {Nazarov, Yuli V. and Blanter, Yaroslav M.},
}

@book{nazarov2009quantum,
	title        = {Quantum Transport: Introduction to Nanoscience},
	publisher    = {Cambridge University Press},
	year         = 2009,
	author       = {Nazarov, Yuli V. and Blanter, Yaroslav M.},
}

@article{Nelin.2007,
	author       = {Nelin, Evgenii A.},
	title        = {Impedance model for quantum-mechanical barrier problems},
	journal      = {Physics-Uspekhi},
	year         = 2007,
	volume       = 50,
	pages        = 293,
}
@article{nelin2007impedance,
	author       = {Nelin, Evgenii A.},
	title        = {Impedance model for quantum-mechanical barrier problems},
	journal      = {Physics-Uspekhi},
	year         = 2007,
	volume       = 50,
	pages        = 293,
}

@article{nicolau2020orbital,
	author       = {Nicolau, Eul\`alia and Mompart, Jordi and Juli\'a-D\'{\i}az, Bruno and Ahufinger, Ver\`onica},
	title        = {Orbital angular momentum dynamics of Bose-Einstein condensates trapped in two stacked rings},
	journal      = {Phys. Rev. A},
	year         = 2020,
	volume       = 102,
	pages        = {023331},
	month        = {Aug},
}

@article{Nietner:2014aa,
	author       = {Nietner, Christian and Schaller, Gernot and Brandes, Tobias},
	title        = {Transport with ultracold atoms at constant density},
	journal      = {Phys. Rev. A},
	year         = 2014,
	volume       = 89,
	pages        = {013605},
	month        = {Jan},
}
@article{nietner2014transport,
	author       = {Nietner, Christian and Schaller, Gernot and Brandes, Tobias},
	title        = {Transport with ultracold atoms at constant density},
	journal      = {Phys. Rev. A},
	year         = 2014,
	volume       = 89,
	pages        = {013605},
	month        = {Jan},
}
@article{PhysRevLett.97.200405,
	author       = {Nirrengarten, T. and Qarry, A. and Roux, C. and Emmert, A. and Nogues, G. and Brune, M. and Raimond, J.-M. and Haroche, S.},
	title        = {Realization of a Superconducting Atom Chip},
	journal      = {Phys. Rev. Lett.},
	year         = 2006,
	volume       = 97,
	pages        = 200405,
	month        = {Nov},
}
@article{nirrengarten2006realization,
	author       = {Nirrengarten, Thomas and Qarry, Angie and Roux, C\'{e}dric and Emmert, Andreas and Nogues, Gilles and Brune, Michel and Raimond, J-M and Haroche, Serge},
	title        = {Realization of a superconducting atom chip},
	journal      = {Phys. Rev. Lett.},
	year         = 2006,
	volume       = 97,
	number       = 20,
	pages        = 200405,
	month        = {Nov},
}
@article{nitzan2003electron,
	author       = {Nitzan, Abraham and Ratner, Mark A},
	title        = {Electron transport in molecular wire junctions},
	journal      = {Science},
	year         = 2003,
	volume       = 300,
	number       = 5624,
	pages        = {1384--1389},
}
@article{Nogrette:2014aa,
	author       = {Nogrette, F. and Labuhn, H. and Ravets, S. and Barredo, D. and B\'eguin, L. and Vernier, A. and Lahaye, T. and Browaeys, A.},
	title        = {Single-Atom Trapping in Holographic 2D Arrays of Microtraps with Arbitrary Geometries},
	journal      = {Phys. Rev. X},
	year         = 2014,
	volume       = 4,
	pages        = {021034},
	month        = {May},
}
@article{nogrette2014single-atom,
	author       = {Nogrette, F. and Labuhn, H. and Ravets, S. and Barredo, D. and B\'eguin, L. and Vernier, A. and Lahaye, T. and Browaeys, A.},
	title        = {Single-Atom Trapping in Holographic 2D Arrays of Microtraps with Arbitrary Geometries},
	journal      = {Phys. Rev. X},
	year         = 2014,
	volume       = 4,
	pages        = {021034},
	month        = {May},
}
@article{nunnekamp2008generation,
	author       = {Nunnenkamp, Andreas and Rey, Ana Maria and Burnett, Keith},
	title        = {Generation of macroscopic superposition states in ring superlattices},
	journal      = {Physical Review A},
	year         = 2008,
	volume       = 77,
	number       = 2,
	pages        = {023622},
}
@article{nunnenkamp2008generation,
	author       = {Nunnenkamp, Andreas and Rey, Ana Maria and Burnett, Keith},
	title        = {Generation of macroscopic superposition states in ring superlattices},
	journal      = {Physical Review A},
	year         = 2008,
	volume       = 77,
	number       = 2,
	pages        = {023622},
}
@article{nunnenkamp2010superposition,
	author       = {Nunnenkamp, Andreas and Rey, Ana Maria and Burnett, Keith},
	title        = {Superposition states of ultracold bosons in rotating rings with a weak potential barrier},
	journal      = {gas]},
	year         = 2010,
}
@article{nunnenkamp2011superposition,
	author       = {Nunnenkamp, Andreas and Rey, Ana Maria and Burnett, Keith},
	title        = {Superposition states of ultracold bosons in rotating rings with a realistic potential barrier},
	journal      = {Phys. Rev. A},
	year         = 2011,
	volume       = 84,
	number       = 5,
	pages        = {053604},
}
@article{Oelkers_2007,
	author       = {Oelkers, Norman and Links, Jon},
	title        = {Ground-state properties of the attractive one-dimensional Bose-Hubbard model},
	journal      = {Phys. Rev. B},
	year         = 2007,
	volume       = 75,
	pages        = 115119,
	month        = {Mar},
}
@article{oelkers2007ground-state,
	author       = {Oelkers, Norman and Links, Jon},
	title        = {Ground-state properties of the attractive one-dimensional Bose-Hubbard model},
	journal      = {Phys. Rev. B},
	year         = 2007,
	volume       = 75,
	pages        = 115119,
	month        = {Mar},
}
@article{AB_fundations_RMP,
	author       = {Olariu, S. and Popescu, I. Iovitzu},
	title        = {The quantum effects of electromagnetic fluxes},
	journal      = {Rev. Mod. Phys.},
	year         = 1985,
	volume       = 57,
	pages        = {339--436},
	month        = {Apr},
}
@article{olariu1985the,
	author       = {Olariu, S. and Popescu, I. Iovitzu},
	title        = {The quantum effects of electromagnetic fluxes},
	journal      = {Rev. Mod. Phys.},
	year         = 1985,
	volume       = 57,
	pages        = {339--436},
	month        = {Apr},
}
@article{olson2007cold,
	author       = {Olson, S. E. and Terraciano, M. L. and Bashkansky, M. and Fatemi, F. K.},
	title        = {Cold-atom confinement in an all-optical dark ring trap},
	journal      = {Physical Review A (Atomic, Molecular, and Optical Physics)},
	year         = 2007,
	volume       = 76,
	number       = 6,
	pages        = {061404},
	month        = dec,
}
@article{olson2007cold-atom,
	author       = {Olson, S. E. and Terraciano, M. L. and Bashkansky, M. and Fatemi, F. K.},
	title        = {Cold-atom confinement in an all-optical dark ring trap},
	journal      = {Physical Review A (Atomic, Molecular, and Optical Physics)},
	year         = 2007,
	volume       = 76,
	number       = 6,
	pages        = {061404},
	month        = dec,
}
@article{onofrio2000surface,
	author       = {Onofrio, R. and Durfee, D. S. and Raman, C. and Kohl, M. and Kuklewicz, C. E. and Ketterle, W.},
	title        = {Surface excitations of a Bose-Einstein condensate},
	journal      = {Physical Review Letters},
	year         = 2000,
	volume       = 84,
	number       = 5,
	pages        = {810--13},
}

@article{li2015stability,
  title={Stability of persistent currents in open dissipative quantum fluids},
  author={Li, Guangyao and Fraser, Michael D and Yakimenko, Alexander and Ostrovskaya, Elena A},
  journal={Physical Review B},
  volume={91},
  number={18},
  pages={184518},
  year={2015},
  publisher={APS}
}


@article{ozawa2019topological,
	author       = {Ozawa, Tomoki and Price, Hannah M},
	title        = {Topological quantum matter in synthetic dimensions},
	journal      = {Nature Reviews Physics},
	year         = 2019,
	volume       = 1,
	number       = 5,
	pages        = {349--357},
}
@article{Packard:1998aa,
	author       = {Packard, Richard E.},
	title        = {The role of the Josephson-Anderson equation in superfluid helium},
	journal      = {Rev. Mod. Phys.},
	year         = 1998,
	volume       = 70,
	pages        = {641--651},
	month        = {Apr},
}
@article{packard1998the,
	author       = {Packard, Richard E.},
	title        = {The role of the Josephson-Anderson equation in superfluid helium},
	journal      = {Rev. Mod. Phys.},
	year         = 1998,
	volume       = 70,
	pages        = {641--651},
	month        = {Apr},
}
@book{padron2012interferometry,
	title        = {Interferometry: Research and Applications in Science and Technology},
	publisher    = {BoD--Books on Demand},
	year         = 2012,
	author       = {Padron, Ivan},
}
@book{padron2012interferometry:,
	title        = {Interferometry: Research and Applications in Science and Technology},
	publisher    = {BoD--Books on Demand},
	year         = 2012,
	author       = {Padron, Ivan},
}
@article{pagano2015strongly,
	author       = {Pagano, G and Mancini, M and Cappellini, G and Livi, L and Sias, C and Catani, J and Inguscio, M and Fallani, L},
	title        = {Strongly interacting gas of two-electron fermions at an orbital Feshbach resonance},
	journal      = {Phys. Rev. Lett.},
	year         = 2015,
	volume       = 115,
	number       = 26,
	pages        = 265301,
}
@article{pandey2019hypersonic,
	author       = {Pandey, Saurabh and Mas, Hector and Drougakis, Giannis and Thekkeppatt, Premjith and Bolpasi, Vasiliki and Vasilakis, Georgios and Poulios, Konstantinos and von Klitzing, Wolf},
	title        = {Hypersonic Bose--Einstein condensates in accelerator rings},
	journal      = {Nature},
	year         = 2019,
	volume       = 570,
	number       = 7760,
	pages        = 1,
	month        = jun,
}
@article{Papoular:2014aa,
	author       = {Papoular, D. J. and Pitaevskii, L. P. and Stringari, S.},
	title        = {Fast Thermalization and Helmholtz Oscillations of an Ultracold Bose Gas},
	journal      = {Phys. Rev. Lett.},
	year         = 2014,
	volume       = 113,
	pages        = 170601,
	month        = {Oct},
}
@article{papoular2014fast,
	author       = {Papoular, D. J. and Pitaevskii, L. P. and Stringari, S.},
	title        = {Fast Thermalization and Helmholtz Oscillations of an Ultracold Bose Gas},
	journal      = {Phys. Rev. Lett.},
	year         = 2014,
	volume       = 113,
	pages        = 170601,
	month        = {Oct},
}
@article{Papoular:2016aa,
	author       = {Papoular, D. J. and Pitaevskii, L. P. and Stringari, S.},
	title        = {Quantized conductance through the quantum evaporation of bosonic atoms},
	journal      = {Phys. Rev. A},
	year         = 2016,
	volume       = 94,
	pages        = {023622},
	month        = {Aug},
}
@article{papoular2016quantized,
	author       = {Papoular, D. J. and Pitaevskii, L. P. and Stringari, S.},
	title        = {Quantized conductance through the quantum evaporation of bosonic atoms},
	journal      = {Phys. Rev. A},
	year         = 2016,
	volume       = 94,
	pages        = {023622},
	month        = {Aug},
}
@article{pecci2020probing,
	author       = {Pecci, Giovanni and Naldesi, Piero and Minguzzi, Anna and Amico, Luigi},
	title        = {Probing the BCS-BEC crossover with persistent currents},
	journal      = {arXiv preprint arXiv:2010..03552},
	year         = 2020,
}
@article{pecci2021phase,
	author       = {Pecci, Giovanni and Naldesi, Piero and Minguzzi, Anna and Amico, Luigi},
	title        = {The phase of a degenerate Fermi gas},
	journal      = {arXiv preprint arXiv:2105.XXXX},
	year         = 2021,
}
@article{pecci2021the,
	author       = {Pecci, Giovanni and Naldesi, Piero and Minguzzi, Anna and Amico, Luigi},
	title        = {The phase of a degenerate Fermi gas},
	journal      = {arXiv preprint arXiv:2105.XXXX},
	year         = 2021,
}
@article{peierls1933theorie,
	author       = {Peierls, Rudolph},
	title        = {Zur theorie des diamagnetismus von leitungselektronen},
	journal      = {Zeitschrift f\"{u}r Physik},
	year         = 1933,
	volume       = 80,
	number       = {11-12},
	pages        = {763--791},
}
@article{peierls1933zur,
	author       = {Peierls, Rudolph},
	title        = {Zur theorie des diamagnetismus von leitungselektronen},
	journal      = {Zeitschrift f\"{u}r Physik},
	year         = 1933,
	volume       = 80,
	number       = {11-12},
	pages        = {763--791},
}

@article{pelegri2018quantum,
	doi = {10.1088/1367-2630/aae107},
	url = {https://doi.org/10.1088/1367-2630/aae107},
	year = 2018,
	month = {oct},
	publisher = {{IOP} Publishing},
	volume = {20},
	number = {10},
	pages = {103001},
	author = {G Pelegr{\'{\i}} and J Mompart and V Ahufinger},
	title = {Quantum sensing using imbalanced counter-rotating Bose{\textendash}Einstein condensate modes},
	journal = {New Journal of Physics},
	abstract = {A quantum device for measuring two-body interactions, scalar magnetic fields and rotations is proposed using a Bose–Einstein condensate (BEC) in a ring trap. We consider an imbalanced superposition of orbital angular momentum modes with opposite winding numbers for which a rotating minimal atomic density line appears. We derive an analytical model relating the angular frequency of the minimal density line rotation to the strength of the nonlinear atom–atom interactions and the difference between the populations of the counter-propagating modes. Additionally, we propose a full experimental protocol based on direct fluorescence imaging of the BEC that allows to measure all the quantities involved in the analytical model and use the system for sensing purposes.}
}

@article{pepino2009atomtronic,
	author       = {Pepino, RA and Cooper, J and Anderson, DZ and Holland, MJ},
	title        = {Atomtronic circuits of diodes and transistors},
	journal      = {Phys. Rev. Lett.},
	year         = 2009,
	volume       = 103,
	number       = 14,
	pages        = 140405,
}
@article{pepino2021advances,
	author       = {Pepino, Ron A},
	title        = {Advances in atomtronics},
	journal      = {Entropy},
	year         = 2021,
	volume       = 23,
	number       = 5,
	pages        = 534,
}
@article{Perrin2017AIAMAOP,
	author       = {Perrin, H\'{e}l\`{e}ne and Garraway, Barry M.},
	title        = {Trapping Atoms With Radio Frequency Adiabatic Potentials},
	journal      = {Advances In Atomic, Molecular, and Optical Physics},
	year         = 2017,
}
@article{perrin2017trapping,
	author       = {Perrin, H\'{e}l\`{e}ne and Garraway, Barry M.},
	title        = {Trapping Atoms With Radio Frequency Adiabatic Potentials},
	journal      = {Advances In Atomic, Molecular, and Optical Physics},
	year         = 2017,
}
@article{Pershoguba:2019aa,
	author       = {Pershoguba, Sergey S. and Glazman, Leonid I.},
	title        = {Thermopower and thermal conductance of a superconducting quantum point contact},
	journal      = {Phys. Rev. B},
	year         = 2019,
	volume       = 99,
	pages        = 134514,
	month        = {Apr},
}
@article{pershoguba2019thermopower,
	author       = {Pershoguba, Sergey S. and Glazman, Leonid I.},
	title        = {Thermopower and thermal conductance of a superconducting quantum point contact},
	journal      = {Phys. Rev. B},
	year         = 2019,
	volume       = 99,
	pages        = 134514,
	month        = {Apr},
}
@article{Petrich1995PRL,
	author       = {Petrich, W. and Anderson, M. H. and Ensher, J. R. and Cornell, E. A.},
	title        = {Stable, Tightly Confining Magnetic Trap for Evaporative Cooling of Neutral Atoms},
	journal      = {Physical Review Letters},
	year         = 1995,
	volume       = 74,
	number       = 17,
	pages        = {3352--3355},
	month        = 3,
}
@article{petrich1995stable,
	author       = {Petrich, W. and Anderson, M. H. and Ensher, J. R. and Cornell, E. A.},
	title        = {Stable, Tightly Confining Magnetic Trap for Evaporative Cooling of Neutral Atoms},
	journal      = {Physical Review Letters},
	year         = 1995,
	volume       = 74,
	number       = 17,
	pages        = {3352--3355},
	month        = 3,
}
@article{petrosyan2019microwave,
	author       = {Petrosyan, David and M\o{}lmer, Klaus and Fort\'{a}gh, J\'{o}zsef and Saffman, Mark},
	title        = {Microwave to optical conversion with atoms on a superconducting chip},
	journal      = {New Journal of Physics},
	year         = 2019,
	volume       = 21,
	number       = 7,
	pages        = {073033},
}
@article{Pezze:2018aa,
	author       = {Pezz\`e, Luca and Smerzi, Augusto and Oberthaler, Markus K. and Schmied, Roman and Treutlein, Philipp},
	title        = {Quantum metrology with nonclassical states of atomic ensembles},
	journal      = {Rev. Mod. Phys.},
	year         = 2018,
	volume       = 90,
	pages        = {035005},
	month        = {Sep},
}
@article{pezze2018quantum,
	author       = {Pezz\`e, Luca and Smerzi, Augusto and Oberthaler, Markus K. and Schmied, Roman and Treutlein, Philipp},
	title        = {Quantum metrology with nonclassical states of atomic ensembles},
	journal      = {Rev. Mod. Phys.},
	year         = 2018,
	volume       = 90,
	pages        = {035005},
	month        = {Sep},
}
@article{piazza2009vortex,
	author       = {Piazza, F. and Collins, L. A. and Smerzi, A.},
	title        = {Vortex-induced phase-slip dissipation in a toroidal Bose-Einstein condensate flowing through a barrier},
	journal      = {Phys. Rev. A},
	year         = 2009,
	volume       = 80,
	number       = 2,
	pages        = {021601(R)},
	month        = {aug},
}
@article{piazza2009vortex-induced,
	author       = {Piazza, F. and Collins, L. A. and Smerzi, A.},
	title        = {Vortex-induced phase-slip dissipation in a toroidal Bose-Einstein condensate flowing through a barrier},
	journal      = {Phys. Rev. A},
	year         = 2009,
	volume       = 80,
	number       = 2,
	pages        = {021601(R)},
	month        = {aug},
}
@article{polo2016transport,
	author       = {Polo, Joan and Benseny, Albert and Busch, Th and Ahufinger, Ver\`{o}nica and Mompart, Jordi},
	title        = {Transport of ultracold atoms between concentric traps via spatial adiabatic passage},
	journal      = {New J. Phys.},
	year         = 2016,
	volume       = 18,
	number       = 1,
	pages        = {015010},
}
@article{polo2018damping,
	author       = {Polo, Juan and Ahufinger, V and Hekking, Frank WJ and Minguzzi, Anna},
	title        = {Damping of Josephson oscillations in strongly correlated one-dimensional atomic gases},
	journal      = {Phys. Rev. Lett.},
	year         = 2018,
	volume       = 121,
	number       = 9,
	pages        = {090404},
}
@article{polo2013soliton,
	author       = {Polo, Juan and Ahufinger, Ver\`{o}nica},
	title        = {Soliton-based matter-wave interferometer},
	journal      = {Physical Review A},
	year         = 2013,
	volume       = 88,
	number       = 5,
	pages        = {053628},
}
@article{polo2013soliton-based,
	author       = {Polo, Juan and Ahufinger, Ver\`{o}nica},
	title        = {Soliton-based matter-wave interferometer},
	journal      = {Physical Review A},
	year         = 2013,
	volume       = 88,
	number       = 5,
	pages        = {053628},
}
@article{polo2019oscillations,
	author       = {Polo, Juan and Dubessy, Romain and Pedri, Paolo and Perrin, H\'el\`ene and Minguzzi, Anna},
	title        = {Oscillations and Decay of Superfluid Currents in a One-Dimensional Bose Gas on a Ring},
	journal      = {Phys. Rev. Lett.},
	year         = 2019,
	volume       = 123,
	pages        = 195301,
	month        = {Nov},
}

@article{polo2020quantum,
	author       = {Polo, Juan and Naldesi, Piero and Minguzzi, Anna and Amico, Luigi},
	title        = {The quantum solitons atomtronic interference device},
	journal      = {arXiv preprint arXiv:2012.06269},
	year         = 2020,
}

@article{polo2020the,
	author       = {Polo, Juan and Naldesi, Piero and Minguzzi, Anna and Amico, Luigi},
	title        = {The quantum solitons atomtronic interference device},
	journal      = {arXiv preprint arXiv:2012.06269},
	year         = 2020,
}
@article{Price:2017aa,
	author       = {Price, Hannah M. and Ozawa, Tomoki and Goldman, Nathan},
	title        = {Synthetic dimensions for cold atoms from shaking a harmonic trap},
	journal      = {Phys. Rev. A},
	year         = 2017,
	volume       = 95,
	pages        = {023607},
	month        = {Feb},
}
@article{price2017synthetic,
	author       = {Price, Hannah M. and Ozawa, Tomoki and Goldman, Nathan},
	title        = {Synthetic dimensions for cold atoms from shaking a harmonic trap},
	journal      = {Phys. Rev. A},
	year         = 2017,
	volume       = 95,
	pages        = {023607},
	month        = {Feb},
}
@article{pritchard1983cooling,
	author       = {Pritchard, D. E.},
	title        = {Cooling Neutral Atoms in a Magnetic Trap for Precision Spectroscopy},
	journal      = {Physical Review Letters},
	year         = 1983,
	volume       = 51,
	number       = 15,
	pages        = {1336--1339},
}
@article{Pritchard1983PRL,
	author       = {Pritchard, D. E.},
	title        = {Cooling Neutral Atoms in a Magnetic Trap for Precision Spectroscopy},
	journal      = {Physical Review Letters},
	year         = 1983,
	volume       = 51,
	number       = 15,
	pages        = {1336--1339},
}
@article{pritchard2012demonstration,
	author       = {Pritchard, J D and Dinkelaker, A N and Arnold, A S and Griffin, P F and Riis, E},
	title        = {Demonstration of an inductively coupled ring trap for cold atoms},
	journal      = {New Journal of Physics},
	year         = 2012,
	volume       = 14,
	number       = 10,
	pages        = 103047,
	month        = oct,
}
@article{pyykkonen2021flat,
	author       = {Pyykk\"onen, Ville A. J. and Peotta, Sebastiano and Fabritius, Philipp and Mohan, Jeffrey and Esslinger, Tilman and T\"orm\"a, P\"aivi},
	title        = {Flat-band transport and Josephson effect through a finite-size sawtooth lattice},
	journal      = {Phys. Rev. B},
	year         = 2021,
	volume       = 103,
	pages        = 144519,
	month        = {Apr},
}
@article{pyykkonen2021flat-band,
	author       = {Pyykk\"onen, Ville A. J. and Peotta, Sebastiano and Fabritius, Philipp and Mohan, Jeffrey and Esslinger, Tilman and T\"orm\"a, P\"aivi},
	title        = {Flat-band transport and Josephson effect through a finite-size sawtooth lattice},
	journal      = {Phys. Rev. B},
	year         = 2021,
	volume       = 103,
	pages        = 144519,
	month        = {Apr},
}
@article{Qi2017APL,
	author       = {Qi, Lu and Hu, Zhaohui and Valenzuela, Tristan and Zhang, Yuchi and Zhai, Yueyang and Quan, Wei and Waltham, Nick and Fang, Jiancheng},
	title        = {Magnetically guided Cesium interferometer for inertial sensing},
	journal      = {Applied Physics Letters},
	year         = 2017,
	volume       = 110,
	number       = 15,
	pages        = 153502,
	month        = {Apr},
}
@article{qi2017magnetically,
	author       = {Qi, Lu and Hu, Zhaohui and Valenzuela, Tristan and Zhang, Yuchi and Zhai, Yueyang and Quan, Wei and Waltham, Nick and Fang, Jiancheng},
	title        = {Magnetically guided Cesium interferometer for inertial sensing},
	journal      = {Applied Physics Letters},
	year         = 2017,
	volume       = 110,
	number       = 15,
	pages        = 153502,
	month        = {Apr},
}
@article{ramanathan2011superflow,
	author       = {Ramanathan, A. and Wright, K. C. and Muniz, S. R. and Zelan, M. and Hill, W. T. and Lobb, C. J. and Helmerson, K. and Phillips, W. D. and Campbell, G. K.},
	title        = {Superflow in a Toroidal Bose-Einstein Condensate: An Atom Circuit with a Tunable Weak Link},
	journal      = {Phys. Rev. Lett.},
	year         = 2011,
	volume       = 106,
	number       = 13,
	pages        = 130401,
	month        = {Mar},
}
@article{reichel1999atomic,
	author       = {Reichel, J. and H\"{a}nsel, W. and H\"{a}nsch, T. W.},
	title        = {Atomic Micromanipulation with Magnetic Surface Traps},
	journal      = {Physical Review Letters},
	year         = 1999,
	volume       = 83,
	number       = 17,
	pages        = {3398--3401},
	month        = {oct},
}
@article{Reichel1999PRL,
	author       = {Reichel, J. and H\"{a}nsel, W. and H\"{a}nsch, T. W.},
	title        = {Atomic Micromanipulation with Magnetic Surface Traps},
	journal      = {Physical Review Letters},
	year         = 1999,
	volume       = 83,
	number       = 17,
	pages        = {3398--3401},
	month        = {oct},
}
@article{renn1996evanescent,
	author       = {Renn, Michael J. and Donley, Elizabeth A. and Cornell, Eric A. and Wieman, Carl E. and Anderson, Dana Z.},
	title        = {Evanescent-wave guiding of atoms in hollow optical fibers},
	journal      = {Physical Review A},
	year         = 1996,
	volume       = 53,
	number       = 2,
	pages        = {R648-R651},
}
@article{renn1996evanescent-wave,
	author       = {Renn, Michael J. and Donley, Elizabeth A. and Cornell, Eric A. and Wieman, Carl E. and Anderson, Dana Z.},
	title        = {Evanescent-wave guiding of atoms in hollow optical fibers},
	journal      = {Physical Review A},
	year         = 1996,
	volume       = 53,
	number       = 2,
	pages        = {R648-R651},
}
@article{rhodes2002guiding,
	author       = {Rhodes, D. P. and Lancaster, G. P. T. and Livesey, J. and McGloin, D. and Arlt, J. and Dholakia, K.},
	title        = {Guiding a cold atomic beam along a co-propagating and oblique hollow light guide},
	journal      = {Optics Communications},
	year         = 2002,
	volume       = 214,
	number       = {1--6},
	pages        = {247--254},
}
@article{riedel1993mesoscopic,
	author       = {Riedel, Eberhard K and von Oppen, Felix},
	title        = {Mesoscopic persistent current in small rings},
	journal      = {Physical Review B},
	year         = 1993,
	volume       = 47,
	number       = 23,
	pages        = 15449,
}
@article{rieger2005continuous,
	author       = {Rieger, Thomas and Junglen, Tobias and Rangwala, Sadiqali A and Pinkse, Pepijn WH and Rempe, Gerhard},
	title        = {Continuous loading of an electrostatic trap for polar molecules},
	journal      = {Phys. Rev. Lett.},
	year         = 2005,
	volume       = 95,
	number       = 17,
	pages        = 173002,
}
@article{rincon2009features,
	author       = {Rinc\'{o}n, Juli\'{a}n and Aligia, AA and Hallberg, K},
	title        = {Features of spin-charge separation in the equilibrium conductance through finite rings},
	journal      = {Phys. Rev. B},
	year         = 2009,
	volume       = 79,
	number       = 3,
	pages        = {035112},
}
@article{rincon2008spin,
	author       = {Rinc\'{o}n, Juli\'{a}n and Hallberg, K and Aligia, AA},
	title        = {Spin-charge separation in strongly interacting finite ladder rings},
	journal      = {Phys. Rev. B},
	year         = 2008,
	volume       = 78,
	number       = 12,
	pages        = 125115,
}
@article{rincon2008spin-charge,
	author       = {Rinc\'{o}n, Juli\'{a}n and Hallberg, K and Aligia, AA},
	title        = {Spin-charge separation in strongly interacting finite ladder rings},
	journal      = {Phys. Rev. B},
	year         = 2008,
	volume       = 78,
	number       = 12,
	pages        = 125115,
}
@article{roscilde2016from,
	author       = {Roscilde, Tommaso and Faulkner, Michael F and Bramwell, Steven T and Holdsworth, Peter C W},
	title        = {From quantum to thermal topological-sector fluctuations of strongly interacting Bosons in a ring lattice},
	journal      = {New J. Phys.},
	year         = 2016,
	volume       = 18,
	number       = 7,
	pages        = {075003},
}
@article{Rubinsztein_Dunlop_2016,
	author       = {Rubinsztein-Dunlop, Halina and Forbes, Andrew and Berry, M V and Dennis, M R and Andrews, David L and Mansuripur, Masud and Denz, Cornelia and Alpmann, Christina and Banzer, Peter and Bauer, Thomas and Karimi, Ebrahim and Marrucci, Lorenzo and Padgett, Miles and Ritsch-Marte, Monika and Litchinitser, Natalia M and Bigelow, Nicholas P and Rosales-Guzm{\'{a}}n, C and Belmonte, A and Torres, J P and Neely, Tyler W and Baker, Mark and Gordon, Reuven and Stilgoe, Alexander B and Romero, Jacquiline and White, Andrew G and Fickler, Robert and Willner, Alan E and Xie, Guodong and McMorran, Benjamin and Weiner, Andrew M},
	title        = {Roadmap on structured light},
	journal      = {Journal of Optics},
	year         = 2016,
	volume       = 19,
	number       = 1,
	pages        = {013001},
	month        = {nov},
}
@article{rubinsztein-dunlop2016roadmap,
	author       = {Rubinsztein-Dunlop, Halina and Forbes, Andrew and Berry, M V and Dennis, M R and Andrews, David L and Mansuripur, Masud and Denz, Cornelia and Alpmann, Christina and Banzer, Peter and Bauer, Thomas and Karimi, Ebrahim and Marrucci, Lorenzo and Padgett, Miles and Ritsch-Marte, Monika and Litchinitser, Natalia M and Bigelow, Nicholas P and Rosales-Guzm{\'{a}}n, C and Belmonte, A and Torres, J P and Neely, Tyler W and Baker, Mark and Gordon, Reuven and Stilgoe, Alexander B and Romero, Jacquiline and White, Andrew G and Fickler, Robert and Willner, Alan E and Xie, Guodong and McMorran, Benjamin and Weiner, Andrew M},
	title        = {Roadmap on structured light},
	journal      = {Journal of Optics},
	year         = 2016,
	volume       = 19,
	number       = 1,
	pages        = {013001},
	month        = {nov},
}
@article{Ruostekoski:1998aa,
	author       = {Ruostekoski, Janne and Walls, Dan F.},
	title        = {Bose-Einstein condensate in a double-well potential as an open quantum system},
	journal      = {Phys. Rev. A},
	year         = 1998,
	volume       = 58,
	pages        = {R50--R53},
	month        = {Jul},
}
@article{ruostekoski1998bose-einstein,
	author       = {Ruostekoski, Janne and Walls, Dan F.},
	title        = {Bose-Einstein condensate in a double-well potential as an open quantum system},
	journal      = {Phys. Rev. A},
	year         = 1998,
	volume       = 58,
	pages        = {R50--R53},
	month        = {Jul},
}

@article{ryu2007observation,
	Author = {C. Ryu and M. Andersen and P. Clad{\'{e}} and Vasant Natarajan and K. Helmerson and W. Phillips},
	Title = {Observation of Persistent Flow of a Bose-Einstein Condensate in a Toroidal Trap},
	Journal = {Physical Review Letters},
	Year = 2007,
	Volume = {99},
	Number = {26},
	Pages = {},
	Month = {dec},
	URL = {https://doi.org/10.1103/physrevlett.99.260401},
	DOI = {10.1103/PhysRevLett.99.260401},
}


@article{ryu2013experimental,
	author       = {Ryu, C and Blackburn, PW and Blinova, AA and Boshier, MG},
	title        = {Experimental realization of Josephson junctions for an atom SQUID},
	journal      = {Phys. Rev. Lett.},
	year         = 2013,
	volume       = 111,
	number       = 20,
	pages        = 205301,
	month        = {Nov},
}
@article{Ryu2015NJOP,
	author       = {Ryu, C. and Boshier, M. G.},
	title        = {Integrated coherent matter wave circuits},
	journal      = {New Journal of Physics},
	year         = 2015,
	volume       = 17,
	number       = 9,
}
@article{ryu2014creation,
	author       = {Ryu, C. and Henderson, K. C. and Boshier, M. G.},
	title        = {Creation of matter wave Bessel beams and observation of quantized circulation in a Bose--Einstein condensate},
	journal      = {New Journal of Physics},
	year         = 2014,
	volume       = 16,
	number       = 1,
	pages        = {013046},
	month        = {jan},
}
@article{ryu2020quantum,
	author       = {Ryu, C. and Samson, E. C. and Boshier, M. G.},
	title        = {Quantum interference of currents in an atomtronic SQUID},
	journal      = {Nature Communications},
	year         = 2020,
	volume       = 11,
	number       = 1,
	pages        = 3338,
}
@article{ryu2015integrated,
	author       = {Ryu, Changhyun and Boshier, Malcolm Geoffrey},
	title        = {Integrated coherent matter wave circuits},
	journal      = {New Journal of Physics},
	year         = 2015,
	volume       = 17,
	number       = 9,
	pages        = {092002},
	month        = {sep},
}
@article{safaei2018two,
	author       = {Safaei, Shabnam and Gr\'{e}maud, Beno\^{\i}t and Dumke, Rainer and Kwek, L-C and Amico, Luigi and Miniatura, Christian},
	title        = {Two-dimensional network of atomtronic qubits},
	journal      = {Physical Review A},
	year         = 2018,
	volume       = 97,
	number       = 4,
	pages        = {042306},
}
@article{safaei2018two-dimensional,
	author       = {Safaei, Shabnam and Gr\'{e}maud, Beno\^{\i}t and Dumke, Rainer and Kwek, L-C and Amico, Luigi and Miniatura, Christian},
	title        = {Two-dimensional network of atomtronic qubits},
	journal      = {Physical Review A},
	year         = 2018,
	volume       = 97,
	number       = 4,
	pages        = {042306},
}
@article{saffman2010quantum,
	author       = {Saffman, Mark and Walker, Thad G and M\o{}lmer, Klaus},
	title        = {Quantum information with Rydberg atoms},
	journal      = {Reviews of Modern Physics},
	year         = 2010,
	volume       = 82,
	number       = 3,
	pages        = 2313,
}
@article{Salerno:2019aa,
	author       = {Salerno, G. and Price, H. M. and Lebrat, M. and H\"ausler, S. and Esslinger, T. and Corman, L. and Brantut, J.-P. and Goldman, N.},
	title        = {Quantized Hall Conductance of a Single Atomic Wire: A Proposal Based on Synthetic Dimensions},
	journal      = {Phys. Rev. X},
	year         = 2019,
	volume       = 9,
	pages        = {041001},
	month        = {Oct},
}
@article{salerno2019quantized,
	author       = {Salerno, G. and Price, H. M. and Lebrat, M. and H\"ausler, S. and Esslinger, T. and Corman, L. and Brantut, J.-P. and Goldman, N.},
	title        = {Quantized Hall Conductance of a Single Atomic Wire: A Proposal Based on Synthetic Dimensions},
	journal      = {Phys. Rev. X},
	year         = 2019,
	volume       = 9,
	pages        = {041001},
	month        = {Oct},
}
@article{salim2013high,
	author       = {Salim, Evan A and Caliga, Seth C and Pfeiffer, Jonathan B and Anderson, Dana Z},
	title        = {High resolution imaging and optical control of Bose-Einstein condensates in an atom chip magnetic trap},
	journal      = {Applied Physics Letters},
	year         = 2013,
	volume       = 102,
	number       = 8,
	pages        = {084104},
}
@article{saminadayar2004equilibrium,
	author       = {Saminadayar, L. and Bauerle, C. and Mailly, D.},
	title        = {Equilibrium properties of mesoscopic quantum conductors},
	journal      = {Enc. Nanosci. Nanotech},
	year         = 2004,
	volume       = 4,
	pages        = 267,
}

@article{sanvitto2010persistent,
  title={Persistent currents and quantized vortices in a polariton superfluid},
  author={Sanvitto, D and Marchetti, FM and Szyma{\'n}ska, MH and Tosi, Guilherme and Baudisch, M and Laussy, Fabrice P and Krizhanovskii, DN and Skolnick, MS and Marrucci, L and Lemaitre, A and others},
  journal={Nature Physics},
  volume={6},
  number={7},
  pages={527--533},
  year={2010},
  publisher={Nature Publishing Group}
}


@article{sauer2001storage,
	author       = {Sauer, J. A. and Barrett, M. D. and Chapman, M. S.},
	title        = {Storage Ring for Neutral Atoms},
	journal      = {Phys. Rev. Lett.},
	year         = 2001,
	volume       = 87,
	number       = 27,
	pages        = 270401,
	month        = {Dec},
}
@article{schenke2011nonadiabatic,
	author       = {Schenke, C. and Minguzzi, A. and Hekking, F. W. J.},
	title        = {Nonadiabatic creation of macroscopic superpositions with strongly correlated one-dimensional bosons in a ring trap},
	journal      = {Phys. Rev. A},
	year         = 2011,
	volume       = 84,
	pages        = {053636},
	month        = {Nov},
}
@article{schmiedmayer1995guiding,
	author       = {Schmiedmayer, J.},
	title        = {Guiding and trapping a neutral atom on a wire},
	journal      = {Physical Review A},
	year         = 1995,
	volume       = 52,
	number       = 1,
	pages        = {R13-R16},
	month        = 7,
}
@article{Schmiedmayer1995PRA,
	author       = {Schmiedmayer, J.},
	title        = {Guiding and trapping a neutral atom on a wire},
	journal      = {Physical Review A},
	year         = 1995,
	volume       = 52,
	number       = 1,
	pages        = {R13-R16},
	month        = 7,
}
@article{schnelle2008versatile,
	author       = {Schnelle, S. K. and Van Ooijen, E. D. and Davis, M. J. and Heckenberg, N. R. and Rubinsztein-Dunlop, H.},
	title        = {Versatile two-dimensional potentials for ultra-cold atoms},
	journal      = {Optics Express},
	year         = 2008,
	volume       = 16,
	number       = 3,
	pages        = {1405--1412},
}
@article{Schumm2005Matter,
	author       = {Schumm, T. and Hofferberth, S. and Andersson, L. M. and Wildermuth, S. and Groth, S. and Bar-Joseph, I. and Schmiedmayer, J. and Kruger, P.},
	title        = {Matter-wave interferometry in a double well on an atom chip},
	journal      = {Nature Physics},
	year         = 2005,
	volume       = 1,
	number       = 1,
	pages        = {57--62},
	month        = 10,
}
@article{schumm2005matter-wave,
	author       = {Schumm, T. and Hofferberth, S. and Andersson, L. M. and Wildermuth, S. and Groth, S. and Bar-Joseph, I. and Schmiedmayer, J. and Kruger, P.},
	title        = {Matter-wave interferometry in a double well on an atom chip},
	journal      = {Nature Physics},
	year         = 2005,
	volume       = 1,
	number       = 1,
	pages        = {57--62},
	month        = 10,
}
@article{seaman2007atomtronics,
	author       = {Seaman, BT and Kr\"{a}mer, M and Anderson, DZ and Holland, MJ},
	title        = {Atomtronics: Ultracold-atom analogs of electronic devices},
	journal      = {Phys. Rev. A},
	year         = 2007,
	volume       = 75,
	number       = 2,
	pages        = {023615},
	month        = {Feb},
}
@article{seaman2007atomtronics:,
	author       = {Seaman, BT and Kr\"{a}mer, M and Anderson, DZ and Holland, MJ},
	title        = {Atomtronics: Ultracold-atom analogs of electronic devices},
	journal      = {Phys. Rev. A},
	year         = 2007,
	volume       = 75,
	number       = 2,
	pages        = {023615},
	month        = {Feb},
}
@article{Sekera:2016aa,
	author       = {Sekera, Tibor and Bruder, Christoph and Belzig, Wolfgang},
	title        = {Thermoelectricity in a junction between interacting cold atomic Fermi gases},
	journal      = {Phys. Rev. A},
	year         = 2016,
	volume       = 94,
	pages        = {033618},
	month        = {Sep},
}
@article{sekera2016thermoelectricity,
	author       = {Sekera, Tibor and Bruder, Christoph and Belzig, Wolfgang},
	title        = {Thermoelectricity in a junction between interacting cold atomic Fermi gases},
	journal      = {Phys. Rev. A},
	year         = 2016,
	volume       = 94,
	pages        = {033618},
	month        = {Sep},
}
@article{sherlock2011time,
	author       = {Sherlock, B. E. and Gildemeister, M. and Owen, E. and Nugent, E. and Foot, C. J.},
	title        = {Time-averaged adiabatic ring potential for ultracold atoms},
	journal      = {Physical Review A},
	year         = 2011,
	volume       = 83,
	number       = 4,
	month        = apr,
}
@article{sherlock2011time-averaged,
	author       = {Sherlock, B. E. and Gildemeister, M. and Owen, E. and Nugent, E. and Foot, C. J.},
	title        = {Time-averaged adiabatic ring potential for ultracold atoms},
	journal      = {Physical Review A},
	year         = 2011,
	volume       = 83,
	number       = 4,
	month        = apr,
}
@article{shmakov2013aharonov,
	author       = {Shmakov, PM and Dmitriev, AP and Kachorovskii, V Yu},
	title        = {Aharonov-Bohm conductance of a disordered single-channel quantum ring},
	journal      = {Phys. Rev. B},
	year         = 2013,
	volume       = 87,
	number       = 23,
	pages        = 235417,
}
@article{shmakov2013aharonov-bohm,
	author       = {Shmakov, PM and Dmitriev, AP and Kachorovskii, V Yu},
	title        = {Aharonov-Bohm conductance of a disordered single-channel quantum ring},
	journal      = {Phys. Rev. B},
	year         = 2013,
	volume       = 87,
	number       = 23,
	pages        = 235417,
}
@article{shuman2010laser,
	author       = {Shuman, Edward S and Barry, John F and DeMille, David},
	title        = {Laser cooling of a diatomic molecule},
	journal      = {Nature},
	year         = 2010,
	volume       = 467,
	number       = 7317,
	pages        = {820--823},
}
@article{Simpson:2014aa,
	author       = {Simpson, DP and Gangardt, DM and Lerner, IV and Kr\"{u}ger, P},
	title        = {One-dimensional transport of bosons between weakly linked reservoirs},
	journal      = {Physical review letters},
	year         = 2014,
	volume       = 112,
	number       = 10,
	pages        = 100601,
}
@article{simpson2014one-dimensional,
	author       = {Simpson, DP and Gangardt, DM and Lerner, IV and Kr\"{u}ger, P},
	title        = {One-dimensional transport of bosons between weakly linked reservoirs},
	journal      = {Physical review letters},
	year         = 2014,
	volume       = 112,
	number       = 10,
	pages        = 100601,
}
@article{sinclair2005bose-einstein,
	author       = {Sinclair, C. D. J. and Curtis, E. A. and Garcia, I. Llorente and Retter, J. A. and Hall, B. V. and Eriksson, S. and Sauer, B. E. and Hinds, E. A.},
	title        = {Bose-Einstein condensation on a permanent-magnet atom chip},
	journal      = {Physical Review A},
	year         = 2005,
	volume       = 72,
	pages        = {031603},
	month        = {Sep},
}
@article{Sinclair2005PRA,
	author       = {Sinclair, C. D. J. and Curtis, E. A. and Garcia, I. Llorente and Retter, J. A. and Hall, B. V. and Eriksson, S. and Sauer, B. E. and Hinds, E. A.},
	title        = {Bose-Einstein condensation on a permanent-magnet atom chip},
	journal      = {Physical Review A},
	year         = 2005,
	volume       = 72,
	pages        = {031603},
	month        = {Sep},
}
@article{Singh:2020aa,
	author       = {Singh, Vijay Pal and Luick, Niclas and Sobirey, Lennart and Mathey, Ludwig},
	title        = {Josephson junction dynamics in a two-dimensional ultracold Bose gas},
	journal      = {Phys. Rev. Research},
	year         = 2020,
	volume       = 2,
	pages        = {033298},
	month        = {Aug},
}
@article{singh2020josephson,
	author       = {Singh, Vijay Pal and Luick, Niclas and Sobirey, Lennart and Mathey, Ludwig},
	title        = {Josephson junction dynamics in a two-dimensional ultracold Bose gas},
	journal      = {Phys. Rev. Research},
	year         = 2020,
	volume       = 2,
	pages        = {033298},
	month        = {Aug},
}
@article{Smerzi:1997aa,
	author       = {Smerzi, A. and Fantoni, S. and Giovanazzi, S. and Shenoy, S. R.},
	title        = {Quantum Coherent Atomic Tunneling between Two Trapped Bose-Einstein Condensates},
	journal      = {Phys. Rev. Lett.},
	year         = 1997,
	volume       = 79,
	number       = 25,
	pages        = {4950--4953},
	month        = {Dec},
}
@article{smerzi1997quantum,
	author       = {Smerzi, Augusto and Fantoni, Stefano and Giovanazzi, Stefano and Shenoy, SR},
	title        = {Quantum coherent atomic tunneling between two trapped Bose-Einstein condensates},
	journal      = {Phys. Rev. Lett.},
	year         = 1997,
	volume       = 79,
	number       = 25,
	pages        = 4950,
	month        = {dec},
}
@article{solenov_qubit,
	author       = {Solenov, Dmitry and Mozyrsky, Dmitry},
	title        = {Macroscopic two-state systems in trapped atomic condensates},
	journal      = {Physical Review A},
	year         = 2010,
	volume       = 82,
	number       = 6,
	pages        = {061601},
}
@article{solenov2010macroscopic,
	author       = {Solenov, Dmitry and Mozyrsky, Dmitry},
	title        = {Macroscopic two-state systems in trapped atomic condensates},
	journal      = {Physical Review A},
	year         = 2010,
	volume       = 82,
	number       = 6,
	pages        = {061601},
}
@article{Sommer:2011uq,
	author       = {Sommer, Ariel and Ku, Mark and Roati, Giacomo and Zwierlein, Martin W.},
	title        = {Universal spin transport in a strongly interacting Fermi gas},
	journal      = {Nature},
	year         = 2011,
	volume       = 472,
	number       = 7342,
	pages        = {201--204},
	month        = {04},
}
@article{sommer2011universal,
	author       = {Sommer, Ariel and Ku, Mark and Roati, Giacomo and Zwierlein, Martin W.},
	title        = {Universal spin transport in a strongly interacting Fermi gas},
	journal      = {Nature},
	year         = 2011,
	volume       = 472,
	number       = 7342,
	pages        = {201--204},
	month        = {04},
}
@article{Spagnolli:2017aa,
	author       = {Spagnolli, G. and Semeghini, G. and Masi, L. and Ferioli, G. and Trenkwalder, A. and Coop, S. and Landini, M. and Pezz\`e, L. and Modugno, G. and Inguscio, M. and Smerzi, A. and Fattori, M.},
	title        = {Crossing Over from Attractive to Repulsive Interactions in a Tunneling Bosonic Josephson Junction},
	journal      = {Phys. Rev. Lett.},
	year         = 2017,
	volume       = 118,
	pages        = 230403,
	month        = {Jun},
}
@article{spagnolli2017crossing,
	author       = {Spagnolli, G. and Semeghini, G. and Masi, L. and Ferioli, G. and Trenkwalder, A. and Coop, S. and Landini, M. and Pezz\`e, L. and Modugno, G. and Inguscio, M. and Smerzi, A. and Fattori, M.},
	title        = {Crossing Over from Attractive to Repulsive Interactions in a Tunneling Bosonic Josephson Junction},
	journal      = {Phys. Rev. Lett.},
	year         = 2017,
	volume       = 118,
	pages        = 230403,
	month        = {Jun},
}
@article{spehner2021persistent,
	author       = {Spehner, Dominique and Morales-Molina, Luis and Reyes, Sebastian A},
	title        = {Persistent currents in Bose-Bose mixtures after an interspecies interaction quench},
	journal      = {New Journal of Physics},
	year         = 2021,
}
@article{Stadler:2012kx,
	author       = {Stadler, David and Krinner, Sebastian and Meineke, Jakob and Brantut, Jean-Philippe and Esslinger, Tilman},
	title        = {Observing the drop of resistance in the flow of a superfluid Fermi gas},
	journal      = {Nature},
	year         = 2012,
	volume       = 491,
	number       = 7426,
	pages        = {736--739},
	month        = 11,
}
@article{stadler2012observing,
	author       = {Stadler, David and Krinner, Sebastian and Meineke, Jakob and Brantut, Jean-Philippe and Esslinger, Tilman},
	title        = {Observing the drop of resistance in the flow of a superfluid Fermi gas},
	journal      = {Nature},
	year         = 2012,
	volume       = 491,
	number       = 7426,
	pages        = 736,
	month        = 11,
}
@article{Stevenson2015PRL,
	author       = {Stevenson, R. and Hush, Michael R. and Bishop, Thomas and Lesanovsky, I. and Fernholz, Thomas},
	title        = {Sagnac Interferometry with a Single Atomic Clock},
	journal      = {Physical Review Letters},
	year         = 2015,
	volume       = 115,
	pages        = 163001,
	month        = {Oct},
}
@article{stevenson2015sagnac,
	author       = {Stevenson, R. and Hush, Michael R. and Bishop, Thomas and Lesanovsky, I. and Fernholz, Thomas},
	title        = {Sagnac Interferometry with a Single Atomic Clock},
	journal      = {Physical Review Letters},
	year         = 2015,
	volume       = 115,
	pages        = 163001,
	month        = {Oct},
}
@article{stickney2007transistorlike,
	author       = {Stickney, James A and Anderson, Dana Z and Zozulya, Alex A},
	title        = {Transistorlike behavior of a Bose-Einstein condensate in a triple-well potential},
	journal      = {Physical Review A},
	year         = 2007,
	volume       = 75,
	number       = 1,
	pages        = {013608},
	month        = {Jan},
}
@article{stockton2011absolute,
	author       = {Stockton, JK and Takase, K and Kasevich, MA},
	title        = {Absolute geodetic rotation measurement using atom interferometry},
	journal      = {Phys. Rev. Lett.},
	year         = 2011,
	volume       = 107,
	number       = 13,
	pages        = 133001,
}
@article{sugarbakeratom,
	author       = {Sugarbaker, Alex and Dickerson, Susannah M and Hogan, Jason M and Johnson, David MS and Kasevich, Mark A},
	title        = {Atom Interferometry in a 10 Meter Atomic Fountain},
}
@article{Sun2018PRA,
	author       = {Sun, Kuei and Padavi{\'{c}}, Karmela and Yang, Frances and Vishveshwara, Smitha and Lannert, Courtney},
	title        = {Static and dynamic properties of shell-shaped condensates},
	journal      = {Physical Review A},
	year         = 2018,
	volume       = 98,
	number       = 1,
	month        = {jul},
}
@article{sun2018static,
	author       = {Sun, Kuei and Padavi{\'{c}}, Karmela and Yang, Frances and Vishveshwara, Smitha and Lannert, Courtney},
	title        = {Static and dynamic properties of shell-shaped condensates},
	journal      = {Physical Review A},
	year         = 2018,
	volume       = 98,
	number       = 1,
	month        = {jul},
}
@article{sutherland1968further,
	author       = {Sutherland, Bill},
	title        = {Further results for the many-body problem in one dimension},
	journal      = {Phys. Rev. Lett.},
	year         = 1968,
	volume       = 20,
	number       = 3,
	pages        = 98,
}
@article{sutherland1975model,
	author       = {Sutherland, Bill},
	title        = {Model for a multicomponent quantum system},
	journal      = {Phys. Rev. B},
	year         = 1975,
	volume       = 12,
	pages        = {3795--3805},
	month        = {Nov},
}
@article{thouless1982quantized,
	author       = {Thouless, David J and Kohmoto, Mahito and Nightingale, M Peter and den Nijs, Md},
	title        = {Quantized Hall conductance in a two-dimensional periodic potential},
	journal      = {Phys. Rev. Lett.},
	year         = 1982,
	volume       = 49,
	number       = 6,
	pages        = 405,
}
@article{thouless1983quantization,
	author       = {Thouless, DJ},
	title        = {Quantization of particle transport},
	journal      = {Phys. Rev. B},
	year         = 1983,
	volume       = 27,
	number       = 10,
	pages        = 6083,
}
@book{Tinkham2012introduction,
	title        = {Introduction to superconductivity},
	publisher    = {Courier Dover Publications},
	year         = 2012,
	author       = {Tinkham, Michael},
}
@book{tinkham2012introduction,
	title        = {Introduction to superconductivity},
	publisher    = {Courier Dover Publications},
	year         = 2012,
	author       = {Tinkham, Michael},
}
@article{tokuno2008dynamics,
	author       = {Tokuno, Akiyuki and Oshikawa, Masaki and Demler, Eugene},
	title        = {Dynamics of one-dimensional Bose liquids: Andreev-like reflection at Y junctions and the absence of the Aharonov-Bohm effect},
	journal      = {Phys. Rev. Lett.},
	year         = 2008,
	volume       = 100,
	number       = 14,
	pages        = 140402,
}
@article{Tollett1995Permanent,
	author       = {Tollett, J. J. and Bradley, C. C. and Sackett, C. A. and Hulet, R. G.},
	title        = {Permanent magnet trap for cold atoms},
	journal      = {Phys. Rev. A},
	year         = 1995,
	volume       = 51,
	pages        = {R22--R25},
	month        = {Jan},
}
@article{tollett1995permanent,
	author       = {Tollett, J. J. and Bradley, C. C. and Sackett, C. A. and Hulet, R. G.},
	title        = {Permanent magnet trap for cold atoms},
	journal      = {Phys. Rev. A},
	year         = 1995,
	volume       = 51,
	pages        = {R22--R25},
	month        = {Jan},
}
@article{tononi2020dephasing,
  title={Dephasing--rephasing dynamics of one-dimensional tunneling quasicondensates},
  author={Tononi, Andrea and Toigo, Flavio and Wimberger, Sandro and Cappellaro, Alberto and Salasnich, Luca},
  journal={New Journal of Physics},
  volume={22},
  number={7},
  pages={073020},
  year={2020},
  publisher={IOP Publishing}
}

@article{tosto2019optically,
	author       = {Tosto, Francesca and Baw Swe, Phyo and Nguyen, Nghia Tin and Hufnagel, Christoph and Mart\'{\i}nez Valado, Mar\'{\i}a and Prigozhin, Leonid and Sokolovsky, Vladimir and Dumke, Rainer},
	title        = {Optically tailored trapping geometries for ultracold atoms on a type-II superconducting chip},
	journal      = {Applied Physics Letters},
	year         = 2019,
	volume       = 114,
	number       = 22,
	pages        = 222601,
}
@article{trebbia2007roughness,
	author       = {Trebbia, J.-B. and Garrido Alzar, C. L. and Cornelussen, R. and Westbrook, C. I. and Bouchoule, I.},
	title        = {Roughness Suppression via Rapid Current Modulation on an Atom Chip},
	journal      = {Phys. Rev. Lett.},
	year         = 2007,
	volume       = 98,
	pages        = 263201,
	month        = {Jun},
}
@article{Trenkwalder:2016aa,
	author       = {Trenkwalder, A. and Spagnolli, G. and Semeghini, G. and Coop, S. and Landini, M. and Castilho, P. and Pezz\`{e}, L. and Modugno, G. and Inguscio, M. and Smerzi, A. and Fattori, M.},
	title        = {Quantum phase transitions with parity-symmetry breaking and hysteresis},
	journal      = {Nature Physics},
	year         = 2016,
	volume       = 12,
	number       = 9,
	pages        = {826--829},
}
@article{trenkwalder2016quantum,
	author       = {Trenkwalder, A. and Spagnolli, G. and Semeghini, G. and Coop, S. and Landini, M. and Castilho, P. and Pezz\`{e}, L. and Modugno, G. and Inguscio, M. and Smerzi, A. and Fattori, M.},
	title        = {Quantum phase transitions with parity-symmetry breaking and hysteresis},
	journal      = {Nature Physics},
	year         = 2016,
	volume       = 12,
	number       = 9,
	pages        = {826--829},
}
@article{truscott2001observation,
	author       = {Truscott, Andrew G and Strecker, Kevin E and McAlexander, William I and Partridge, Guthrie B and Hulet, Randall G},
	title        = {Observation of Fermi pressure in a gas of trapped atoms},
	journal      = {Science},
	year         = 2001,
	volume       = 291,
	number       = 5513,
	pages        = {2570--2572},
}
@article{turpin2015blue,
	author       = {Turpin, A. and Polo, J. and Loiko, Yu V. and K\"{u}ber, J. and Schmaltz, F. and Kalkandjiev, T. K. and Ahufinger, V. and Birkl, G. and Mompart, J.},
	title        = {Blue-detuned optical ring trap for Bose-Einstein condensates based on conical refraction},
	journal      = {Optics Express},
	year         = 2015,
	volume       = 23,
	number       = 2,
	pages        = {1638--1650},
	month        = {Jan},
}
@article{turpin2015blue-detuned,
	author       = {Turpin, A. and Polo, J. and Loiko, Yu V. and K\"{u}ber, J. and Schmaltz, F. and Kalkandjiev, T. K. and Ahufinger, V. and Birkl, G. and Mompart, J.},
	title        = {Blue-detuned optical ring trap for Bose-Einstein condensates based on conical refraction},
	journal      = {Optics Express},
	year         = 2015,
	volume       = 23,
	number       = 2,
	pages        = {1638--1650},
	month        = {Jan},
}
@article{uchino2019bosonic,
	author       = {Uchino, Shun and Brantut, Jean-Philippe},
	title        = {Bosonic superfluid transport in a quantum point contact},
	journal      = {arXiv preprint arXiv:1906.09191},
	year         = 2019,
}
@article{Uchino:2020aa,
	author       = {Uchino, Shun and Brantut, Jean-Philippe},
	title        = {Bosonic superfluid transport in a quantum point contact},
	journal      = {Phys. Rev. Research},
	year         = 2020,
	volume       = 2,
	pages        = {023284},
	month        = {Jun},
}
@article{uchino2020bosonic,
	author       = {Uchino, Shun and Brantut, Jean-Philippe},
	title        = {Bosonic superfluid transport in a quantum point contact},
	journal      = {Phys. Rev. Research},
	year         = 2020,
	volume       = 2,
	pages        = {023284},
	month        = {Jun},
}
@article{Uchino:2018ab,
	author       = {Uchino, Shun and Ueda, Masahito and Brantut, Jean-Philippe},
	title        = {Universal noise in continuous transport measurements of interacting fermions},
	journal      = {Phys. Rev. A},
	year         = 2018,
	volume       = 98,
	pages        = {063619},
	month        = {Dec},
}
@article{uchino2018universal,
	author       = {Uchino, Shun and Ueda, Masahito and Brantut, Jean-Philippe},
	title        = {Universal noise in continuous transport measurements of interacting fermions},
	journal      = {Phys. Rev. A},
	year         = 2018,
	volume       = 98,
	pages        = {063619},
	month        = {Dec},
}
@article{Uchino:2017aa,
	author       = {Uchino, Shun and Ueda, Masahito},
	title        = {Anomalous Transport in the Superfluid Fluctuation Regime},
	journal      = {Phys. Rev. Lett.},
	year         = 2017,
	volume       = 118,
	pages        = 105303,
	month        = {Mar},
}
@article{uchino2017anomalous,
	author       = {Uchino, Shun and Ueda, Masahito},
	title        = {Anomalous Transport in the Superfluid Fluctuation Regime},
	journal      = {Phys. Rev. Lett.},
	year         = 2017,
	volume       = 118,
	pages        = 105303,
	month        = {Mar},
}
@article{Uchino:2020ab,
	author       = {Uchino, Shun},
	title        = {Role of Nambu-Goldstone modes in the fermionic-superfluid point contact},
	journal      = {Phys. Rev. Research},
	year         = 2020,
	volume       = 2,
	pages        = {023340},
	month        = {Jun},
}
@article{uchino2020role,
	author       = {Uchino, Shun},
	title        = {Role of Nambu-Goldstone modes in the fermionic-superfluid point contact},
	journal      = {Phys. Rev. Research},
	year         = 2020,
	volume       = 2,
	pages        = {023340},
	month        = {Jun},
}
@article{AB_fundations_Vaidman,
	author       = {Vaidman, Lev},
	title        = {Role of potentials in the Aharonov-Bohm effect},
	journal      = {Phys. Rev. A},
	year         = 2012,
	volume       = 86,
	pages        = {040101},
	month        = {Oct},
}
@article{vaidman2012role,
	author       = {Vaidman, Lev},
	title        = {Role of potentials in the Aharonov-Bohm effect},
	journal      = {Phys. Rev. A},
	year         = 2012,
	volume       = 86,
	pages        = {040101},
	month        = {Oct},
}
@article{Valtolina:2017aa,
	author       = {Valtolina, G. and Scazza, F. and Amico, A. and Burchianti, A. and Recati, A. and Enss, T. and Inguscio, M. and Zaccanti, M. and Roati, G.},
	title        = {Exploring the ferromagnetic behaviour of a repulsive Fermi gas through spin dynamics},
	journal      = {Nat Phys},
	year         = 2017,
	volume       = 13,
	number       = 7,
	pages        = {704--709},
	month        = {07},
}
@article{valtolina2017exploring,
	author       = {Valtolina, G. and Scazza, F. and Amico, A. and Burchianti, A. and Recati, A. and Enss, T. and Inguscio, M. and Zaccanti, M. and Roati, G.},
	title        = {Exploring the ferromagnetic behaviour of a repulsive Fermi gas through spin dynamics},
	journal      = {Nat Phys},
	year         = 2017,
	volume       = 13,
	number       = 7,
	pages        = {704--709},
	month        = {07},
}
@article{Valtolina:2015ab,
	author       = {Valtolina, Giacomo and Burchianti, Alessia and Amico, Andrea and Neri, Elettra and Xhani, Klejdja and Seman, Jorge Amin and Trombettoni, Andrea and Smerzi, Augusto and Zaccanti, Matteo and Inguscio, Massimo and Roati, Giacomo},
	title        = {Josephson effect in fermionic superfluids across the BEC-BCS crossover},
	journal      = {Science},
	year         = 2015,
	volume       = 350,
	number       = 6267,
	pages        = {1505--1508},
	month        = 12,
}
@article{valtolina2015josephson,
	author       = {Valtolina, Giacomo and Burchianti, Alessia and Amico, Andrea and Neri, Elettra and Xhani, Klejdja and Seman, Jorge Amin and Trombettoni, Andrea and Smerzi, Augusto and Zaccanti, Matteo and Inguscio, Massimo and Roati, Giacomo},
	title        = {Josephson effect in fermionic superfluids across the BEC-BCS crossover},
	journal      = {Science},
	year         = 2015,
	volume       = 350,
	number       = 6267,
	pages        = {1505--1508},
}
@article{Wees:1988aa,
	author       = {van Wees, B. J. and van Houten, H. and Beenakker, C. W. J. and Williamson, J. G. and Kouwenhoven, L. P. and van der Marel, D. and Foxon, C. T.},
	title        = {Quantized conductance of point contacts in a two-dimensional electron gas},
	journal      = {Phys. Rev. Lett.},
	year         = 1988,
	volume       = 60,
	pages        = {848--850},
	month        = {Feb},
}
@article{wees1988quantized,
	author       = {van Wees, B. J. and van Houten, H. and Beenakker, C. W. J. and Williamson, J. G. and Kouwenhoven, L. P. and van der Marel, D. and Foxon, C. T.},
	title        = {Quantized conductance of point contacts in a two-dimensional electron gas},
	journal      = {Phys. Rev. Lett.},
	year         = 1988,
	volume       = 60,
	pages        = {848--850},
	month        = {Feb},
}
@article{van2010bose,
	author       = {van Zoest, Tim and Gaaloul, N and Singh, Y and Ahlers, H and Herr, W and Seidel, ST and Ertmer, W and Rasel, E and Eckart, Michael and Kajari, Endre and others},
	title        = {Bose-Einstein condensation in microgravity},
	journal      = {Science},
	year         = 2010,
	volume       = 328,
	number       = 5985,
	pages        = {1540--1543},
}
@article{zoest2010bose-einstein,
	author       = {van Zoest, Tim and Gaaloul, N and Singh, Y and Ahlers, H and Herr, W and Seidel, ST and Ertmer, W and Rasel, E and Eckart, Michael and Kajari, Endre and others},
	title        = {Bose-Einstein condensation in microgravity},
	journal      = {Science},
	year         = 2010,
	volume       = 328,
	number       = 5985,
	pages        = {1540--1543},
}
@article{verdu2009strong,
	author       = {Verd\'{u}, J and Zoubi, H and Koller, Ch and Majer, J and Ritsch, H and Schmiedmayer, J},
	title        = {Strong magnetic coupling of an ultracold gas to a superconducting waveguide cavity},
	journal      = {Phys. Rev. Lett.},
	year         = 2009,
	volume       = 103,
	number       = 4,
	pages        = {043603},
	month        = {Jul},
}
@article{victorin2019nonclassical,
	author       = {Victorin, Nicolas and Haug, Tobias and Kwek, Leong-Chuan and Amico, Luigi and Minguzzi, Anna},
	title        = {Nonclassical states in strongly correlated bosonic ring ladders},
	journal      = {Physical Review A},
	year         = 2019,
	volume       = 99,
	number       = 3,
	pages        = {033616},
}
@article{victorin2018bosonic,
	author       = {Victorin, Nicolas and Hekking, Frank and Minguzzi, Anna},
	title        = {Bosonic double ring lattice under artificial gauge fields},
	journal      = {Phys. Rev. A},
	year         = 2018,
	volume       = 98,
	pages        = 053626,
	month        = {Nov},
}
@article{waintal2008persistent,
	author       = {Waintal, Xavier and Fleury, Genevieve and Kazymyrenko, Kyryl and Houzet, Manuel and Schmitteckert, Peter and Weinmann, Dietmar},
	title        = {Persistent currents in one dimension: the counterpart of {L}eggett's theorem},
	journal      = {Phys. Rev. Lett.},
	year         = 2008,
	volume       = 101,
	number       = 10,
	pages        = 106804,
}
@article{wang2015resonant,
	author       = {Wang, Yi-Hsieh and Kumar, A and Jendrzejewski, F and Wilson, Ryan M and Edwards, Mark and Eckel, S and Campbell, G K and Clark, Charles W},
	title        = {Resonant wavepackets and shock waves in an atomtronic SQUID},
	journal      = {New Journal of Physics},
	year         = 2015,
	volume       = 17,
	pages        = 125012,
}
@article{wang2005atom,
	author       = {Wang, Ying-Ju and Anderson, Dana Z. and Bright, Victor M. and Cornell, Eric A. and Diot, Quentin and Kishimoto, Tetsuo and Prentiss, Mara and Saravanan, R. A. and Segal, Stephen R. and Wu, Saijun},
	title        = {Atom Michelson Interferometer on a Chip Using a Bose-Einstein Condensate},
	journal      = {Physical Review Letters},
	year         = 2005,
	volume       = 94,
	number       = 9,
	pages        = {090405},
	month        = 3,
}
@article{watabe2008reflection,
	author       = {Watabe, Shohei and Kato, Yusuke},
	title        = {Reflection and refraction of Bose-Einstein-condensate excitations},
	journal      = {Phys. Rev. A},
	year         = 2008,
	volume       = 78,
	number       = 6,
	pages        = {063611},
}
@article{webb1985observation,
	author       = {Webb, Richard A and Washburn, Simon and Umbach, CP and Laibowitz, RB},
	title        = {Observation of h/e Aharonov-Bohm oscillations in normal-metal rings},
	journal      = {Phys. Rev. Lett.},
	year         = 1985,
	volume       = 54,
	number       = 25,
	pages        = 2696,
}
@article{weiss2009creation,
	author       = {Weiss, Christoph and Castin, Yvan},
	title        = {Creation and detection of a mesoscopic gas in a nonlocal quantum superposition},
	journal      = {Phys. Rev. Lett.},
	year         = 2009,
	volume       = 102,
	number       = 1,
	pages        = {010403},
	month        = {Jan},
}
@article{Wharam:1988aa,
	author       = {Wharam, D A and Thornton, T J and Newbury, R and Pepper, M and Ahmed, H and Frost, J E F and Hasko, D G and Peacock, D C and Ritchie, D A and Jones, G A C},
	title        = {One-dimensional transport and the quantisation of the ballistic resistance},
	journal      = {Journal of Physics C: Solid State Physics},
	year         = 1988,
	volume       = 21,
	number       = 8,
	pages        = {L209},
}
@article{wharam1988one-dimensional,
	author       = {Wharam, D A and Thornton, T J and Newbury, R and Pepper, M and Ahmed, H and Frost, J E F and Hasko, D G and Peacock, D C and Ritchie, D A and Jones, G A C},
	title        = {One-dimensional transport and the quantisation of the ballistic resistance},
	journal      = {Journal of Physics C: Solid State Physics},
	year         = 1988,
	volume       = 21,
	number       = 8,
	pages        = {L209},
}
@article{White:2019aa,
	author       = {White, Donald H and Haase, Thomas A and Brown, Dylan J and Hoogerland, Maarten D and Najafabadi, Mojdeh S and Helm, John L and Gies, Christopher and Schumayer, Daniel and Hutchinson, David AW},
	title        = {Observation of two-dimensional Anderson localisation of ultracold atoms},
	journal      = {arXiv preprint arXiv:1911.04858},
	year         = 2019,
}
@article{white2019observation,
	author       = {White, Donald H and Haase, Thomas A and Brown, Dylan J and Hoogerland, Maarten D and Najafabadi, Mojdeh S and Helm, John L and Gies, Christopher and Schumayer, Daniel and Hutchinson, David AW},
	title        = {Observation of two-dimensional Anderson localisation of ultracold atoms},
	journal      = {arXiv preprint arXiv:1911.04858},
	year         = 2019,
}
@article{wright2000toroidal,
	author       = {Wright, EM and Arlt, Jochen and Dholakia, K},
	title        = {Toroidal optical dipole traps for atomic Bose-Einstein condensates using Laguerre-Gaussian beams},
	journal      = {Physical Review A},
	year         = 2000,
	volume       = 63,
	number       = 1,
	pages        = {013608},
	month        = {Dec},
}
@article{wright_driving_2013,
	author       = {Wright, K. C. and Blakestad, R. B. and Lobb, C. J. and Phillips, W. D. and Campbell, G. K.},
	title        = {Driving {Phase} {Slips} in a {Superfluid} {Atom} {Circuit} with a {Rotating} {Weak} {Link}},
	journal      = {Phys. Rev. Lett.},
	year         = 2013,
	volume       = 110,
	number       = 2,
	pages        = {025302},
	month        = jan,
}
@article{Wright:2013aa,
	author       = {Wright, K. C. and Blakestad, R. B. and Lobb, C. J. and Phillips, W. D. and Campbell, G. K.},
	title        = {Driving Phase Slips in a Superfluid Atom Circuit with a Rotating Weak Link},
	journal      = {Phys. Rev. Lett.},
	year         = 2013,
	volume       = 110,
	pages        = {025302},
	month        = {Jan},
}
@article{wright2013driving,
	author       = {Wright, K. C. and Blakestad, R. B. and Lobb, C. J. and Phillips, W. D. and Campbell, G. K.},
	title        = {Driving Phase Slips in a Superfluid Atom Circuit with a Rotating Weak Link},
	journal      = {Phys. Rev. Lett.},
	year         = 2013,
	volume       = 110,
	number       = 2,
	pages        = {025302},
	month        = {Jan},
}
@article{wright2013threshold,
	author       = {Wright, K. C. and Blakestad, R. B. and Lobb, C. J. and Phillips, W. D. and Campbell, G. K.},
	title        = {Threshold for creating excitations in a stirred superfluid ring},
	journal      = {Phys. Rev. A},
	year         = 2013,
	volume       = 88,
	number       = 6,
	pages        = {063633},
	month        = {Dec},
}
@article{wu2007demonstration,
	author       = {Wu, Saijun and Su, Edward and Prentiss, Mara},
	title        = {Demonstration of an area-enclosing guided-atom interferometer for rotation sensing},
	journal      = {Phys. Rev. Lett.},
	year         = 2007,
	volume       = 99,
	number       = 17,
	month        = {OCT 26},
}
@article{Wu2007PRL,
	author       = {Wu, Saijun and Su, Edward and Prentiss, Mara},
	title        = {Demonstration of an area-enclosing guided-atom interferometer for rotation sensing},
	journal      = {Phys. Rev. Lett.},
	year         = 2007,
	volume       = 99,
	number       = 17,
	month        = {OCT 26},
}
@article{wu2005splitting,
	author       = {Wu, Saijun and Wang, Ying-Ju and Diot, Quentin and Prentiss, Mara},
	title        = {Splitting matter waves using an optimized standing-wave light-pulse sequence},
	journal      = {Physical Review A},
	year         = 2005,
	volume       = 71,
	number       = 4,
	pages        = {043602},
}
@article{Xhani:2020aa,
	author       = {Xhani, K. and Neri, E. and Galantucci, L. and Scazza, F. and Burchianti, A. and Lee, K.-L. and Barenghi, C. F. and Trombettoni, A. and Inguscio, M. and Zaccanti, M. and Roati, G. and Proukakis, N. P.},
	title        = {Critical Transport and Vortex Dynamics in a Thin Atomic Josephson Junction},
	journal      = {Phys. Rev. Lett.},
	year         = 2020,
	volume       = 124,
	pages        = {045301},
	month        = {Jan},
}
@article{xhani2020critical,
	author       = {Xhani, K. and Neri, E. and Galantucci, L. and Scazza, F. and Burchianti, A. and Lee, K.-L. and Barenghi, C. F. and Trombettoni, A. and Inguscio, M. and Zaccanti, M. and Roati, G. and Proukakis, N. P.},
	title        = {Critical Transport and Vortex Dynamics in a Thin Atomic Josephson Junction},
	journal      = {Phys. Rev. Lett.},
	year         = 2020,
	volume       = 124,
	pages        = {045301},
	month        = {Jan},
}
@article{xiang_hybrid_2013,
	author       = {Xiang, Ze-Liang and Ashhab, Sahel and You, J. Q. and Nori, Franco},
	title        = {Hybrid quantum circuits: {Superconducting} circuits interacting with other quantum systems},
	journal      = {Rev. Mod. Phys.},
	year         = 2013,
	volume       = 85,
	number       = 2,
	pages        = {623--653},
	month        = apr,
}
@article{xiang2013hybrid,
	author       = {Xiang, Ze-Liang and Ashhab, Sahel and You, J. Q. and Nori, Franco},
	title        = {Hybrid quantum circuits: {Superconducting} circuits interacting with other quantum systems},
	journal      = {Rev. Mod. Phys.},
	year         = 2013,
	volume       = 85,
	number       = 2,
	pages        = {623--653},
	month        = apr,
}
@article{Yao:2018aa,
	author       = {Yao, Juan and Liu, Boyang and Sun, Mingyuan and Zhai, Hui},
	title        = {Controlled transport between Fermi superfluids through a quantum point contact},
	journal      = {Phys. Rev. A},
	year         = 2018,
	volume       = 98,
	pages        = {041601},
	month        = {Oct},
}
@article{yao2018controlled,
	author       = {Yao, Juan and Liu, Boyang and Sun, Mingyuan and Zhai, Hui},
	title        = {Controlled transport between Fermi superfluids through a quantum point contact},
	journal      = {Phys. Rev. A},
	year         = 2018,
	volume       = 98,
	pages        = {041601},
	month        = {Oct},
}
@article{You:2019aa,
	author       = {You, Jhih-Shih and Schmidt, Richard and Ivanov, Dmitri A. and Knap, Michael and Demler, Eugene},
	title        = {Atomtronics with a spin: Statistics of spin transport and nonequilibrium orthogonality catastrophe in cold quantum gases},
	journal      = {Phys. Rev. B},
	year         = 2019,
	volume       = 99,
	pages        = 214505,
	month        = {Jun},
}
@article{you2019atomtronics,
	author       = {You, Jhih-Shih and Schmidt, Richard and Ivanov, Dmitri A. and Knap, Michael and Demler, Eugene},
	title        = {Atomtronics with a spin: Statistics of spin transport and nonequilibrium orthogonality catastrophe in cold quantum gases},
	journal      = {Phys. Rev. B},
	year         = 2019,
	volume       = 99,
	pages        = 214505,
	month        = {Jun},
}
@article{yu2017superconducting,
	author       = {Yu, Deshui and Kwek, Leong Chuan and Amico, Luigi and Dumke, Rainer},
	title        = {Superconducting qubit-resonator-atom hybrid system},
	journal      = {Quantum Science and Technology},
	year         = 2017,
	volume       = 2,
	number       = 3,
	pages        = {035005},
	month        = {jul},
}
@article{yu2017theoretical,
	author       = {Yu, Deshui and Kwek, Leong Chuan and Amico, Luigi and Dumke, Rainer},
	title        = {Theoretical description of a micromaser in the ultrastrong-coupling regime},
	journal      = {Physical Review A},
	year         = 2017,
	volume       = 95,
	number       = 5,
	pages        = {053811},
}
@article{yu2018charge,
	author       = {Yu, Deshui and Kwek, Leong Chuan and Amico, Luigi and Dumke, Rainer},
	title        = {Charge-Qubit-Resonator-Interface-Based Nonlinear Circuit QED},
	journal      = {arXiv preprint arXiv:1809.06542},
	year         = 2018,
}
@article{yu2018charge-qubit-resonator-interface-based,
	author       = {Yu, Deshui and Kwek, Leong Chuan and Amico, Luigi and Dumke, Rainer},
	title        = {Charge-Qubit-Resonator-Interface-Based Nonlinear Circuit QED},
	journal      = {arXiv preprint arXiv:1809.06542},
	year         = 2018,
}
@article{yu2018stabilizing,
	author       = {Yu, Deshui and Landra, Alessandro and Kwek, Leong Chuan and Amico, Luigi and Dumke, Rainer},
	title        = {Stabilizing Rabi oscillation of a charge qubit via the atomic clock technique},
	journal      = {New Journal of Physics},
	year         = 2018,
	volume       = 20,
	number       = 2,
	pages        = {023031},
}
@article{yu2016superconducting,
	author       = {Yu, Deshui and Landra, Alessandro and Valado, Mar\'{\i}a Mart\'{\i}nez and Hufnagel, Christoph and Kwek, Leong Chuan and Amico, Luigi and Dumke, Rainer},
	title        = {Superconducting resonator and Rydberg atom hybrid system in the strong coupling regime},
	journal      = {Physical Review A},
	year         = 2016,
	volume       = 94,
	number       = 6,
	pages        = {062301},
	month        = {Dec},
}
@article{yu2016charge,
	author       = {Yu, Deshui and Valado, Mar\'{\i}a Mart\'{\i}nez and Hufnagel, Christoph and Kwek, Leong Chuan and Amico, Luigi and Dumke, Rainer},
	title        = {Charge-qubit--atom hybrid},
	journal      = {Physical Review A},
	year         = 2016,
	volume       = 93,
	number       = 4,
	pages        = {042329},
	month        = {Apr},
}
@article{yu2016charge-qubit--atom,
	author       = {Yu, Deshui and Valado, Mar\'{\i}a Mart\'{\i}nez and Hufnagel, Christoph and Kwek, Leong Chuan and Amico, Luigi and Dumke, Rainer},
	title        = {Charge-qubit--atom hybrid},
	journal      = {Physical Review A},
	year         = 2016,
	volume       = 93,
	number       = 4,
	pages        = {042329},
	month        = {Apr},
}
@article{yu2016quantum,
	author       = {Yu, Deshui and Valado, Mar\'{\i}a Mart\'{\i}nez and Hufnagel, Christoph and Kwek, Leong Chuan and Amico, Luigi and Dumke, Rainer},
	title        = {Quantum state transmission in a superconducting charge qubit-atom hybrid},
	journal      = {Scientific reports},
	year         = 2016,
	volume       = 6,
	pages        = 38356,
	month        = {Dec},
}
@article{yu1992persistent,
	author       = {Yu, Naichang and Fowler, Michael},
	title        = {Persistent current of a Hubbard ring threaded with a magnetic flux},
	journal      = {Phys. Rev. B},
	year         = 1992,
	volume       = 45,
	pages        = {11795--11804},
	month        = {May},
}
@article{Zollner:2008aa,
	author       = {Z\"ollner, Sascha and Meyer, Hans-Dieter and Schmelcher, Peter},
	title        = {Few-Boson Dynamics in Double Wells: From Single-Atom to Correlated Pair Tunneling},
	journal      = {Phys. Rev. Lett.},
	year         = 2008,
	volume       = 100,
	pages        = {040401},
	month        = {Jan},
}
@article{zollner2008few-boson,
	author       = {Z\"ollner, Sascha and Meyer, Hans-Dieter and Schmelcher, Peter},
	title        = {Few-Boson Dynamics in Double Wells: From Single-Atom to Correlated Pair Tunneling},
	journal      = {Phys. Rev. Lett.},
	year         = 2008,
	volume       = 100,
	pages        = {040401},
	month        = {Jan},
}
@article{zabow2004coherent,
	author       = {Zabow, G. and Conroy, R. S. and Prentiss, M. G.},
	title        = {Coherent matter-wave manipulation in the diabatic limit},
	journal      = {Phys. Rev. Lett.},
	year         = 2004,
	volume       = 92,
	number       = 18,
	pages        = 180404,
	month        = {May},
}
@article{Zabow2004PRL,
	author       = {Zabow, G. and Conroy, R. S. and Prentiss, M. G.},
	title        = {Coherent matter-wave manipulation in the diabatic limit},
	journal      = {Phys. Rev. Lett.},
	year         = 2004,
	volume       = 92,
	number       = 18,
	pages        = 180404,
	month        = {May},
}
@article{Zaccanti:2019aa,
	author       = {Zaccanti, M. and Zwerger, W.},
	title        = {Critical Josephson current in BCS-BEC--crossover superfluids},
	journal      = {Phys. Rev. A},
	year         = 2019,
	volume       = 100,
	pages        = {063601},
	month        = {Dec},
}
@article{zaccanti2019critical,
	author       = {Zaccanti, M. and Zwerger, W.},
	title        = {Critical Josephson current in BCS-BEC--crossover superfluids},
	journal      = {Phys. Rev. A},
	year         = 2019,
	volume       = 100,
	pages        = {063601},
	month        = {Dec},
}
@article{zapata2009andreev,
	author       = {Zapata, I and Sols, F},
	title        = {Andreev reflection in bosonic condensates},
	journal      = {Phys. Rev. Lett.},
	year         = 2009,
	volume       = 102,
	number       = 18,
	pages        = 180405,
}
@article{Zapata:1998aa,
	author       = {Zapata, Ivar and Sols, Fernando and Leggett, Anthony J.},
	title        = {Josephson effect between trapped Bose-Einstein condensates},
	journal      = {Phys. Rev. A},
	year         = 1998,
	volume       = 57,
	pages        = {R28--R31},
	month        = {Jan},
}
@article{zapata1998josephson,
	author       = {Zapata, Ivar and Sols, Fernando and Leggett, Anthony J.},
	title        = {Josephson effect between trapped Bose-Einstein condensates},
	journal      = {Phys. Rev. A},
	year         = 1998,
	volume       = 57,
	pages        = {R28--R31},
	month        = {Jan},
}
@article{PhysRevA.85.013404,
	author       = {Zhang, B. and Siercke, M. and Chan, K. S. and Beian, M. and Lim, M. J. and Dumke, R.},
	title        = {Magnetic confinement of neutral atoms based on patterned vortex distributions in superconducting disks and rings},
	journal      = {Phys. Rev. A},
	year         = 2012,
	volume       = 85,
	pages        = {013404},
	month        = {Jan},
}
@article{zhang2012magnetic,
	author       = {Zhang, B. and Siercke, M. and Chan, K. S. and Beian, M. and Lim, M. J. and Dumke, R.},
	title        = {Magnetic confinement of neutral atoms based on patterned vortex distributions in superconducting disks and rings},
	journal      = {Phys. Rev. A},
	year         = 2012,
	volume       = 85,
	pages        = {013404},
	month        = {Jan},
}
@article{Zobay2001PRL,
	author       = {Zobay, O. and Garraway, B. M.},
	title        = {Two-Dimensional Atom Trapping in Field-Induced Adiabatic Potentials},
	journal      = {Phys. Rev. Lett.},
	year         = 2001,
	volume       = 86,
	number       = 7,
	pages        = {1195--1198},
	month        = 3,
}
@article{zobay2001two-dimensional,
	author       = {Zobay, O. and Garraway, B. M.},
	title        = {Two-Dimensional Atom Trapping in Field-Induced Adiabatic Potentials},
	journal      = {Phys. Rev. Lett.},
	year         = 2001,
	volume       = 86,
	number       = 7,
	pages        = {1195--1198},
	month        = 3,
}
@article{Zozulya.20134s8,
	author       = {Zozulya, Alex A and Anderson, Dana Z.},
	title        = {Principles of an atomtronic battery},
	journal      = {Physical Review A},
	year         = 2013,
	volume       = 88,
	number       = 4,
}
@article{zozulya2013principles,
	author       = {Zozulya, Alex A and Anderson, Dana Z.},
	title        = {Principles of an atomtronic battery},
	journal      = {Physical Review A},
	year         = 2013,
	volume       = 88,
	number       = 4,
}

@article{zupancic2016ultra,
	author       = {Zupancic, Philip and Preiss, Philipp M and Ma, Ruichao and Lukin, Alexander and Tai, M Eric and Rispoli, Matthew and Islam, Rajibul and Greiner, Markus},
	title        = {Ultra-precise holographic beam shaping for microscopic quantum control},
	journal      = {Optics express},
	year         = 2016,
	volume       = 24,
	number       = 13,
	pages        = {13881--13893},
}

@article{zupancic2016ultra-precise,
	author       = {Zupancic, Philip and Preiss, Philipp M and Ma, Ruichao and Lukin, Alexander and Tai, M Eric and Rispoli, Matthew and Islam, Rajibul and Greiner, Markus},
	title        = {Ultra-precise holographic beam shaping for microscopic quantum control},
	journal      = {Optics express},
	year         = 2016,
	volume       = 24,
	number       = 13,
	pages        = {13881--13893},
}
@article{zvyagin1995persistent,
	author       = {Zvyagin, A. A. and Krive, I. V.},
	title        = {Persistent currents in one-dimensional systems of strongly correlated electrons},
	journal      = {Low Temperature Physics},
	year         = 1995,
	volume       = 21,
	pages        = 533,
}

@Article{khondker1988a,
author = {Khondker, AN and Khan, M Rezwan and Anwar, AFM}, 
editor = {}, 
title = {Transmission line analogy of resonance tunneling phenomena: The generalized impedance concept}, 
journal = {Journal of applied physics}, 
volume = {63}, 
number = {10}, 
pages = {5191--5193}, 
year = {1988}, 
abstract = {This paper presents a simple yet accurate method for solving the Schr{\"o}dinger equation to calculate the quantum mechanical transmission probability across arbitrary potential barriers. It is based on the concept of wave impedance analogous to transmission line ...}, 
location = {}, 
keywords = {}}


@Article{anwar1989a,
author = {Anwar, AFM and Khondker, AN and Khan, M Rezwan}, 
editor = {}, 
title = {Calculation of the traversal time in resonant tunneling devices}, 
journal = {Journal of applied physics}, 
volume = {65}, 
number = {7}, 
pages = {2761--2765}, 
year = {1989}, 
abstract = {Transmission line techniques are used to calculate the traversal time of electrons in resonant tunneling structures. It is suggested that the real part of the quantum-mechanical wave impedance Re [(2?/m*) ?'/?], at resonance, can be used to calculate the electron ...}, 
location = {}, 
keywords = {}}


@Article{kabir1991,
author = {Kabir, SM Fazlul and Khan, MR and Alam, MA}, 
editor = {}, 
title = {Application of quantum mechanical wave impedance in the solution of Schrodinger's equation in quantum wells}, 
journal = {Solid-state electronics}, 
volume = {34}, 
number = {12}, 
pages = {1466--1468}, 
year = {1991}, 
abstract = {Determination of eigenenergies and eigenfunctions are important in the design of quantum tunneling devices and in other quantum mechanical problems. The geometry of the quantum well can make the solution of the time-dependent Schrodinger's equation very complicated ...}, 
location = {}, 
keywords = {}}


@Article{stamp1996,
author = {Stamp, AP and McIntosh, GC}, 
editor = {}, 
title = {A time-dependent study of resonant tunneling through a double barrier}, 
journal = {American Journal of Physics}, 
volume = {64}, 
number = {3}, 
pages = {264--276}, 
year = {1996}, 
abstract = {The resonant tunneling of a wave packet is studied, for a one-dimensional double barrier, by solving the time-dependent Schr{\"o}dinger equation. The transmission is determined as a function of the spatial width of the incident wave packet. It is shown that if the double barrier ...}, 
location = {}, 
keywords = {}}


@Article{mokhov2008,
author = {Mokhov, Sergiy and Zeldovich, Boris Ya}, 
editor = {}, 
title = {Strength of electromagnetic, acoustic and Schr{\"o}dinger reflections}, 
journal = {Proceedings of the Royal Society A: Mathematical, Physical and Engineering Sciences}, 
volume = {464}, 
number = {2099}, 
pages = {3071--3080}, 
year = {2008}, 
abstract = {The notion of reflection strength S of a plane wave by an arbitrary non-absorbing layer is introduced, so that the intensity of reflection is R= tanh2 S. We have shown that the total strength of reflection by a sequence of elements is expressed through particular element ...}, 
location = {}, 
keywords = {}}


@phdthesis{Dinardo2018,
   author = {Dinardo, Brad Anthony},
   title = {Single Atom Delivery into a Bottle Beam Trap Using an Optical Conveyor Belt and Quantum Coherent Gain in a Matterwave Transistor},
   type = {Dissertation},
   URL = { https://scholar.colorado.edu/concern/graduate_thesis_or_dissertations/qz20ss555},
   type = {Thesis}
}

@article{Lui.1986, 
year = {1986}, 
title = {{Exact solution of the Schrodinger equation across an arbitrary one‐dimensional piecewise‐linear potential barrier}}, 
author = {Lui, Wayne W and Fukuma, Masao}, 
journal = {Journal of Applied Physics}, 
issn = {0021-8979}, 
doi = {10.1063/1.337788}, 
pages = {1555--1559}, 
number = {5}, 
volume = {60}, 
local-url = {file://localhost/Users/dana/Documents/Papers%20Library/Lui-Exact%20solution%20of%20the%20Schrodinger%20equation%20across%20an%20arbitrary%20one‐dimensional%20piecewise‐linear%20potential%20barrier-1986-Journal%20of%20Applied%20Physics.pdf}
}
@article{Ando.1987, 
year = {1987}, 
title = {{Calculation of transmission tunneling current across arbitrary potential barriers}}, 
author = {Ando, Yuji and Itoh, Tomohiro}, 
journal = {Journal of Applied Physics}, 
issn = {0021-8979}, 
doi = {10.1063/1.338082}, 
pages = {1497--1502}, 
number = {4}, 
volume = {61}, 
local-url = {file://localhost/Users/dana/Documents/Papers%20Library/Ando-Calculation%20of%20transmission%20tunneling%20current%20across%20arbitrary%20potential%20barriers-1987-Journal%20of%20Applied%20Physics.pdf}
}
@article{Nelin.2007, 
year = {2007}, 
keywords = {Impedance}, 
title = {{Impedance model for quantum-mechanical barrier problems}}, 
author = {Nelin, Evgenii A.}, 
journal = {Physics-Uspekhi}, 
doi = {10.1070/pu2007v050n03abeh006091}, 
url = {https://iopscience.iop.org/article/10.1070/PU2007v050n03ABEH006091/pdf}, 
abstract = {{Application of the impedance model to typical quan- tum-mechanical barrier problems, including those for structures with resonant electron tunneling, is discussed. The efficiency of the approach is illustrated. The physical transparency and compactness of the model and its potential as a teaching and learning tool are discussed.}}, 
pages = {293}, 
volume = {50}, 
local-url = {file://localhost/Users/dana/Documents/Papers%20Library/Nelin-Impedance%20model%20for%20quantum-mechanical%20barrier%20problems-2007-Physics-Uspekhi.pdf}
}
@article{Gutiérrez-Medina.2013, 
year = {2013}, 
title = {{Wave transmission through periodic, quasiperiodic, and random one-dimensional finite lattices}}, 
author = {Gutiérrez-Medina, Braulio}, 
journal = {American Journal of Physics}, 
issn = {0002-9505}, 
doi = {10.1119/1.4765628}, 
pages = {104--111}, 
number = {2}, 
volume = {81}, 
local-url = {file://localhost/Users/Dana/Downloads/1.4765628.pdf}
}

@article{anderson2021matterwaves,
      title={Matterwaves, Matterons, and the Atomtronic Transistor Oscillator}, 
      author={Dana Z. Anderson},
      year={2021},
      eprint={2106.10550},
      archivePrefix={arXiv},
      primaryClass={quant-ph}
}
